Understanding new tasks through the lens of training data via exponential tilting

Deploying machine learning models to new tasks is a major challenge despite the large size of the modern training datasets. However, it is conceivable that the training data can be reweighted to be more representative of the new (target) task. We consider the problem of reweighing the training samples to gain insights into the distribution of the target task. Specifically, we formulate a distribution shift model based on the exponential tilt assumption and learn train data importance weights minimizing the KL divergence between labeled train and unlabeled target datasets. The learned train data weights can then be used for downstream tasks such as target performance evaluation, fine-tuning, and model selection. We demonstrate the efficacy of our method on Waterbirds and Breeds benchmarks.

==> YK-macros.tex <==

\def\Avar{\textrm{Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{\textrm{aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{\textrm{avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{\textrm{bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{\textrm{Ber}}
\def\bin{\textrm{bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{\textrm{cat}}
\def\Cov{\textrm{Cov}}
\def\cov{\textrm{cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{\textrm{cl}}
\def\complex{{\bbC}}
\def\cone{\textrm{cone}}
\def\conv{\textrm{conv}}
\def\deq{\overset{d}{=}}
\def\det{\textrm{det}}
\def\diag{\textrm{diag}}
\def\diam{\textrm{diam}}
\def\dist{\textrm{dist}}
\def\dom{\textrm{dom}}
\def\doop{\textrm{do}}
\def\dto{\overset{d}{\to}}
\def\Ex{{\bE}}
\def\Exp{\textrm{Exp}}
\def\exp{\textrm{exp}}
\def\eg{{\it e.g.}}
\def\epi{\textrm{epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\IID{\textrm{IID}}
\def\ind{\textrm{ind}}
\def\intr{\textrm{int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{\textrm{KL}}
\def\ker{\textrm{ker}}
\def\lspan{\textrm{span}}
\def\maximize{\textrm{maximize}}
\def\med{\textrm{med}}
\def\minimize{\textrm{minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{\textrm{Poi}}
\def\Pr{{\bP}}
\def\peq{\overset{p}{=}}
\def\plim{\textrm{plim}}
\def\proj{\textrm{proj}}
\def\prox{\textrm{prox}}
\def\pto{\overset{p}{\to}}
\def\ran{\textrm{ran}}
\def\rank{\textrm{rank}}
\def\reals{{\bR}}
\def\relint{\textrm{relint}}
\def\sign{\textrm{sign}}
\def\st{\textrm{st}}
\def\subjectto{\textrm{subject to}}
\def\supp{\textrm{supp}}
\def\symm{{\bS}}

\def\Tr{\textrm{Tr}}
\def\tr{\textrm{tr}}
\def\tube{\textrm{tube}}
\def\TV{\textrm{TV}}
\def\unif{\textrm{unif}}
\def\Var{\textrm{Var}}
\def\var{\textrm{var}}
\def\vct{\textrm{vec}}
\def\veps{\varepsilon}
\def\vol{\textrm{vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> exponential-tilt(ICLR2023)/SM-macros.tex <==
\newcommand{\klloss}{\mathfrak{L}}
\def\heta{\widehat{\eta}}
\def\hf{{\hat f}}
\def\hP{\widehat{P}}
\def\hp{\widehat{p}}
\def\hQ{\widehat{Q}}
\def\hq{\widehat{q}}
\def\htheta{\widehat{\theta}}
\def\sf{{f^\star}}
\def\tf{{\tilde f}}
\def\htheta{{\hat \theta}}
\def\stheta{{\theta^\star}}
\def\hL{\hat L}
\def\sL{{L^\star}}
\renewcommand{\Vec}{\operatorname{vec}}
\newcommand{\breeds}{\textsc{Breeds}}
\newcommand{\waterbirds}{\textsc{Waterbirds}}
\newcommand{\strongconvexity}{\mu}
\newcommand{\nsource}{{n_P}}
\newcommand{\ntarget}{{n_Q}}
\newcommand{\weight}{\omega}
\newcommand{\coef}{\xi}
\newcommand{\scoef}{\coef^\star}
\newcommand{\hcoef}{{\hat \coef}}

==> exponential-tilt(ICLR2023)/YK-macros.tex <==

\def\Avar{\textrm{Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{\textrm{aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{\textrm{avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{\textrm{bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{\textrm{Ber}}
\def\bin{\textrm{bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{\textrm{cat}}
\def\Cov{\textrm{Cov}}
\def\cov{\textrm{cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{\textrm{cl}}
\def\complex{{\bbC}}
\def\cone{\textrm{cone}}
\def\conv{\textrm{conv}}
\def\deq{\overset{d}{=}}
\def\det{\textrm{det}}
\def\diag{\textrm{diag}}
\def\diam{\textrm{diam}}
\def\dist{\textrm{dist}}
\def\dom{\textrm{dom}}
\def\doop{\textrm{do}}
\def\dto{\overset{d}{\to}}
\def\Ex{{\bE}}
\def\Exp{\textrm{Exp}}
\def\exp{\textrm{exp}}
\def\eg{{\it e.g.}}
\def\epi{\textrm{epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\IID{\textrm{IID}}
\def\ind{\textrm{ind}}
\def\intr{\textrm{int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{\textrm{KL}}
\def\ker{\textrm{ker}}
\def\lspan{\textrm{span}}
\def\maximize{\textrm{maximize}}
\def\med{\textrm{med}}
\def\minimize{\textrm{minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{\textrm{Poi}}
\def\Pr{{\bP}}
\def\peq{\overset{p}{=}}
\def\plim{\textrm{plim}}
\def\proj{\textrm{proj}}
\def\prox{\textrm{prox}}
\def\pto{\overset{p}{\to}}
\def\ran{\textrm{ran}}
\def\rank{\textrm{rank}}
\def\reals{{\bR}}
\def\relint{\textrm{relint}}
\def\sign{\textrm{sign}}
\def\st{\textrm{st}}
\def\subjectto{\textrm{subject to}}
\def\supp{\textrm{supp}}
\def\symm{{\bS}}

\def\Tr{\textrm{Tr}}
\def\tr{\textrm{tr}}
\def\tube{\textrm{tube}}
\def\TV{\textrm{TV}}
\def\unif{\textrm{unif}}
\def\Var{\textrm{Var}}
\def\var{\textrm{var}}
\def\vct{\textrm{vec}}
\def\veps{\varepsilon}
\def\vol{\textrm{vol}}
\def\zeros{\mathbf{0}}


==> exponential-tilt(ICLR2023)/YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> exponential-tilt(ICLR2023)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> exponential-tilt(ICLR2023)/sections/LDA.tex <==
\section{Synthetic experiment: normal mixture}
\label{sec:normal-mixture}
% \begin{wrapfigure}[15]{r}{0.5\linewidth}
% \vspace{-0.12in}
%     \centering
%     \includegraphics[width=\linewidth]{plots/LDA_data.pdf}
%     \vspace{-0.23in}
%     \caption{Data for synthetic experiments}
%     \label{fig:LDA-data}
% \end{wrapfigure}

\begin{wrapfigure}[14]{r}{0.5\linewidth}
\vspace{-0.25in}
    \centering
    \includegraphics[width=\linewidth]{plots/Acc.pdf}
    \vspace{-0.23in}
    \caption{Target accuracies for different models and for different $\delta$ values. }
    \label{fig:LDA-exptilt}
\end{wrapfigure}

We demonstrate utility of the ExTRA weights for reweighing source data in the following synthetic experiment. As seen in Figure \ref{fig:LDA-data} both the source and target distributions are associated with binary classification tasks and their class conditionals are normally distributed in $\reals^2$. More specifically, the class conditionals in source distribution have means $(-\delta, -2)^\top$ and $(\delta, 2)^\top$ for classes 1 and 0 resp., whereas the means in target distributions are $(\delta, -2)^\top$ and $(-\delta, 2)$. All the class conditionals have variances $\bI_2$. This is an instance of concept drift which does not fall under subpopulation shift (considering classes as subpopulations).

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{plots/LDA_data.pdf}~\includegraphics[width=0.45\linewidth]{plots/LDA_data2.pdf}
    \caption{Source and target data with $\delta = 1$ (left) and $\delta = 2$ (right).}
    \label{fig:LDA-data}
\end{figure}



The distribution shift in this example satisfies exponential tilt assumption with sufficient statistic $T(x_1, x_2) = x_1$. In our experiment we use two sufficient statistics: (1) $T(x_1, x_2) = x_1$ - an ideal sufficient statistic for this example and (2) $T(x_1,x_2) = (x_1, x_ 2) $ - a simple choice for a sufficient statistic. 
Here, we vary $\delta$ to control the overlap between the class conditionals in corresponding classes. For a small $\delta$ the source and target class conditionals for class 0 (or 1) have overlapping support, satisfying the anchor-set assumption in Definition \ref{def:anchor-set}.



We compare the target accuracies of three different models trained on: (1) source data (S->T), (2) ExTRA weighted source data using $T(x_1, x_2) = x_1$, and (3) ExTRA weighted source data using $T(x_1, x_2) = (x_1, x_2)$. As we see in Figure \ref{fig:LDA-exptilt}, the ideal sufficient statistic $T(x_1, x_2) = x_1$ produces better target accuracy than the other two models. We also observe that $T(x_1, x_2) = (x_1, x_2)$ has better target accuracy than S->T for small values of $\delta$. The reason for such observation goes back to the anchor set condition in Definition \ref{def:anchor-set}. As we see in Figure \ref{fig:LDA-data}, left plot, a small $\delta$ ($\delta = 1$) results in support overlap between source and target class conditionals for class $0$ (and $1$), and the overlapped region of support works as anchor set. On contrary, large $\delta$'s (Figure \ref{fig:LDA-data}, right plot) has very little overlap, resulting in violation in  the anchor set assumption and leading to a non-identifiability in the exponential tilt model for sufficient statistic $T(x_1, x_2) = (x_1, x_2)$. Nevertheless, the ideal sufficient statistic $T(x_1, x_2) = x_1$ continues to work even for large $\delta$.

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{plots/wd.pdf}~\includegraphics[width=0.45\linewidth]{plots/LDA_weighted.pdf}
    \caption{\emph{Left}: Wasserstein distances between source vs target, weighted source vs target and target vs target data. \emph{Right}: Scatter plot for weighted source (highlighted according to the ExTRA weights) and target data. }
    \label{fig:LDA-distribution-matching}
\end{figure}

% \begin{wrapfigure}[15]{r}{0.5\linewidth}
% \vspace{-0.12in}
%     \centering
%     \includegraphics[width=\linewidth]{plots/wd.pdf}
%     \vspace{-0.23in}
%     \caption{}
%     \label{fig:LDA-wd}
% \end{wrapfigure}

We also investigate whether reweighed source data with ExTRA weights better approximates the target data compared to the uniformly weighted source data. We first compare the following Wasserstein distances between target and: (1) source (S->T), (2) target (T->T), (3) ExTRA weighted source with $T(x_1, x_2) = (x_1, x_2)$, and (4) ExTRA weighted source with $T(x_1, x_2) = x_1$ for several values of $\delta$. 
As we see in Figure \ref{fig:LDA-distribution-matching} left plot, ExTRA weighted source data is closer to the target data compared to the uniformly weighted source data. Similar to the target accuracy inspection (Figure \ref{fig:LDA-exptilt}), the sufficient statistic  $T(x_1, x_2) = x_1$ shows better performance in adapting to the target distribution than $T(x_1, x_2) = (x_1, x_2)$. In  Figure \ref{fig:LDA-distribution-matching} right panel, we compare the weighted source data for $\delta = 1$ when the ExTRA weights are calculated with sufficient statistic $T(x_1, x_2) = (x_1, x_2)$. Compared to the uniformly weighted source data (see Figure \ref{fig:LDA-data}, left plot) we see that ExTRA weighted source data is also closer to the target one qualitatively.



==> exponential-tilt(ICLR2023)/sections/conclusion.tex <==
\vspace{-0.25cm}
\section{Conclusion}
% \vspace{-0.25cm}
In this paper, we developed an importance weighing method for approximating expectations of interest on new domains leveraging unlabeled samples (in addition to a labeled dataset from the source domain). We demonstrated the applicability of our method on downstream tasks such as model evaluation/selection and fine-tuning both theoretically and empirically.
% evaluating the out-of-distribution risk of ML models that leverages unlabeled samples from the target domain (in addition to a labeled validation dataset from the source domain).
Unlike other importance weighing methods that only allow covariate shift between the source and target domains, we permit concept drift between the source and target. Though we demonstrate the efficacy of our method in synthetic setup of concept drift (Appendix \ref{sec:normal-mixture}), in a future research it would be interesting to investigate the performance in more realistic setups (\eg\ 
 CIFAR10.2 to CIFAR10.2 \citep{lu2020harder}, Imagenet to Imagenetv2 \citep{recht2019imagenet}). 
% We demonstrate the efficacy of the method by using it to perform fine-tuning and model selection.

Despite its benefits, the exponential tilt model does suffer from a few limitations. Implicit in the exponential tilt assumption is that the supports of the target class conditionals have some overlap with the corresponding source class conditionals. Although this assumption is likely satisfied 
in many instances of 
% in the subpopulation shift setting, they are violated in
domain generalization problems (and is always satisfied in the subpopulation shift setting), 
% \citep{koh2020WILDS},
an interesting avenue for future studies is to accommodate support alignment in the distribution shift model, \ie\ to align the supports for class conditioned feature distributions in source and target domains. One way to approach this is to utilize distribution matching techniques from domain adaptation literature \citep{ganin2016Domainadversarial,sun2016Deep,shen2018wasserstein}, similarly to \citet{cai2021Theory}. We hope aligning supports via distribution matching will allow our method to succeed on domain generalization problems where the support overlap assumption is violated.  



==> exponential-tilt(ICLR2023)/sections/convergence-tilt.tex <==


\subsection{Consistency in estimation of the tilt parameters}


Here, we establish a convergence rate for the estimated tilt parameters (Lemma \eqref{lemma:KL-distribution-matching}) and the ExTRA importance weights (Equation \eqref{lemma:KL-distribution-matching}). To simplify the notation, we define $S(x) = (1, T(x)^\top)^\top$ as the extended sufficient statistics for the exponential tilt and denote the corresponding tilt parameters as $\coef_k = (\alpha_k, \theta_k^\top)^\top$.  We let $\coef_k^\star = (\alpha_k^\star, {\theta_k^\star}^\top )^\top$'s  be the true values of the tilt parameters $\coef_k$'s and let $\coef = (\coef_1^\top, \dots, \coef_K^\top)^\top\in \reals^{K(p+1)}$  be the long vector containing  all the tilt parameters. 
We recall that estimating the parameters from the optimization stated in Lemma  \ref{lemma:KL-distribution-matching}  requires a classifier $\heta_P$ on the source data. So, we define our objective for estimating $\coef$ through a generic  classifier $\eta : \cX \rightarrow \Delta^{K}$. Denoting $\eta_k(x)$ as the $k$-th co-ordinate of $\eta(x)$ we define the expected log-likelihood objective as:
\[
\textstyle
\klloss(\eta, \coef) = \Ex_{Q_X}[\log \{ \sum_{k = 1}^K \eta_k(X) \exp(\coef_k^\top S(X)) \}] - \log [\Ex_{P} \{  \exp(\coef_Y^\top S(X)) \}]\,,
\] and its empirical version as 
\[
\textstyle
\hat \klloss(\eta, \coef) = \Ex_{\hQ_X}[\log \{ \sum_{k = 1}^K \eta_k(X) \exp(\coef_k^\top S(X)) \}] - \log [\Ex_{\hP} \{  \exp(\coef_Y^\top S(X)) \}]\,.
\] 


% The term   $\log [\Ex_{P} \{  \exp(\coef_Y^\top S(X)) \}]$ in the  objective works as a normalizer: for any $\eta : \cX \to \Delta^K$ the function $[ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) ]/[\Ex_{P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}] $ is a density over the support $\cX$ with respect to the base measure $P_X$. Furthermore, plugging in the Bayes classifier $\eta^\star_P$ (defined as $\eta^\star_{P, k}(x) = p\{x, Y = k\}/p_X(x)$) and  $\scoef$ we realize that the quantity $\sum_{k = 1}^K \eta_{P, k}^\star(x) \exp(\coef_k^\top S(x))$ is a density with respect to the base measure $P_X$, as we explain in the following display: 
% \[\textstyle
% \sum_{k = 1}^K \eta_{P, k}^\star(x) \exp\{{\coef_k^\star}^\top S(x)\} = \sum_{k = 1}^K \frac{p\{x, Y = k\}}{p_X(x)} \exp\{{\coef_k^\star}^\top S(x)\} =  \frac{\sum_{k = 1}^K q\{x, Y = k\}}{p_X(x)} = \frac{q_X(x)}{p_X(x)}
% \]
% and hence it holds $\Ex_{P_X} \{ \sum_{k = 1}^K \eta_{P, k}^\star(x) \exp\{{\coef_k^\star}^\top S(x)\} = 1$. In the next lemma we establish that $\scoef$ is the unique maximizer of $\klloss(\eta_P^\star, \coef)$, which is crucial for establishing that $\hcoef$ converges to $\scoef$. 

% \begin{lemma}\label{lemma:uniqueness}
% $\coef \mapsto \klloss(\eta_P^\star, \coef)$ is uniquely maximized at $\scoef$. 
% \end{lemma}



To establish the consistency of MLE we first make an assumption that the loss $\coef \mapsto -\klloss(\eta^\star_P, \coef)$ is strongly convex at the true parameter value. 
\begin{assumption}
\label{assmp:strong-convexity}
The loss $\coef \mapsto -\klloss(\eta^\star_P, \coef)$ is  strongly convex at $\scoef$, \ie, there exists a constant $\strongconvexity>0$ such that for any $\coef$ it holds:
\[ \textstyle
-\klloss(\eta^\star_P, \coef) \ge -\klloss(\eta^\star_P, \scoef) - \partial_\coef\klloss(\eta^\star_P, \scoef)  ^\top (\coef - \scoef) +\frac{\mu}{2}\|\coef - \scoef\|_2^2\,. 
\]
\end{assumption}
We note that the assumption is a restriction on the distribution $Q$ rather than the objective itself. For technical convenience we next assume that the feature space is bounded. 


\begin{assumption} \label{assump:bounded-covariate}
$\cX$ is bounded, \ie, there exists  an $M>0$ such that $\cX \subset B(0, M)$.
\end{assumption}

Recall, from Lemma \ref{lemma:KL-distribution-matching}, that we need a fitted source classifier $\heta_P$  to estimate the tilt parameter: $\scoef$ is estimated by maximizing $\hat \klloss(\heta_P, \coef)$ rather than the unknown $\hat \klloss(\eta_P^\star, \coef)$. While analyzing the convergence of $\hcoef$ we are required to control the difference  $\hat \klloss(\hat \eta_P, \coef) - \hat \klloss(\eta_P^\star, \coef)$. 
% This  requires the preactivated logit functions (definition follows) for $\heta_P$ to be close to $\eta_P^\star$.
% \begin{definition}[Preactivated logit function] \label{def:pre-activation-logit}
% A  function $f: \cX \to \reals^K$ is a preactivation logit
% function for a generic  probabilistic classifier $\eta: \cX \to \Delta^K$ if it satisfies \[ \textstyle
% \frac{\exp(f_k(x))}{\sum_{j = 1}^K \exp(f_j(x))} =  \eta_k(x)\,.
% \]
% \end{definition}
% We notice that the preactivation logit functions are not unique:  if $f$ is a pre-activation function for a probabilistic classifier $\eta$ then for any $a:\cX\to \reals$ it holds \[
% \textstyle
% \frac{\exp(f_k(x))}{\sum_{j = 1}^K \exp(f_j(x))} = \frac{\exp(f_k(x)+a(x))}{\sum_{j = 1}^K \exp(f_j(x) +a(x))} 
% \]   \ie\ both $\{f_k(x)\}_{k = 1}^K$ and $\{f_k(x) + a(x)\}_{k = 1}^K$ are valid preactivation functions $\eta$.  We induce the uniqueness by considering  the centered logit function: a preactivation logit  function $f$ of a classifier $\eta$ is centered if it satisfies $\sum_{k = 1}^Kf_k(x) = 0 $ for all $x \in \cX$. The centered logit functions are unique since it holds:
% \[ \textstyle
% \frac{\exp(f_k(x))}{\sum_{j = 1}^K \exp(f_j(x))} =  \eta_k(x), ~ \sum_{j = 1}^K{f_j(x)} = 0  \Longleftrightarrow f_k(x) = \log\{\eta_k(x)\} - \frac1K \sum_{j = 1}^K \log\{\eta_j(x)\}\,.\]
To ensure the difference is small, assume the pilot estimate of the source regression function $\heta_P$ is consistent at some rate $r_{n_P}$.
% We next assume that the centered logit for $\heta_P$ convegres to the one for $\eta_P^\star $. 
\begin{assumption}
\label{assmp:source-classifier}
Let $f_{P, k}^\star(x) = \log\{\eta_{P, k}^\star(x)\} - \frac 1K \sum_{j = 1}^K \log\{\eta_{P, j}^\star(x)\}$. We assume that there exist an estimators $\{\hat f _{P, k}(x)\}_{k =1 }^K$ for $\{f^\star_{P, k}(x)\}_{k = 1}^K$ such that the following holds: there exists a constant $c>0$ and a sequence  $r_{n_P} \to 0$ such that  for almost surely $[\bbP_X]$  it holds
\[\textstyle
\Pr(\|\hat f_P(x) - f_P^\star(x)\|_{2} > t) \le \exp(-c t^2 /r_{n_P}^2), ~ t > 0\,.
\]
\end{assumption}
We use the estimated logits $\{\hat f _{P, k}(x)\}_{k =1 }^K$ to construct the regression functions as  $\heta_{P, k}(x) = \exp(\hat f_{P, k}(x))/\{\sum_{j = 1}^K \exp(\hat f_{P, j}(x))\}$, which we use in the objective stated in Lemma  \ref{lemma:KL-distribution-matching} to analyze the convergence of the tilt parameter estimates and the ExTRA weights.  With the above assumptions we're now ready to state concentration bounds for $\hcoef - \scoef$ and  $\hat \weight - \weight^\star$, where  the true importance weight $\weight^\star$ is  defined as $\weight^\star(x, y) = \exp({\coef_y^\star}^\top S(x))$. 

\begin{theorem} \label{thm:tilt-concentration}
Let the assumptions \ref{assmp:strong-convexity}, \ref{assump:bounded-covariate} and \ref{assmp:source-classifier} hold. For the sample sizes $n_P, n_Q$ define $\alpha_{n_P, n_Q} = r_{n_P} \sqrt{\log(n_Q)}+ {\{(p+1)K/{n_P}\} }^{1/2} + {\{(p+1)K/n_Q\} }^{1/2}$. There exists constants $k_1, k_2>0$ such that for any $\delta>0$ with probability at least $1 - (2K+ 1)\delta$ the following hold:
\[
\|\hcoef - \scoef \|_2 \le k_1 \alpha_{n_P, n_Q}\sqrt{\log(1/\delta)}, \text{ and } \|\hat \weight - \weight^\star\|_{1, P} \le k_2 \alpha_{n_P, n_Q}\sqrt{\log(1/\delta)}. 
\]
\end{theorem}
In Theorem \ref{thm:tilt-concentration} we notice that as long as $r_{n_P} \log(n_Q) \to 0$ for $n_P, n_Q\to \infty$ we have $\alpha_{n_P,n_Q} \to 0$. This implies both \emph{the estimated tilt parameters and the ExTRA weights converge to their true values as the sample sizes $n_P, n_Q\to \infty$}. 



% \my{summarize the implications of theoretical results}
% \YK{If we need space, we can defer the fine-tuning theory and model evaluation theory to the supplement}
We next provide theoretical guarantees for the downstream tasks (1) fine-tuning and (2) target performance evaluation that we described in Section \ref{sec:exponential-tilt}. 

\paragraph{Fine-tuning}
We establish a generalization bound for the fitted model \eqref{eq:weighted-ERM} using weighted-ERM on source domain.
% To begin with we define notations. 
We denote $\cF$ as the classifier hypothesis class. For $f \in \cF$ and a weight function $\weight: \cX \times \cY \to \reals_{\ge 0} $ define the weighted loss function and its empirical version on source data as: 
\[ \textstyle
\cL_P(f, w) = \Ex_{P} [\weight(X, Y)\ell(f(X), Y)], ~ \hat \cL_P (f, w) = \Ex_{\hP} [\weight(X, Y)\ell(f(X), Y)]\,.
\] We also define the loss function on the target data as: $
\cL_Q(f) = \Ex_{Q} \big[\ell(f(X), Y)\big]\,.$
If $\{(\theta_k^\star, \alpha_k^\star)\}_{k = 1}^K$ is the true value of the tilt parameters in  \eqref{eq:exponential-tilt}, \ie, the following holds:
\[ \textstyle
  q\{x, Y = k\} = p\{x, Y = k\} \exp\{\alpha_k^\star + (\theta_k^\star)^\top T(x)\}; \ k \in [K]\,,
\] then defining $\weight^\star(x, k) = \exp\{\alpha_k^\star + (\theta_k^\star)^\top T(x)  \}$ as the true weight we notice that  $\cL_P(f, \weight^\star) = \cL_Q(f)$, which is easily observed by setting $g(x, y) = \ell(f(x), y)$ in the display \eqref{eq:true-weighted-expectation}.

% as we show in the  following display:
% \[ \textstyle
% \begin{aligned}
% \cL_P(f, \weight^\star) 
%  & = \int \sum_{y= 1}^K \weight^\star (x, y) \ell\{f(x), y\} p\{x, Y = y\} dx\\
%  & = \int \sum_{y= 1}^K  \ell\{f(x), y\} q\{x, Y = y\} dx=\cL_Q(f)\,.
% \end{aligned}
% \] 

% We next define the Rademacher complexity \cite{bartlett2002rademacher} that  has been frequently used in  machine learning literature to establish a generalization bound. 
% Instead of considering the Rademacher complexity on $\cF$ we define the class of weighted losses $\cG(\ell, \cF) = \{g_f(x, y) = w^\star(x, y) \ell(f(x), y): \ f \in \cF\}$  and for $n \in \bbN$ we define its Rademacher complexity measure as 
% \[ \textstyle
%     \cR_n(\cG) \triangleq \Ex_{\{(u_i, v_i)\}_{i = 1}^n\stackrel{\IID}{\sim} P} \big[\Ex_{\{\xi_i\}_{i = 1}^n}[\sup_{f \in \cF} \frac1{n} \sum_{i = 1}^n \xi_i \weight^\star(u_i, v_i) \ell \{f(u_i), v_i\}]\big]
% \]
% where $\{\xi_i\}_{i = 1}^n $ are \IID \ symmetric Rademacher random variables. 


To establish our generalization bound we require Rademacher complexity \citep{bartlett2002rademacher} (denoted as $\cR_{n_P}(\cG)$; see Appendix \ref{supp:rademacher} for details) and the following assumption on the loss function.

\begin{assumption}
\label{assump:bounded-loss}
The loss function $\ell$ is bounded, \ie, for some $B>0$, $|\ell\{f(x), y\}| \le B$ for any $f\in \cF$, $x \in \cX$ and $y \in [K]$. 
\end{assumption}

With the above definitions and the assumption we  establish our generalization bound. 

\begin{lemma}
\label{lemma:generalization-bound} For a weight function $\weight$ and the source samples $\{(X_{P, i}, Y_{P, i})\}_{i = 1}^\nsource$ of size $\nsource$ let $\hat f_{\weight} = \argmin_{f\in\cF} \hat \cL_P(f, \weight)$. There exists a constant $c> 0$ such that  the following generalization bound holds with probability at least $1 -\delta$
\begin{equation}\textstyle
\label{eq:gen-bound}
    \cL_Q(\hat f_{ \weight}) - \min_{f\in\cF}\cL_Q (f) \le  2 \cR_{n_P}(\cG) + B  \| \weight - \weight^\star \|_{1, P} + c \sqrt{\frac{\log(1/\delta)}{\nsource}} \,,
\end{equation} where $\cR_{n_P}(\cG)$ is the Rademacher complexity of $\cG = \{ \weight^\star(x, y) \ell(f(x), y): \ f \in \cF\}$  defined in Appendix A.1. 
\end{lemma}
In Theorem \ref{thm:tilt-concentration} we established an upper bound for the estimated weights $\hat \weight$, which concludes that $\hat f_{\hat \weight}$ has the following generalization bound:  for any $\delta > 0$, with probability at least $1 - (2K+ 2)\delta$
\[ \textstyle
\cL_Q(\hat f_{ \hat \weight}) - \min_{f\in\cF}\cL_Q (f) \le  2 \cR_{n_P}(\cG)  + k_2\alpha_{\nsource, \ntarget} \sqrt{\log(1/\delta)} + c \sqrt{\log(1/\delta)/\nsource} \,,
\] where $k_2$ is the constant in Theorem \ref{thm:tilt-concentration} and $c$ is the constant in Lemma \ref{lemma:generalization-bound}. The generalization bound implies that for large sample sizes ($n_P, n_Q\to \infty$) the target accuracy of weighted ERM on source data well approximates the accuracy of ERM on target data.


\paragraph{Target performance evaluation}

We provide a theoretical guarantee for the target performance evaluation \eqref{eq:target-performance} using our importance weights. Here we only consider the functions $g:\cX \times \cY \to \reals$ which are bounded by some $B>0$, \ie\ $|g(x, y)| \le B$ for all $x\in \cX$ and $y \in \cY$. The simplest and the most frequently used example is the model accuracy which uses $0\text{-} 1$-loss as the loss function: for a model $f$ the loss $g(x, y) = \bbI\{f(x) = y\}$ is bounded with $B = 1$. For such functions  we notice that $\Ex_{Q}[g(X, Y)] = \Ex_{P}[g(X, Y)\weight^\star(X, Y)]$, as observed in display \eqref{eq:true-weighted-expectation}.
% \[
% \begin{aligned}
% \Ex_{Q}[g(X, Y)] & = \textstyle\int \sum_{y= 1}^K  g(x, y) q\{x, Y = y\} dx\\
% &=\textstyle \int \sum_{y= 1}^K  g(x, y) p\{x, Y = y\} \weight^\star(x, y) dx = \Ex_{P}[g(X, Y)\weight^\star(X, Y)]
% \end{aligned}
% \] 
This implies the following bound on the target performance evaluation error 
\[
\begin{aligned}
\big|\Ex_{Q}[g(X, Y)] - \Ex_{P}[g(X, Y)\hat \weight(X, Y)]\big|& = \big|\Ex_{P}[g(X, Y)\weight^\star(X, Y)] - \Ex_{P}[g(X, Y)\hat \weight(X, Y)]\big|\\
& \le B \Ex_{P}[|\hat \weight^\star(X, Y)- \weight^\star (X, Y)|]
 \le B \|\hat \weight - \weight^\star\|_{1, P}\,.
\end{aligned}
\] We recall the concentration bound for $\|\hat \weight - \weight^\star\|_{1, P}$ from Theorem \ref{thm:tilt-concentration} and conclude that the \emph{estimated target performance in \eqref{eq:target-performance} converges to the true target performance} at rate $\alpha_{\nsource, \ntarget}$. 

==> exponential-tilt(ICLR2023)/sections/estimation.tex <==
\section{Estimation of the exponential tilt parameters}

In this section we present a method for estimating the tilt parameters.  Throughout the section we assume that the condition \ref{assmp:non-linear} is satisfied and the tilt parameters in \eqref{eq:exponential-tilt} are uniquely identified.



% There are several ways one can estimate the tilt parameters, a  popular approach is matching the distributions, where one can minimize a distribution between $q_X$ and the exponentially tilted mixture \eqref{eq:rep1}. In the following  subsection we consider the simple approach of moment matching. 

% \subsection{Moment matching approach}
% We estimate the tilt parameters by matching some moments for target marginal $q_X$ and source class conditionals $p_0$ and $p_1$. Specifically, for a suitably chosen $f(x)$ we solve the equation 
% \begin{equation}
%     \label{eq:moment-matching}
%     E_{\hat Q_X} [f(x)] = \hat \pi_Q E_{\hat P_1}\left[f(x) e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[f(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right]
%     \end{equation} to get the estimates $\hat \pi_Q, \hat \beta_0$ and $\hat \beta_1$. In the traditional moment matching setup we consider $f = 1, \Phi^{\otimes 1}(x) \Phi(x), \Phi^{\otimes 2}(x) = \Phi(x)\Phi(x)^\top, \dots $ to get the sufficiently many independent equations to estimate the parameters. More explicitly saying the parameters as estimated from the following independent equations: 
%     \begin{equation}
%         \begin{aligned}
%         1 = \hat \pi_Q E_{\hat P_1}\left[ e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[ e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right],\\
%         E_{\hat Q_X} [\Phi(x)] = \hat \pi_Q E_{\hat P_1}\left[\Phi(x) e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[\Phi(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right],\\
%         E_{\hat Q_X} [\Phi(x)\Phi(x)^\top] = \hat \pi_Q E_{\hat P_1}\left[\Phi(x)\Phi(x)^\top e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[\Phi(x)\Phi(x)^\top e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right],
%         \end{aligned}
%     \end{equation} where we note that any one of the three equations cannot be derived from the other two equations. 
    
    
    
    
%     A couple of questions immediately one might ask  are the followings:  What is the rate of convergence for the estimates and how does it depend on $f$? What would be a \emph{good} choice of $f$? To answers these question we decompose the right hand side of the equation \eqref{eq:moment-matching}. Here, we note that 
%     \begin{equation}
%         \begin{aligned}
% &  \hat \pi_Q E_{\hat P_1}\left[f(x) e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[f(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right]\\
% & =  \underbrace{\pi_Q E_{ P_1}\left[f(x) e^{ \alpha_1 + \beta_1^\top \Phi(x)}\right] + (1- \pi_Q) E_{ P_0}\left[f(x) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right]}_{(1)} \\
%  & ~~ + \underbrace{(1 - \hat \pi_Q) \big( E_{\hat P_0} - E_{P_0} \big) \left[f(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right]}_{(2.a)} + \underbrace{\hat \pi_Q \big( E_{\hat P_1} - E_{P_1} \big) \left[f(x) e^{\hat \alpha_1 + \hat \beta_1^\top
%  \Phi(x)}\right]}_{(2.b)} \\ 
%  & ~~ + \underbrace{(1 - \hat \pi_Q) E_{P_0} \left[f(x) \Big(e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}- e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\Big)\right]}_{(3.a)} \\
%  & ~~ +  \underbrace{\hat \pi_Q E_{P_1} \left[f(x) \Big(e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}- e^{ \alpha_1 +  \beta_1^\top \Phi(x)}\Big)\right]}_{(3.b)} \\
%  & ~~ + \underbrace{(\hat \pi_Q - \pi_Q) \left(E_{ P_1}\left[f(x) e^{ \alpha_1 + \beta_1^\top \Phi(x)}\right] -  E_{ P_0}\left[ f(x) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right]\right)}_{(4)}\,.
%         \end{aligned}
%     \end{equation}
    
    
% We start by observing that (1) is equal to $E_{Q_X}[f(x)]$ which is the population mean of the left hand side in equation \eqref{eq:moment-matching}. Hence, taking (1) in the other side would make the left hand side 
% \[(5)\triangleq E_{\hat Q_X}[f(x)] - E_{Q_X}[f(x)] \,,\] which is small in limit.   
% The magnitude of the  term $E_{ P_1}\left[f(x) e^{ \alpha_1 + \beta_1^\top \Phi(x)}\right] -  E_{ P_0}\left[ f(x) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right] = E_{ Q_1}[f(x)] - E_{ Q_0}[f(x)]$ in (4) contributes in the rate of convergence of $\hat \pi_Q - \pi_Q$, in a way that a bigger magnitude of $E_{ Q_1}[f(x)] - E_{ Q_0}[f(x)]$ would make $\hat \pi_Q - \pi_Q$ converge faster. So we require $E_{ Q_1}[f(x)] - E_{ Q_0}[f(x)]$ to be as big as possible in some norm. With the first order Taylor expansion on (3.a) we have \[
% \begin{aligned}
% & E_{P_0} \left[f(x) \Big(e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}- e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\Big)\right]\\
% & \approx E_{P_0} \left[f(x)\big((\hat \alpha_0 - \alpha_0 ) + (\hat \beta_0 - \beta_0)^\top \Phi(x)\big) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right]\\
% & = E_{Q_0} \left[f(x)\big((\hat \alpha_0 - \alpha_0 ) + (\hat \beta_0 - \beta_0)^\top \Phi(x)\big)\right]\,.
% \end{aligned}
% \] This implies that we require the magnitudes of $E_{Q_0}[f(x)]$ and $E_{Q_0}[\Phi(x)f(x)]$ to be as large as possible and similarly from (3.b) we require the magnitudes of $E_{Q_1}[f(x)]$ and $E_{Q_1}[\Phi(x)f(x)]$ to be as large as possible. The  error in estimation arises from (2.a), (2.b) and (5) and the error is higher for larger $\|f\|_\infty$. This contradicts with the requirement that larger magnitude of  $E_{Q_0}[f(x)\Phi(x)]$ and $E_{Q_1}[f(x)\Phi(x)]$ is better for estimation of $\hat \beta_0$ and $\hat \beta_1$. So, we fix some $L>0$ and try to find the best possible choice of $f$ with $\|f\|_\infty = L. $

\subsection{Maximum likelihood approach}

% Here one can consider maximizing the likelihood for the semi-supervised data. We denote $\eta_P(x)\triangleq P(y = 1|x) = \frac{\pi_P p_1(x)}{\pi_P p_1(x) + (1-\pi_P) p_0(x)}$ as the source regression function. With the labeled data for source and unlabeled data for target the likelihood is
% \begin{equation}
% \begin{aligned}
%  \cL & = \prod_{i = 1}^m \big(\pi_P p_1(x_i^{(P)})\big)^{y_i^{(P)}}\big((1-\pi_P) p_0(x_i^{(P)})\big)^{1-y_i^{(P)}}\\
%  & ~~~ \times \prod_{i=1}^n \left( \pi_Qp_1(x_i^{(Q)})e^{\alpha_1 + \beta_1^\top \Phi(x_i^{(Q)})} + (1-\pi_Q)p_0(x_i^{(Q)})e^{\alpha_0 + \beta_0^\top \Phi(x_i^{(Q)})}\right)\,.
% \end{aligned}
%   \end{equation}
%   Denoting $\tilde q (x) \triangleq \pi_Qp_1(x_i^{(Q)})e^{\alpha_1 + \beta_1^\top \Phi(x_i^{(Q)})} + (1-\pi_Q)p_0(x_i^{(Q)})e^{\alpha_0 + \beta_0^\top \Phi(x_i^{(Q)})}$ we see that maximizing the likelihood loss is equivalent to minimizing the following loss:
   
%   \[
%  \big[  \text{Classification loss with } \{(x_i^{(P)}, y_i^{(P)})\}_{i = 1}^m \big]+ \text{KL} (\hat Q_X || \tilde Q_X ). 
%   \]

Given the source class conditionals $p_j(x)$, the transfer parameters $ \{(\beta_j, \pi_j)\}_{j = 1}^K$ and the tilt transformation $T$ the likelihood for the target data $\{x_i\}_{i = m+1 }^{m + n}$ is 
\begin{equation}
    \label{eq:likelihood-target}
    \cL\Big((\beta_j, \pi_j)\big\vert x_i; ~ i = m+1, \dots, m+n \Big) = \prod_{i = m+1}^{m+n} \Bigg\{\sum_{j = 1}^K  \frac{\pi_j} {\alpha_j}  p_j(x_i) e^{\beta_j ^\top T(x)} \Bigg\}
\end{equation} where $\alpha_j = \int p_j(x_i) e^{\beta_j ^\top T(x)}$. The unknown $p_j$'s are replaced by estimates $\hat p_j$'s obtained from the source data and the likelihood is maximized to estimate the transfer parameters. 

\begin{equation}
    \label{eq:mle}
  \{(\hat \beta_j, \hat \pi_j)\}_{j = 1}^K  = \underset{\{(\beta_j, \pi_j)\}_{j = 1}^K}{\argmin} - \sum_{i = m+1}^{m+n}\log \Bigg\{\sum_{j = 1}^K  \frac{\pi_j} {\hat \alpha_j}  \hat p_j(x_i) e^{\beta_j ^\top T(x)} \Bigg\},
\end{equation} where $\hat \alpha_j = \int \hat p_j(x_i) e^{\beta_j ^\top T(x)}$.


\subsection{Self-training approach}
The self-training approach minimizes the average entropy to estimate the tilt parameters. We notice that the exponentially tilted model implies the log odds difference between source and target is a linear function of $T(x)$: \begin{equation}
\begin{aligned}
&\textsc{logit}_j^{(Q)}(x) - \textsc{logit}_k^{(Q)}(x)\\  &=\log\Bigg(\frac{ \pi_j^{(Q)} q_j(x) }{ \pi_k^{(Q)} q_k(x) }\Bigg)\\
 &= \log\Bigg(\frac{\pi_j^{(P)} p_j(x)}{\pi_k^{(P)} p_k(x)}\Bigg) + (\beta_j - \beta_k)^\top T(x) - (\alpha_j - \alpha_k)\\ & ~~~~ + \log \Bigg(\frac{ \pi_j^{(Q)}  }{ \pi_k^{(Q)}}\Bigg)- \log \Bigg(\frac{ \pi_j^{(P)}  }{ \pi_k^{(P)}}\Bigg)\\
 & = \big\{\textsc{logit}_j^{(P)}(x) + \beta_j^\top T(x) + \gamma_j\big\}  -\big\{ \textsc{logit}_k^{(P)}(x) + \beta_k^\top T(x) + \gamma_k\big\}
\end{aligned}
   \end{equation} But the above may not imply \begin{equation}
        \textsc{logit}_j^{(Q)}(x)  =   \textsc{logit}_j^{(P)}(x) + \beta_j^\top T(x) + \gamma_j\,.
   \end{equation} So, we consider a modification of logits which satisfies  the restriction that \begin{equation}
       \sum_j \textsc{logit}_j^{(P)}(x) = 0, ~~~ \text{ for all}~~ x\,,
   \end{equation} which is satisfied by the unique modification that 
   \begin{equation}
       \textsc{c-logit}_j^{(P)}(x) \gets \textsc{logit}_j^{(P)}(x) - \frac{1}{K}\sum_k \textsc{logit}_k^{(P)}(x)
   \end{equation} and the followings are satisfied. \begin{equation}\begin{aligned}
   \textsc{c-logit}_j^{(Q)}(x)  =   \textsc{c-logit}_j^{(P)}(x) + \big\{\beta_j - \frac1 K \sum_k \beta_k \big\}^\top T(x) + \big\{\gamma_j - \frac1K \sum_K \gamma_K\big\},\\
   q(y = j|x; \beta_k, \gamma_k; k \in 1, \dots, K) = \frac{e^{\textsc{c-logit}_j^{(Q)}(x)}}{\sum_k e^{\textsc{c-logit}_k^{(Q)}(x)}}.
   \end{aligned}
      \end{equation} 
Finally, denoting $\beta \equiv (\beta_1, \dots, \beta_K)^\top\in \reals^{K \times \text{dim}(T(x))}$ and $\gamma = (\gamma_1, \dots,\gamma_K)^\top \in \reals^K$ the  parameters are estimated by minimizing the loss
\begin{equation}
   (\hat \beta, \hat \gamma) \equiv \underset{\beta^\top 1_K = 0, \gamma^\top 1_K = 0}{\mathrm{argmin}} \bbE_{\widehat Q_X}\Big[ -\sum_{j= 1}^K q(y = j | x; \beta, \gamma) \log \{q(y = j | x; \beta, \gamma)\}\Big]
\end{equation} and the final classifier is obtained as \begin{equation}
  \hat y(x) \equiv  \argmax_{j} \{\textsc{c-logit}_j^{(Q)}(x)  =   \textsc{c-logit}_j^{(P)}(x) + \hat \beta_j^\top T(x) + \hat \gamma_j\}
\end{equation}
\textcolor{blue}{Write down the LDA proof of self-training}

\begin{theorem}
Self-training for balanced-LDA works. 
\end{theorem}

\begin{proof}
For a classifier $\sigma(x^\top w)$ the self-training loss function is 
\begin{equation}
    L(w) = E_{Q_X}\big[ - \sigma(x^\top w) \log \big( \sigma(x^\top w) \big) - \big(1 - \sigma(x^\top w )\big) \log \big( 1- \sigma(x^\top w)  \big)\big]
     \end{equation}
Assuming the data is being generated from the LDA model, \ie,  $Q_X \sim \frac 12 N(\mu, I) + \frac12 N(-\mu, I)$ we show that \begin{equation}
    \Bigg(I - \frac{\mu \mu^\top }{\|\mu\|_2^2}\Bigg) \nabla_{w} L(\mu) = 0
\end{equation} We start by noticing that 
\[
\begin{aligned}
\nabla_{w} L(w) & = E_{Q_X}\Bigg[ - \log \bigg(\frac{\sigma(x^\top w)}{1- \sigma(x^\top w)} \bigg) \sigma(x^\top w) \big(1- \sigma(x^\top w)\big) x\Bigg]\\
&= E_{Q_X}\Bigg[ -  \sigma(x^\top w) \big(1- \sigma(x^\top w)\big) xx^\top \Bigg]w\,,
\end{aligned}
\] and 
\[
E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) xx^\top \Bigg]\mu = E_{N(-\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) xx^\top \Bigg]\mu\,.
\] This implies 
\[
\nabla_w L(\mu) = E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) xx^\top \Bigg]\mu
\] 
Denoting $P_{\mu}^\perp = I - \frac{\mu \mu^\top }{\|\mu\|_2^2}$ we notice that for a random variable $x \sim N(\mu, I)$ the following holds: (1) $P_\mu ^\perp x \perp \!\!\! \perp \mu^\top x$ and (2) $E\big[P_{\mu}^\perp x\big] = 0$. This two facts imply
\[
\begin{aligned}
\Bigg(I - \frac{\mu \mu^\top }{\|\mu\|_2^2}\Bigg) \nabla_{w} L(\mu) &= E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) P_\mu^\perp x x^\top\mu \Bigg] \\
&= E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) x^\top\mu \Bigg] E_{N(\mu, I)}\Big[  P_\mu^\perp x  \Big]
& = 0\,.
\end{aligned}
\]
The fact that $P_\mu \perp \nabla_{w} L(\mu) = 0 $ implies $\nabla_{w} L(\mu) = c\mu$ for some $c\in \reals$. Again 
\[
\begin{aligned}
\nabla_{w} L(\mu) &= E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) P_\mu^\perp x x^\top\mu \Bigg]\\
& ~~~+ E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) \frac{\mu \mu^\top}{\|\mu\|_2^2} x x^\top\mu \Bigg] \\
& = E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big)   (x^\top\mu)^2 \Bigg]\frac{\mu }{\|\mu\|_2^2} \\
& = -\lambda \mu\,,
\end{aligned}
\] where $\lambda>0$. The fact that  $\nabla_{w} L(w) + \lambda w$ is gradient of the regularized loss $L(w) + \frac{\lambda}{2}\|w\|_2^2$ and  $\nabla_{w} L(\mu) + \lambda \mu = 0$ implies $\mu$ is the unique minimizer in an $\ell_2$-ball. For a different $\lambda$ we can replace $\mu$ by $\delta \mu$ for some $\delta>0$ resulting 
\[
\begin{aligned}
\nabla_{w} L(\delta\mu) &= E_{N(\mu, I)}\Bigg[ -  \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)   \delta ^2 (x^\top\mu)^2 \Bigg]\frac{\delta \mu }{\delta^2 \|\mu\|_2^2}\\
& = E_{N(\mu, I)}\Bigg[ -  \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)    (x^\top\mu)^2 \Bigg]\frac{\delta \mu }{ \|\mu\|_2^2}
\end{aligned}
\] where $\delta$ is adjusted accordingly to get $\lambda = \frac{1}{ \|\mu\|_2^2} E_{N(\mu, I)}\Bigg[   \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)    (x^\top\mu)^2 \Bigg]$. Since, 
\[
\begin{aligned}
& \frac{1}{ \|\mu\|_2^2} E_{N(\mu, I)}\Bigg[   \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)    (x^\top\mu)^2 \Bigg]\\
& = E_{N(1, 1)}\Big[   \sigma(\delta' g) \big(1- \sigma(\delta' g )\big)    g^2 \Big], ~~ \delta' \triangleq \delta \|\mu\|_2 \\
& \le \frac 14 E_{N(1, 1)}\big[       g^2 \big] = \frac 12\,.
\end{aligned}
\] So, we have to set $\lambda < \frac 12$. 
\end{proof}

==> exponential-tilt(ICLR2023)/sections/exp-tilt.tex <==
\section{Transfer through exponential tilting}

We consider a problem of domain adaptation in binary classification setup. Let $\cX\subset  \reals^f$ be the space of feature vectors. We assume that the source and target populations are distributed as $P$ and $Q$ respectively, where $P$ and $Q$ are probability distributions on the space $\cX\times \{0, 1\}$.  Assume that we have $m$ many \IID\ labeled observations  $\{(x_i, y_i)\}_{i=1}^m  $ from $P$ and  $n$ \IID\ unlabeled observations $ \{x_i\}_{i = m+1}^{m +n} $ from the target distribution $Q$. Denoting $D = \{(x_i, y_i)\}_{i=1}^m  \cup \{x_i\}_{i = m+1}^{m +n} $ as the full dataset we see that $D \sim P^{\otimes m} \otimes Q_X^{\otimes n}$ where $Q_X$ is the marginal of $x$ under $Q$ distribution.   The task at hand is to construct a classifier for the target population. 


We restrict ourselves to the setup of exponentially tilted transfers. We assume that the class conditional distributions for $P$ and $Q$ are continuous with densities $p_0$, $p_1$ and $q_0$, $q_1$, respectively. Furthermore, we assume that the class conditional densities for target are exponential tilts to the corresponding class conditional densities for source. More specifically, given a transformation $\Phi(x)\in \reals^d$ and some $\beta_0, \beta_1 \in \reals^d$ we have the followings: 
\begin{equation}
    \label{eq:exponential-tilt}
\text{For } y \in \{0, 1\}  ~~~~~   q_y(x) = p_y(x) e^{\alpha_y + \beta_y ^\top \Phi(x)} \text{  where  }  \alpha_y = - \log \left(\int p_y(x) e^{ \beta_y ^\top \Phi(x)} dx \right).
\end{equation}
 In the above tilt the constant $\alpha_y$ is set  to make $q_y$ a valid density, \ie, $\int q_y(x)dx = 1$. 
 
 This type of exponential tilting has a natural connection to the linearly adjusted posterior drift model \cite{maity2021linear} though logistic link function. Denoting $\gamma$ as the logistic link ($\gamma(x) = \log\{x/(1-x)\}$) and $\pi_Q$ and $\pi_P$ as the proportion of having $y = 1$ in the $P$  and $Q$ distribution, respectively,  we notice that \eqref{eq:exponential-tilt} implies 
 \begin{equation}
 \label{eq:target-classifier}
     \begin{aligned}
 \gamma(Q(y = 1| x)) &= \log\left(\frac{q_1(x)}{q_0(x)}\right) + \gamma(\pi_Q)\\
 & = \log\left(\frac{p_1(x)}{p_0(x)}\right) + (\alpha_1 - \alpha_0) + (\beta_1 - \beta_0)^\top \Phi(x) + \gamma(\pi_Q)\\
 & = \gamma(P(y = 1| x)) - \gamma(\pi_P) + (\alpha_1 - \alpha_0) + (\beta_1 - \beta_0)^\top \Phi(x) + \gamma(\pi_Q)\,. 
 \end{aligned}
 \end{equation}
  The calculation in the above display implies that after a logistic transformation, the regression function (conditional probability of having $y = 1$ given that we observe the feature value $x$) for target distribution is just a linear shift of the source regression function. This is the exact modelling assumption in linearly adjusted posterior drift setup when the link function is logistic link \citep[see][Equation (1.1)]{maity2021linear}.
  
  Unlike [1], this paper deals with the more challenging setting 
 
 
\subsection{Identifiability of exponential tilting}
Recalling the calculations in display \eqref{eq:target-classifier} we see that  construction of the target classifier requires us to estimate the the following quantities: $P(y = 1| x)$,  $\pi_P$,  $\alpha_1 - \alpha_0$, $\beta_1 - \beta_0$ and $ \pi_Q.$ Given the labeled source data one can estimate  $P(y = 1| x)$ and $\pi_P$. So the question remains \emph{how do we estimate $\alpha_1 - \alpha_0$, $\beta_1 - \beta_0$ and $ \pi_Q$}? A first step toward estimating of these quantities is unique identification of them. We see that from the labeled data from source one can potentially  estimate the $P$ distribution, but in absence of the target labels the best one can do is to estimate $q_X$. Furthermore, these are the maximal information one can hope to estimate from the data at hand, meaning without additional information on $P$ and $Q_X$ the data $D$ is a \emph{minimal sufficient statistics} for them.   Hence, we ask the following question. 
\begin{quote}
   \textbf{Question}: Given the distributions $P$ and $q_X$ when are the quantities $\alpha_1 - \alpha_0$, $\beta_1 - \beta_0$ and $ \pi_Q$ uniquely identifiable? 
\end{quote}
The rest of this subsection is dedicated to answering this question. We start with noticing that under \eqref{eq:exponential-tilt} the marginal density $q_X$ can be written as 
\begin{equation}
\label{eq:rep1}
  q_X(x) = (1-\pi_Q) p_0(x) e^{\alpha_0 +\beta_0 ^\top \Phi(x)}   + \pi_Q p_1(x) e^{\alpha_1 +\beta_1 ^\top \Phi(x)}\,. 
\end{equation} and by absorbing $\pi_Q$ in $\alpha_1$ and $1-\pi_Q$ in $\alpha_0$ we have 
\begin{equation}
\label{eq:rep2}
    q_X(x) = p_0(x) e^{a_0 +\beta_0 ^\top \Phi(x)}   +  p_1(x) e^{a_1 +\beta_1 ^\top \Phi(x)}\,,
\end{equation} for some $a_0, a_1 \in \reals$. With this two representations one might ask whether these two representations are equivalent, in the sense that is it possible to recover one representation from another.  The following lemma establish that. 
\begin{lemma}
\label{lemma:eqiv-rep}
We have the equivalence between the representations \eqref{eq:rep1} and \eqref{eq:rep2}, \ie, \begin{enumerate}
    \item \eqref{eq:rep1} implies \eqref{eq:rep2} with $a_1 = \alpha_1 + \log(\pi_Q)$ and $a_0 = \alpha_0 + \log(1-\pi_Q)$, and 
    \item \eqref{eq:rep2} implies \eqref{eq:rep1} with $\alpha_y = - \log \left(\int p_y(x) e^{ \beta_y ^\top \Phi(x)} dx \right)$ for $y = 0$ and $1$ and $\pi_Q = e^{a_1 - \alpha_1} = 1 - e^{a_0 - \alpha_0}$. 
\end{enumerate}
\end{lemma}
We stick to the representation in \eqref{eq:rep2} and from the transformed target regression function in display \eqref{eq:target-classifier} we only need to identify $a_1 - a_0 = \alpha_1 - \alpha_0 + \log(\pi_Q) - \log(1 - \pi_Q)$ and $\beta_1 - \beta_0$.  Next  we consider  a condition on the density ratio $\frac{p_1(x)}{p_0(x)}$
with is  necessary and sufficient for unique identification of the parameters $a_0$, $a_1$, $\beta_0$ and $\beta_1$. Later we establish that this condition is also necessary and sufficient for unique identification of $a_1 - a_0 $ and $\beta_1 - \beta_0$. We start with the required conditions, where we assume: 

\begin{assumption}
\label{assmp:range}
    For every $v, w \in \reals^d$ and $M>0$ there exists $x_1, x_2 \in \cX$ such that the followings hold: (1) $\|\Phi(x_1)\|_2 \le \frac1 M \le M \le \|\Phi(x_2)\|_2$, and (2) $v^\top \Phi(x_1) w^\top \Phi(x_1) < 0$ and $v^\top \Phi(x_2) w^\top \Phi(x_2) < 0$. 
\end{assumption}

\begin{assumption}
    \label{assmp:non-linear}
    For any $\theta_0,  \delta_0\in \reals$, $\alpha>0$ and $\theta,  \delta \in\reals^d$   we have an $x$ such that 
    \[p_1(x) e^{\theta_0 + \theta^\top \Phi(x)}\left(e^{\delta_0 + \delta^\top \Phi(x)} - 1\right) \neq  p_0(x) \left(e^{\alpha\delta_0 + \alpha\delta^\top \Phi(x)} - 1\right)\,. \]
    \end{assumption}
    Next we show that this condition is necessary and sufficient for uniquely identifying the parameters $a_0$, $a_1$, $\beta_0$ and $\beta_1$.
    
    
   \begin{lemma}
   
   Assume that a solution of the  equation \eqref{eq:rep2} exists and the range of $\Phi(x)$ satisfies the assumption \ref{assmp:range}.  The solution is unique if and only if the assumption \ref{assmp:non-linear} holds. \label{lemma:uniqueness}
   \end{lemma}
   
   The above Lemma asserts that we have a unique target regression function.
   \[
   \eta_Q(x) = \frac{p_1(x) e^{a_1 + \beta_1^\top \Phi(x)}}{p_1(x) e^{a_1 + \beta_1^\top \Phi(x)} + p_0(x) e^{a_0 + \beta_0^\top \Phi(x)}}\,.
   \]
   But we note that to have a unique target regression function we only need $a_1 - a_0$ and $\beta_1 - \beta_0$ to be uniquely identified. In the next lemma we establish these two requirements are equivalent. 
   
   \begin{lemma}
   \label{lemma:unique-reg-fn}
   Assume that a solution of the  equation \eqref{eq:rep2} exists and the range of $\Phi(x)$ satisfies the assumption \ref{assmp:range}. The quantities $a_1 - a_0$ and $\beta_1 - \beta_0$ are unique if and only if the solution of the  equation \eqref{eq:rep2} is unique. 
   \end{lemma}

\subsection{The case of LDA model}
Here, we consider the case of linear discrimination (LDA) model where the decision boundary is linear. For $j \in \{0, 1\}$ let us assume that $p_j(x) \equiv N(\mu_j^{(P)}, \Sigma)$ and $q_j(x) \equiv N(\mu_j^{(Q)}, \Sigma)$, where $\mu_j^{(P)}, \mu_j^{(Q)} \in \reals^d$ and $\Sigma\in \reals^{d \times d }$ is a positive definite matrix. Noticing that $\log(q_j/p_j) = x^\top \Sigma^{-1} (\mu_j^{(Q)} - \mu_j^{(P)}) + \alpha_j, ~ \alpha_j \in \reals$ the minimal requirement of a linear transformation $\Phi$ is that $\text{Row-space}(\Phi) \supseteq \text{Span}(\Sigma^{-1} (\mu_0^{(Q)} - \mu_0^{(P)}), \Sigma^{-1} (\mu_1^{(Q)} - \mu_1^{(P)}))$. Furthermore,  the fact that $ \log  (p_1/p_0) = x^\top \Sigma^{-1} (\mu_0^{(P)} - \mu_1^{(P)}) + C$ implies $\Sigma^{-1} (\mu_0^{(P)} - \mu_1^{(P)}) \notin \text{Row-space}(\Phi)$. These are necessary and sufficient conditions for the assumption \ref{assmp:non-linear} to be satisfied.  

\subsection{The cases of non-identifiability}

One of the cases that is excluded by the condition \ref{assmp:non-linear} is linear decision boundary (with respect to $\Phi(x)$) for $P$. This is a very popular modeling assumption for the classification task and perhaps the most well-known example of such linear decision boundary is the linear discrimination model, \ie, the class conditionals for source are distributed as normal with different means and the same variance. Given a $P$ it is possible to figure out the means and the commons variance and hence the class conditionals. The exponential tilting model \eqref{eq:exponential-tilt} implies that the target distribution also satisfies the linear discrimination model with the same common variance as the source. But the exponential tilting \ref{eq:exponential-tilt} has the flexibility of covering all the linear discrimination models with a specific variance. With the only available knowledge of $q_X$ from the target, the best possible task one can hope to do is clustering on $q_X$.   With the clustering task in mind, it is possible to identify and estimate these cluster densities for the target, which are the target class conditional densities up to a permutation.  But identifying and estimating the cluster densities is only a part of the task toward building a target classifier, one also needs to know which cluster corresponds to which class, and figuring out this correspondence is not possible without the target labels. So, building a target classifier for this specific case of linear discrimination with exponential tilting requires target labels.  

We end this subsection with an example of linear discrimination model which falls under the condition \ref{eq:exponential-tilt} and hence can be tackled even in absence of the target labels. We assume that the feature $\Phi(x)$ has two independent components, \ie, $\Phi(x) = (\Phi_1(x)^\top, \Phi_2(x)^\top)^\top, ~~ \Phi_1(x)\in \reals^{d_1},  \Phi_2(x) \in  \reals^{d_2}, $ and there does not exists a matrix $A\in \reals^{d_2 \times d_1}$ such that  $\Phi_2(x) = A \Phi_1(x) $ for all $x$. We also assume that  the exponential tilting condition \eqref{eq:exponential-tilt} is satisfied with $\Phi_1(x)$ and that  the source decision boundary is linear in terms of $\Phi(x)$ with a non-trivial component for $\Phi_2(x)$, \ie, there exists $\beta_0\in \reals, \beta_1 \in \reals^{d_1}$ and $\beta_2 \in \reals^{d_2}$ such that
\begin{equation}
    \log\left(\frac{p_1(x)}{p_0(x)}\right) = \beta_0 + \beta_1 ^\top \Phi_1(x) + \beta_2 ^\top \Phi_2(x), ~~~~ \beta_2 \neq 0\,.
\end{equation} Then the condition \ref{assmp:non-linear} is satisfied except some special cases when for some $\delta_0, \theta_0 \in \reals$, $\alpha>0$ and $\theta_1, \beta_1 \in \reals^{d_1}$ and any $x$ we have
\[
\beta_2^\top \Phi_2(x) = \theta_0 + \theta_1 ^\top \Phi_1(x) +  \log\left(\frac{e^{\alpha\delta_0 + \alpha\delta_1^\top \Phi_1(x)} - 1}{e^{\delta_0 + \delta_1^\top \Phi_1(x)} - 1}\right)\,.
\]


\subsection{The case of exponential family distributions} 

% In this subsection we provide an interpretation for the condition \ref{assmp:non-linear} when the class conditional distributions in source and target are from exponential family of distributions. With the definition $\cE(T) = \{p_\beta(x) = \exp(\beta^\top T(x)- \beta_0): \beta_0 = \int \exp(\beta^\top T(x)), ~\beta \in \reals^d\}$ where $T: \cX \to \reals^d$ is a feature map, we assume that $p_j(x) \in \cE(T_j^{(P)})$ and $ q_j(x)\in \cE(T_j^{(Q)})$ for $ j = 0, 1. $ Let $A(x)$ is the transformation used in exponentially tilted adaptation. Then the following conditions are necessary. The condition that 
% \begin{equation}
%     \text{Span} \Big\{ (\beta_j^{(Q)})^\top T_j^{(Q)}(x) - (\beta_j^{(P)})^\top T_j^{(P)}(x);~ j = 0, 1 \Big\} \subseteq \text{Span}\big\{A(x)\big\}
% \end{equation} ensures that $A(x)$ is enough for for adaptation. Furthermore, the condition that 
% \begin{equation}
%     (\beta_1^{(P)})^\top T_1^{(P)}(x) - (\beta_0^{(P)})^\top T_0^{(P)}(x) \notin \text{Span}\big\{A(x)\big\}
% \end{equation} is required to maintain identifiability of the transfer.   


In this subsection, we assume that the source and target class conditionals are from the exponential family. With statistic $T(x) \in \reals^d$ the exponential family of distributions has the following collection of  distributions: 
\begin{equation}
    p_\beta(x) = \frac 1 {\beta_0}\exp(\beta^\top T(x)); ~~ \beta_0 = \int \exp(\beta^\top T(x)), ~\beta \in \reals^d\,.
\end{equation} For national simplicity we let $T(x) = x$ from hereon. The following theorem provides identification for the multi-class transfer. 
\begin{theorem}
\label{th:multi-class-exponential}
Suppose $p_j(x), ~ q_j(x); ~ j = 1, 2, \dots, K$ are exponential family distributions with statistic $x$ and the following are satisfied. 
\begin{enumerate}
    \item $\text{span}  \Big\{ \log\big(\frac{q_j(x)}{p_j(x)}\big); ~ j = 1, \dots, K  \Big\} \subseteq \text{span} \big\{T(x), 1\big\}$.
    \item There does not exist a pair $(j, k)$, a vector $u \in \reals^{|T(x)|}$, and a scalar $v\in \reals$ such that $\frac{p_j(x)}{p_k(x)} = e^{u^\top T(x) + v}$. 
\end{enumerate} Then there exists a unique solution to the equation 
\begin{equation}
\label{eq:target-marginal-multi}
    \sum_{j = 1}^K p_j(x) \alpha_j e^{\beta_j^\top T(x) 
    } = q_X(x)\,,
\end{equation} such that $\alpha_j \ge 0$. The conditions are also necessary for existence of unique solution. 
\end{theorem}

\begin{corollary}[LDA with linear transformation]
Suppose the class conditionals satisfies LDA model for source and target distribution with same covariance matrix. More specifically, we assume  $p_j(x) \sim N(\mu_j, \Sigma)$ and $q_j(x) \sim N(\xi_j, \Sigma)$ for some $\{\mu_j, \xi_j\}_{j = 1}^K \subseteq \reals^d$ and $\Sigma \in \reals^{d \times d}$. Furthermore, we also assume the transformation $T(x)$ is linear. Then the conditions in the Theorem \ref{th:multi-class-exponential} simplifies to the following ones. 
\begin{enumerate}
    \item $\text{span}  \Big\{ \Sigma^{-1}(\xi_j - \mu_j); ~ j = 1, \dots, K  \Big\} \subseteq \text{row-space} \big\{T\big\}$.
    \item There does not exist  $1 \le j \neq k \le K$ such that $\Sigma^{-1}(\mu_j - \mu_k) \notin \text{row-space} \big\{T\big\}$, or equivalently, the projection of the vectors $\big\{\Sigma^{-1}\mu_j\big\}_{j = 1}^K$ in the orthogonal space to $\text{row-space} \big\{T\big\}$ are distinct. 
\end{enumerate} The first condition ensures that the transformation $T$ is sufficient for transferring source class conditional densities to target ones  by the exponential tilt adjustment. The second condition is important for the unique identification, which ensures that after the transformation $T'$ which is orthogonal to $T$ (\ie, each row of $T'$ is orthogonal to each row of $T$) the class conditional distributions in the source are distinct. Furthermore, condition 1. that distribution of $T'(x)|y = j$ is the same between source and target. So the feature $T'(x)$ can be viewed as an invariant one across source and target. 

If some the feature co-ordinates has same class conditional distributions across source and target populations, along with some discriminating power for the labels (\eg, $P(x_1|y = j) = Q(x_1 | y = j)$ and $P(x_1 | y = j)$'s are different) then one can set $T$ to be the transformations in the remaining co-ordinates (in previous example $T$ is the matrix obtained after deleting the first row of identity matrix). One may think that since the invariant coordinates have some discriminating power for labels, they can be used to build a classifier which would also work for the target distribution. The exponential tilt correction can recover the target Bayes classifier and result in a better predictive accuracy. 
\end{corollary}

==> exponential-tilt(ICLR2023)/sections/exp.tex <==
\section{\waterbirds\ case study}
\label{sec:waterbird}
To demonstrate the efficacy of the ExTRA algorithm for reweighing the source data we (i) verify the ability of ExTRA to upweigh samples most relevant to the target task; (ii) evaluate the utility of weights in downstream tasks such as fine-tuning and (iii) model selection.





\textbf{\waterbirds\ dataset} combines bird photographs from the Caltech-UCSD Birds-200-2011 (CUB) dataset \citep{wah2011caltech} and the image backgrounds from the Places dataset \citep{zhou2017places}. The birds are labeled  as one of
$\cY =$ \{waterbird, landbird\} and placed on one of $\cA =$ \{water background, land background\}.
% with
% waterbirds  more frequently appearing against a water  background and landbirds more frequently appearing on land.
The images are divided into four groups: landbirds on land (0); landbirds on water (1); waterbirds on land (2); waterbirds on water (3). The source dataset is highly imbalanced, i.e. the smallest group (2) has 56 samples. We embed all images with a pre-trained ResNet18 \citep{he2016Deep}. See Appendix
\ref{sup:exp:data}
for details.




We consider five subpopulation shift target domains: all pairs of domains with different bird types and the original test set \citep{sagawa2019Distributionally} where all 4 groups are present with proportions vastly different from the source.
% We learn importance weights with ExTRA by (1) maximizing the objective in Lemma  \eqref{lemma:KL-distribution-matching} to estimate the tilt parameters, (2) obtaining importance weight estimates as in \eqref{eq:weights-estimate}.
For all domains, we fit ExTRA weights (with ResNet18 features as $T(x)$) from 10 different initializations and report means and standard deviations for the metrics. See Appendix \ref{sup:exp:model}
for the implementation details.






\textbf{ExTRA weights quality} For a given target domain it is most valuable to upweigh the samples in the source data corresponding to the groups comprising that domain. The most challenging is the target $\{1,2\}$ consisting only of birds appearing on their atypical backgrounds. Groups $\{1,2\}$ correspond to 5\% of the source data making them most difficult to ``find''. To quantify the ability of ExTRA to upweigh these samples we report precision (proportion of samples from groups $\{1,2\}$ within the top $x\%$ of the weights) and recall (proportion of $\{1,2\}$ samples within the top $x\%$ of the weights) in Figure \ref{fig:precision-recall}. We notice that samples corresponding to $10\%$ largest ExTRA weights contain slightly over $80\%$ of the groups $\{1,2\}$ in the source data (recall). This demonstrates the ability of ExTRA to upweigh relevant samples. We present examples of upweighted images and results for other target domains in Appendix
\ref{sup:exp:results}.

\begin{wrapfigure}[13]{r}{0.4\linewidth}
% \vspace{-0.7cm}
\vspace{-0.45cm}
\centering
\includegraphics[width=\linewidth]{plots/precision-recall.pdf}
\vspace{-.7cm}
\caption{ExTRA precision and recall for samples with top $x\%$ weights.}
\label{fig:precision-recall}
\end{wrapfigure}







\textbf{Model fine-tuning}
We demonstrate the utility of ExTRA weights in the fine-tuning  \eqref{eq:weighted-ERM}. The basic goal of such importance weighing is to improve the performance in the target in comparison to training on uniform source weights S -> T, \ie\  ERM. Another baseline is the DRO model \citep{hashimoto2018Fairness} that aims to maximize worst-group performance without access to the group labels, and JTT \citep{liu2021Just} that retrains a model after upweighting the misclassified samples by ERM. We consider two additional baselines that utilize group annotations to improve worst-group performance: re-weighing the source to equalize group proportions (RW$_\text{gr}$) and group DRO (gDRO) \citep{sagawa2019Distributionally}. The aforementioned baselines do not try to adjust to the target domain. Finally, we compare to $\pi$T -> T that fine-tunes the model only using the subset of the source samples corresponding to the target domain groups. In all cases we use logistic regression as model class.


\begin{wrapfigure}[14]{r}{0.45\linewidth}
\vspace{-0.2in}
    \centering
    \includegraphics[width=\linewidth]{plots/waterbirds.pdf}
    \vspace{-0.25in}
    \caption{Performance on \waterbirds.}
    \label{fig:waterbirds}
    % \vspace{-0.3in}
\end{wrapfigure}


We compare target accuracy across domains in Figure \ref{fig:waterbirds}. Analogous comparison with area under the receiver operator curve can be found in Figure \ref{fig:waterbird-auc} in Appendix \ref{sup:exp:waterbirds}. Model trained with ExTRA weights outperforms all ``fair'' baselines and matches the performance of the three baselines that had access to additional information. In all target domains ExTRA fine-tuning is comparable with the $\pi$T -> T supporting its ability to upweigh relevant samples. Notably, on \{1,2\} domain of both minority groups \emph{and} on \{0,3\} domain of both majority groups, ExTRA outperforms RW$_\text{gr}$ and gDRO that utilize group annotations. This emphasizes the advantage of adapting to the target domain instead of pursuing a more conservative goal of worst-group performance maximization. Finally, we note that ExTRA fine-tuning did not perform as well on the domain \{1,3\}, however neither did $\pi$T -> T.
% (although comparable to T -> T). The label distribution in this domain ($\Pr$(waterbird)=\my{XXX}) drastically differs from the source ($\Pr$(waterbird)=\my{XXX}) causing optimization instabilities in solving \eqref{eq:KL-distribution-matching} and resulting in larger standard deviation.






\begin{table}[]
\caption{Model selection results on \waterbirds}
    \centering





{\small
\begin{tabular}{l@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc}
\toprule
{} & \multicolumn{3}{c}{target accuracy} & \multicolumn{3}{c}{rank correlation} \\
\cmidrule[1pt](lr){2-7}
target groups &            ExTRA & SrcVal & ATC-NE &            ExTRA & SrcVal & ATC-NE \\
\midrule
\{0, 2\}       &  0.819$\pm$0.012 &  0.854 &  \textbf{0.871} &   0.419$\pm$0.01 &  \textbf{0.807} &  0.760 \\
\{1, 2\}       &  \textbf{0.741}$\pm$0.047 &  0.616 &  0.646 &  \textbf{0.747}$\pm$0.106 & -0.519 & -0.590 \\
\{0, 3\}       &  \textbf{0.978}$\pm$0.001 &  \textbf{0.978} &  0.976 &  \textbf{0.962}$\pm$0.004 &  0.956 &  0.906 \\
\{1, 3\}       &  \textbf{0.757}$\pm$0.011 &  0.737 &  0.747 &  \textbf{0.361}$\pm$0.168 & -0.318 & -0.411 \\
\{0, 1, 2, 3\} &  \textbf{0.856}$\pm$0.034 &  0.803 &  0.818 &  \textbf{0.658}$\pm$0.295 &  0.263 &  0.178 \\
\midrule
average      &     \textbf{0.83} &  0.798 &  0.812 &    \textbf{0.753} &  0.166 &  0.110 \\
\bottomrule
\end{tabular}}
   \vspace{-0.4cm}
    \label{tab:waterbirds-model-validation}
\end{table}



\textbf{Model selection} out-of-distribution is an important task, that is difficult to perform without target data labels and group annotations \citep{gulrajani2020Search,zhai2021DORO}. We evaluate the ability of choosing a model for the target domain based on accuracy on the ExTRA reweighted source validation data. We compare to the standard source validation model selection (SrcVal) and to the recently proposed ATC-NE \citep{garg2022leveraging} that uses negative entropy of the predicted probabilities on the target domain to score models. We fit a total of 120 logistic regression models with different weighting (uniform, label balancing, and group balancing) and varying regularizers. See Appendix
\ref{sup:exp:model}
for details.

In Table \ref{tab:waterbirds-model-validation} we compare the target performance of models selected using each of the model evaluation scores and rank correlation between the corresponding model scores and true target accuracies. Model selection with ExTRA results in the best target performance and rank correlation on 4 out of 5 domains and on average. Importantly, the rank correlation between the true performance and ExTRA model scores is always positive, unlike the baselines, suggesting its reliability in providing meaningful information about the target domain performance.




\vspace{-0.3cm}
\section{\breeds\ case study}
% \vspace{-0.2cm}
\label{sec:breeds}
\breeds\ \citep{santurkar2020breeds} is a subpopulation shift benchmark derived from ImageNet \citep{deng2009imagenet}. It uses the class hierarchy to define groups within classes. For example, in the Entity-30 task considered in this experiment, class fruit is represented by strawberry, pineapple, jackfruit, Granny Smith in the source and buckeye, corn, ear, acorn in the target. This is an extreme case of subpopulation shift where source and target groups have zero overlap. We modify the dataset by adding a small fraction $\pi$ of random samples from the target to the source for two reasons: (i) our exponential tilt model requires some amount of overlap between source and target; (ii) arguably, in practice, it is more likely that the source dataset has at least a small representation of all groups.
% We remind that our method does not use the subgroup information.


\begin{wrapfigure}[12]{r}{0.4\linewidth}
    \vspace{-0.4cm}
    \centering
    \includegraphics[width=\linewidth]{plots/breeds.pdf}
    \vspace{-0.6cm}
    \caption{Performance on \breeds.}
    \label{fig:breeds}
\end{wrapfigure}

Our goal is to show that ExTRA can identify the target samples mixed into the source for efficient fine-tuning. We obtain feature representations from a pre-trained self-supervised SwAV \citep{caron2020unsupervised}. To obtain the ExTRA weights we use SwAV features as sufficient statistic.  We then train logistic regression models on (i) the source dataset re-weighted with ExTRA, (ii) uniformly weighted source (S -> T), (iii) target samples mixed into the source ($\pi$T -> T), (iv) all target samples (oracle). See Appendix \ref{sup:exp:data}, \ref{sup:exp:model}
for details. We report performance for varying mixing proportion $\pi$ in Figure \ref{fig:breeds}. First, we note that even when $\pi=0$, i.e. source and target have completely disjoint groups (similar to domain generalization), ExTRA improves over the vanilla S -> T. Next, we see that S -> T improves very slowly in comparison to ExTRA as we increase the mixing proportion; $\pi$T -> T improves faster as we increase the number of target samples it has access to, but never suppresses ExTRA and matches its improvement slope for the larger $\pi$ values. We conclude that ExTRA can effectively identify target samples mixed into source that are crucial for the success of fine-tuning \emph{and} find source samples most relevant to the target task allowing it to outperform $\pi$T -> T. We report analogous precision and recall for the \waterbirds\ experiment in Appendix
\ref{sup:exp:results}.
% \ref{sup:exp:results}.








==> exponential-tilt(ICLR2023)/sections/exponential-tilt.tex <==
\section{Domain adaptation via exponential tilting}


At a high-level, the proposed method for domain adaptation consists of two steps:
\begin{enumerate}
\item \textbf{fit exponential tilt model:} estimate the parameters $\theta_k$'s in the exponential tilt model by matching the tilted (marginal) distribution of the inputs from the source domain with that of the inputs from the target domain;
\item \textbf{train classifier for target domain:} construct/train a classifier for the target domain by plugging in the estimates of $q\{x,Y=k\}$ into \eqref{eq:target-regression-function} or weighted empirical risk minimization (ERM).
\end{enumerate}
We elaborate on the two steps in the rest of this section and summarize the method in algorithm \ref{alg:DAET}.

\paragraph{Fit exponential tilt model} In the first step, we estimate the parameters of the exponential tilt model by distribution matching. This step is based on the observation that under the exponential tilt model \eqref{eq:exponential-tilt}
\begin{equation}
q_X\{x\} = \sum_{k=1}^Kp\{x,Y=k\}w_k\exp(\theta_k^\top T(x) - a_k(\theta_k)),
\label{eq:distribution-matching}
\end{equation}
where $q_X$ is the (marginal) density of the inputs in the source domain. It is possible obtain an estimate $\hq_X$ of $q_X$ from the unlabeled samples $\{X_i\}_{i=n_s+1}^{n_s+n_t}$ and estimates $\hp\{x,Y=k\}$ of the $p\{x,Y=k\}$'s from the labeled samples $\{(X_i,Y_i)\}_{i=1}^{n_s}$. This suggests we find $\theta_k$'s such that  
\[
\sum_{k=1}^K\hp\{x,Y=k\}w_k\exp(\theta_k^\top T(x) - a_k(\theta_k)) \approx \hq_X\{x\}.
\]
A more robust approach is to minimize the discrepancy between the two sides with respect to the $\theta_k$'s:
\begin{equation}
\{\htheta_k\}_{k=1}^K \in \argmin_{\{\theta_k\}_{k=1}^K}D\left(\textstyle\hq_X\{x\}\|\sum_{k=1}^K\hp\{x,Y=k\}w_k\exp(\theta_k^\top T(x) - a_k(\theta_k))\right),
\label{eq:robust-distribution-matching}
\end{equation}
where $D$ is a discrepancy between probability distributions on $\cX$. For example if $D$ is the Kulback-Leibler (KL) divergence, then \eqref{eq:robust-distribution-matching} is
\begin{equation}
\begin{aligned}
\{\htheta_k\}_{k=1}^K &\in \argmin_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\hq_X\{X\} - \log\left(\sum_{k=1}^K\hp\{X,Y=k\}\exp(\theta_k^\top T(X) - a_k(\theta_k))\right)\right] \\
% &=\argmin_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\hq_X\{X\} - \log\hp_X\{X\} - \log\left(\sum_{k=1}^K\big[\heta_P(X)\big]_k\exp(\theta_k^\top T(X))\right)\right] \\
&\equiv\argmax_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\left(\sum_{k=1}^K\big[\heta_P(X)\big]_k\exp(\theta_k^\top T(X) - a_k(\theta_k))\right)\right],
\end{aligned}
\label{eq:KL-distribution-matching}
\end{equation}
where $\hQ_X$ is the empirical distribution of the (unlabeled) samples from the target domain and $\heta_P:\cX\to\Delta^{K-1}$ is an estimate of the regression function in the source domain:
\[
\big[\eta_P(x)\big]_k \triangleq P\{Y=k\mid X=x\}.
\]
One benefit of minimizing the KL divergence is the learner does not need to estimate the $p\{x,Y=k\}$'s; they merely need to train a discriminative model to estimate $\eta_P$ from the (labeled) samples from the source domain. In other words, the learner does not needs to train generative models. 

% \YK{Subha's convex method here}

We note that the consistency of \eqref{eq:robust-distribution-matching} depends on the identifiability of the $\theta_k$'s from  \eqref{eq:distribution-matching}; \ie\ the uniqueness of the $\theta_k$'s that satisfy \eqref{eq:distribution-matching}. As long as the $\theta_k$'s are identifiable, then \eqref{eq:robust-distribution-matching} provides consistent estimates of the $\theta_k$'s. Unfortunately, without additional assumptions on the $p\{x,Y=k\}$'s and $T$, the $\theta_k$'s are generally unidentifiable from \eqref{eq:distribution-matching} (see section \ref{sec:identifiability} for an example). We elaborate on the identifiability of the exponential tilt model in section \ref{sec:identifiability}.

\paragraph{Train classifier for target domain} Armed with estimates $\htheta_k$'s of the $\theta_k$'s, we train a classifier for the target domain by weighted ERM in the second step:
\begin{equation}
\heta_Q\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\exp(\htheta_Y^\top T(X))\right],
\label{eq:weighted-ERM}
\end{equation}
where $\ell$ is a loss function. The weight function in \eqref{eq:weighted-ERM} is chosen so that expected value of the cost function in \eqref{eq:weighted-ERM} is exactly the risk in the target domain:
\[
\begin{aligned}
\Ex_P\left[\ell(f(X),Y)\exp(\theta_Y^\top T(X))\right] &= \sum_{k=1}^K\Ex_P\left[\ell(f(X),k)\exp(\theta_k^\top T(X))\ones\{Y=k\}\right] \\
&= \sum_{k=1}^K\Ex_Q\left[\ell(f(X),k)\ones\{Y=k\}\right] \\
&= \Ex_Q\left[\ell(f(X),Y)\right],
\end{aligned}
\]
where we recalled $q\{x,Y=k\} = p\{x,Y=k\}\exp(\theta_k^\top T(x))$ in the second step. Alternatively, it is also possible to plug in estimates of the $p\{x,Y=k\}$'s and the $\theta_k$'s into $\eta_Q$ to obtain
\[
\heta_Q(x) \gets \frac{\hp\{x,Y=k\}\exp(\theta_k^\top T(x))}{\sum_{l=1}^K\hp\{x,Y=l\}\exp(\theta_l^\top T(x))}.
\]
We prefer weighted ERM because it avoids estimating the $p\{x,Y=k\}$'s and it is more robust to model misspecification. \YK{elaborate on robustness to model misspecification}

\begin{algorithm}
\caption{ExTRA: Exponentailly tilted reweighted adaptation}\label{alg:DAET}
\begin{algorithmic}[1]
\State train classifier for source domain: $\heta_P\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\right]$
\State fit exponential tilt model:
\[
\{\htheta_k\}_{k=1}^K\in\argmax_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\left(\sum_{k=1}^K\big[\heta_P(X)\big]_k\exp(\theta_k^\top T(X))\right)\right]
\]
\State train classifier for target domain: $\heta_Q\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\exp(\htheta_Y^\top T(X))\right]$
\end{algorithmic}
\end{algorithm}


==> exponential-tilt(ICLR2023)/sections/expt.tex <==
\section{Experiments}

\subsection{LDA}
We evaluate the performance of the exponentially tilted approach on a simulated data from LDA model. The source ($P$) distribution is a mixture of the two classes ($y = \pm 1$) with probability for class $y = -1$ being $0.75$ , and the class conditional distributions are $x | y \sim N\big((y, y)^\top, I_2\big), ~ y = \pm 1$. The target ($Q$) is also a mixture of two classes with equal probability for the two classes and the class conditional distributions $x | y \sim N\big((-y, y)^\top, I_2\big), ~ y = \pm 1$.    The data-points are plotted in Figure \ref{fig:LDA} along with the decision boundaries. The boundary with unlabeled target distribution is obtained using the exponentially tilted model where the tilt parameters (with $T(x) = x_1$) are calculated from the MLE approach \eqref{eq:mle}.
\begin{figure}
 \vspace{.05in}
\centering
\includegraphics[width=\linewidth]{plots/LDA.pdf}
\vspace{-.3in}
\caption{}
%  \vspace{-.05in}
\label{fig:LDA}
\end{figure}

==> exponential-tilt(ICLR2023)/sections/identifiability.tex <==
\section{Theoretical properties of exponential tilting}
\label{sec:theory}
\subsection{Identifiability of the exponential tilt model}
\label{sec:identifiability}
To show that the $\theta_k$'s and $\alpha_k$'s are identifiable from \eqref{eq:distribution-matching}, we must show that there is a unique solution to \eqref{eq:distribution-matching}. Unfortunately, this is not always the case. For example, consider a linear discriminant analysis (LDA) problem in which the class conditionals drift between the source and target domains:
\[
\begin{aligned}
p\{x,Y=k\} &= \pi_k\phi(x-\mu_{P,k}), ~~~
q\{x,Y=k\} &= \pi_k\phi(x-\mu_{Q,k})\,,
\end{aligned}
\]
where $\phi$ is the standard multivariate normal density, $\pi_k\in(0,1)$ are the class proportions in both source and target domains, and $\mu_{P,k}$'s (resp.\ the $\mu_{Q,k}$'s) are the class conditional means in the source (resp.\ target) domains. We see that this problem satisfies the exponential tilt model with $T(x) = x$:
\[ \textstyle
\log\frac{q\{x,Y=k\}}{p\{x,Y=k\}} = (\mu_{Q,k} - \mu_{P,k})^\top x - \frac12\|\mu_{Q,k}\|_2^2 +\frac12\|\mu_{P,k}\|_2^2\,.
\]
This instance of the exponential tilt model is not identifiable. Any permutation of the class labels $\sigma:[K]\to[K]$ also leads to the same (marginal) distribution of inputs:
\[
\begin{aligned}
&\textstyle\sum_{k=1}^Kp\{x,Y=k\}\exp\left(\textstyle(\mu_{Q,k} - \mu_{P,k})^\top x + \frac12\|\mu_{P,k}\|_2^2 - \frac12\|\mu_{Q,k}\|_2^2\right) \\
&\textstyle\quad= \sum_{k=1}^Kp\{x,Y=k\}\exp\left(\textstyle(\mu_{Q,\sigma(k)} - \mu_{P,k})^\top x + \frac12\|\mu_{P,k}\|_2^2 - \frac12\|\mu_{Q,\sigma(k)}\|_2^2\right).
\end{aligned}
\]
From this example, we see that the non-identifiability of the exponential tilt model is closely related to the label switching problem in clustering. Intuitively, the exponential tilt model in the preceding example is too flexible because it can tilt any $p\{x,Y=k\}$ to $q\{x,Y=l\}$. Thus there is ambiguity in which $p\{x,Y=k\}$ tilts to which $q\{x,Y=l\}$. In the rest of this subsection, we present an identification restriction that guarantees the identifiability of the exponential tilt model.

A standard identification restriction in related work on domain adaptation is a clustering assumption. For example, \citet{tachet2020Domain} assume there is a partition of $\cX$ into disjoint sets $\cX_k$ such that $\supp(P\{\cdot\mid Y=k\}),\ \supp(Q\{\cdot\mid Y=k\}) \subset \cX_k$ for all $k\in[K]$. This assumption is strong: it implies there is a perfect classifier in the source and target domains. Here we consider a weaker version of the clustering assumption: there are sets $\cS_k$ such that
\[
P\{Y=k\mid X\in\cS_k\} = Q\{Y=k\mid X\in\cS_k\} = 1.
\]
We note that the $\cS_k$'s can be much smaller than the $\cX_k$'s; this permits the supports of $P\{\cdot\mid Y=k\}$ and $P\{\cdot\mid Y=l\}$ to overlap. 

\begin{definition}[anchor set]
\label{def:anchor-set}
A set $\cS_k\subset\cX$ is an \textbf{anchor set} for class $k$ if $p\{x,Y=k\} > 0$ and $p\{x,Y=l\} = 0$, $l\ne k$ for all $x\in\cS_k$.
\end{definition}

% In terms of the regression function (in the source domain) $\eta_P$, an anchor set for the $k$-th class is a set of points such that $\big[\eta_P(x)\big]_k = 1$.

\begin{proposition}[identifiability from anchor sets]
\label{prop:anchor-points} 
If there are anchor sets $\cS_k$ for all $K$ classes (in the source domain) and $T(\cS_k)$ is $p$-dimensional, then there is at most one set of $\theta_k$'s and $\alpha_k$'s that satisfies \eqref{eq:distribution-matching}.
\end{proposition}



This identification restriction is also closely related to the linear independence assumption in \citet{gong2016Domain}. Inspecting the proof of proposition \ref{prop:anchor-points} (see Appendix \ref{supp:prop:anchor-points}), we see that the anchor set assumption implies linear independence of $\{p_k(x)\exp(\theta_k^\top T(x) + \alpha_k)\}_{k=1}^K$ for any set of $\theta_k$'s and $\alpha_k$'s. We study the anchor set assumption empirically in a synthetic experiment in Appendix \ref{sec:normal-mixture}. Our experiments show that the assumption is mild and is violated only under extreme data scenarios.
% empirically investigates the importance of the anchor set assumption and demonstrates that it is violated only in extreme cases.
% regarding the effectiveness of our exponential tilt model. 


==> exponential-tilt(ICLR2023)/sections/importance-weight-fitting.tex <==
% \section{Learning importance weights}
% \label{sec:importance-weight-learning}

% We learn the importance weights using our exponential tilt model \eqref{eq:exponential-tilt}. We use the labeled source data and unlabeled target data to  fit the exponential tilt model and get estimates for the tilt parameters, say $\{\hcoef_k\}_{k = 1}^K $. Then we estimate the importance weight for a generic source sample point $(x, y)$ as $\hat w(x, y) = \exp(\hcoef_y^\top S(x))$. 

% At a high-level, the proposed method for domain adaptation consists of two steps:
% \begin{enumerate}
% \item \textbf{fit exponential tilt model:} estimate the parameters $\theta_k$'s in the exponential tilt model by matching the tilted (marginal) distribution of the inputs from the source domain with that of the inputs from the target domain;
% \item \textbf{train classifier for target domain:} construct/train a classifier for the target domain by plugging in the estimates of $q\{x,Y=k\}$ into \eqref{eq:target-regression-function} or weighted empirical risk minimization (ERM).
% \end{enumerate}
% We elaborate on the two steps in the rest of this section and summarize the method in algorithm \ref{alg:DAET}.





\paragraph{Fitting the exponential tilt model} 
We fit the exponential tilt model via distribution matching. This step is based on the observation that under the exponential tilt model \eqref{eq:exponential-tilt}
\begin{equation} \textstyle
q_X\{x\} = \sum_{k=1}^Kp\{x,Y=k\}\exp(\theta_k^\top T(x) + \alpha_k),
\label{eq:distribution-matching}
\end{equation}
where $q_X$ is the (marginal) density of the inputs in the target domain. It is possible to obtain an estimate $\hq_X$ of $q_X$ from the unlabeled samples $\{X_{i, Q}\}_{i=1}^{n}$ and estimates $\hp\{x,Y=k\}$ of the $p\{x,Y=k\}$'s from the labeled samples $\{(X_{i, P},Y_{i, P})\}_{i=1}^{m}$. This suggests we find $\theta_k$'s and $\alpha_k$'s such that  \[ \textstyle
\sum_{k=1}^K\hp\{x,Y=k\}\exp(\theta_k^\top T(x) + \alpha_k) \approx \hq_X\{x\}.
\] 
Note that the $\theta_k$'s and $\alpha_k$'s are dependent because $\widehat{q}_X$ must integrate to one. We enforce this restriction as a constraint in the distribution matching problem:
\begin{equation}
\{(\htheta_k, \hat \alpha_k)\}_{k=1}^K \in \left\{
\begin{aligned}
& \argmin_{\{(\theta_k, \alpha_k)\}_{k=1}^K}D\left(\textstyle\hq_X\{x\}\|\sum_{k=1}^K\hp\{x,Y=k\}\exp(\theta_k^\top T(x) + \alpha_k)\right)\\
& \text{subject to }\textstyle \int_{\cX} \sum_{k=1}^K\hp\{x,Y=k\}\exp(\theta_k^\top T(x) + \alpha_k)dx = 1\,, 
\end{aligned}
\right.
\label{eq:robust-distribution-matching}
\end{equation}
where $D$ is a discrepancy between probability distributions on $\cX$. Although there are many possible choices of $D$, we pick the Kullback-Leibler (KL) divergence in the rest of this paper because it leads to some computational benefits. We reformulate the above optimization for KL-divergence to relax the constraint which we state in the following lemma.  
% For example, if $D$ is the Kulback-Leibler (KL) divergence, then we can rewrite \eqref{eq:robust-distribution-matching} (dropping the constraint to save space) as:
% \begin{equation}
% \begin{aligned}
% & \argmin_{\{(\theta_k, \alpha_k)\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\hq_X\{X\} - \log\Big\{\sum_{k=1}^K\hp\{X,Y=k\}\exp(\theta_k^\top T(X) + \alpha_k)\Big\}\right] \\
% &\quad\equiv\argmax_{\{(\theta_k, \alpha_k)\}_{k=1}^K}\textstyle\Ex_{\hQ_X}\left[\textstyle\log\Big\{\sum_{k=1}^K\heta_{P,k}(X)\exp(\theta_k^\top T(X) + \alpha_k\Big\}\right] - \Ex_{\hQ_X} \Big[\log\Big\{\frac{q_X\{x\}}{p_X\{x\}}\Big\}\Big],
% \end{aligned}
% \label{eq:KL-distribution-matching}
% \end{equation}
% where $\hQ_X$ is the empirical distribution of the (unlabeled) samples from the target domain and $\heta_P:\cX\to\Delta^{K-1}$ is an estimate of the regression function in the source domain:
% \[ \textstyle
% \left[\eta_P(x)\right]_k \triangleq P\{Y=k\mid X=x\}.
% \] The term $-\Ex_{\hQ_X} \big[\log\big\{\frac{q_X\{x\}}{p_X\{x\}}\big\}\big]$ in our objective does not involve any tilt parameters and we drop it from our objective. 
% We rewrite the constraint in  \eqref{eq:robust-distribution-matching} as
% \begin{equation}
%     \textstyle
%     \int_{\cX} \sum_{k=1}^K\hp\{x,Y=k\}\exp(\theta_k^\top T(x) + \alpha_k)dx  = \Ex_{\hP} \big[ \exp(\theta_Y^\top T(X) + \alpha_Y) \big] = 1.
% \end{equation}
% notice that for a given parameter values $\{(\theta_k, \alpha_k)\}_{k = 1}^K$ one can easily enforce the constraint  by setting \[ \textstyle
% \alpha_k' = \alpha_k - \log \big\{\Ex_{\hP} \big[ \exp(\theta_Y^\top T(X) + \alpha_Y) \big]\big\}\,.
% \] 
% Hence, we rewrite \eqref{eq:robust-distribution-matching} as an unconstrained optimization problem:
% $\{(\theta_k, \alpha_k')\}_{k = 1}^K$:
% \begin{equation}
% \begin{aligned}
% \textstyle\{(\htheta_k, \hat \alpha_k')\}_{k=1}^K \in  \argmax_{\{(\theta_k, \alpha_k')\}_{k=1}^K}\Ex_{\hQ_X} \left[\textstyle\log\Big\{\sum_{k=1}^K\heta_{P,k}(X)\exp(\theta_k^\top T(X) + \alpha_k'\Big\}\right]\\
% %  - \textstyle\log \big\{\Ex_{\hP} \big[ \exp(\theta_Y^\top T(X) + \alpha_Y) \big]\big\}.
% \end{aligned}
% \label{eq:KL-distribution-matching}
% \end{equation}


\begin{lemma}
\label{lemma:KL-distribution-matching}
If $D$ is the Kullback-Leibler (KL) divergence then optima in \eqref{eq:distribution-matching} is achieved at $\{(\htheta_k, \hat\alpha_k)\}_{k = 1}^K$ where 
\[
\begin{aligned}
\textstyle\{(\htheta_k, \hat \alpha_k')\}_{k=1}^K \in  \argmax_{\{(\theta_k, \alpha_k')\}_{k=1}^K}\Ex_{\hQ_X} \left[\textstyle\log\Big\{\sum_{k=1}^K\heta_{P,k}(X)\exp(\theta_k^\top T(X) + \alpha_k'\Big\}\right]\\
 - \textstyle\log \big\{\Ex_{\hP} \big[ \exp(\theta_Y^\top T(X) + \alpha_Y') \big]\big\}
\end{aligned}\] $\heta_{P} = \{\heta_{P, k}\}_{k = 1}^K$ is a probabilistic classifier for $P$ and $\hat \alpha_k = \hat \alpha_k' - \log \big\{\Ex_{\hP} \big[ \exp(\htheta_Y^\top T(X) +\hat  \alpha_Y') \big]\big\}$. 
\end{lemma}



One benefit of minimizing the KL divergence is that the learner does not need to estimate the $p\{x,Y=k\}$'s, a generative model that is difficult to train.  They merely need to train a discriminative model to estimate $\heta_P$ from the (labeled) samples from the source domain. 

We plug the fitted $\htheta_k$'s and $\hat \alpha_k$'s into \eqref{eq:weights-estimate} to obtain Exponential Tilt Reweighting Alignment (ExTRA) importance weights:
\begin{equation}
\widehat{\weight}(x,y) = \exp(\htheta_y^\top T(x) + \hat \alpha_y).
\label{eq:weights-estimate}
\end{equation}
We summarize the ExTRA procedure in Algorithm \ref{alg:extra} in Appendix \ref{sup:exp:model}.

Next we describe two downstream tasks where ExTRA weights can be used: 
\begin{enumerate}
\item \textbf{ExTRA model evaluation in the target domain.}
% Armed with estimates of the importance weights, 
Practitioners may estimate the target performance of a model in the target domain by reweighing the empirical risk in the source domain:
\begin{equation}
   \textstyle \label{eq:target-performance}
\Ex\left[\ell(f(X_Q),Y_Q)\right] \approx \frac{1}{n_P}\sum_{i=1}^{n_P}\ell(f(X_{P,i}),Y_{P,i})\widehat{\weight}(X_{P,i}, Y_{P,i}), 
\end{equation}
where $\ell$ is a loss function. This allows to evaluate models in the target domain without target labeled samples \emph{even in the presence of concept drift between the training and target domain}.
\item \textbf{ExTRA fine-tuning for target domain performance.} Since the reweighted empirical risk (in the source domain) is a good estimate of the risk in the target domain, practitioners may fine-tune models for the target domain by minimizing the reweighted empirical risk:
\begin{equation}
\widehat{f}_Q\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\widehat{\weight}(X, Y)\right].
\label{eq:weighted-ERM}
\end{equation}
\end{enumerate}

We note that the correctness of \eqref{eq:robust-distribution-matching} depends on the identifiability of the $\theta_k$'s and $\alpha_k$'s from  \eqref{eq:distribution-matching}; \ie\ the uniqueness of the parameters that satisfy \eqref{eq:distribution-matching}. As long as the tilt parameters are identifiable, then \eqref{eq:robust-distribution-matching} provides consistent estimates of them. However, without additional assumptions on the $p\{x,Y=k\}$'s and $T$, the tilt parameters are generally unidentifiable from \eqref{eq:distribution-matching}. Next we elaborate on the identifiability of the exponential tilt model.
% (see section \ref{sec:identifiability} for an example). We elaborate on the identifiability of the exponential tilt model in section \ref{sec:identifiability}.

% we train a classifier for the target domain by weighted ERM in the second step:
%  The weight function in \eqref{eq:weighted-ERM} is chosen so that expected value of the cost function in \eqref{eq:weighted-ERM} is exactly the risk in the target domain:
% \[
% \begin{aligned}
% \Ex_P\left[\ell(f(X),Y)\exp(\theta_Y^\top T(X))\right] &= \sum_{k=1}^K\Ex_P\left[\ell(f(X),k)\exp(\theta_k^\top T(X))\ones\{Y=k\}\right] \\
% &= \sum_{k=1}^K\Ex_Q\left[\ell(f(X),k)\ones\{Y=k\}\right] \\
% &= \Ex_Q\left[\ell(f(X),Y)\right],
% \end{aligned}
% \]
% where we recalled $q\{x,Y=k\} = p\{x,Y=k\}\exp(\theta_k^\top T(x))$ in the second step. Alternatively, it is also possible to plug in estimates of the $p\{x,Y=k\}$'s and the $\theta_k$'s into $\eta_Q$ to obtain
% \[
% \heta_Q(x) \gets \frac{\hp\{x,Y=k\}\exp(\theta_k^\top T(x))}{\sum_{l=1}^K\hp\{x,Y=l\}\exp(\theta_l^\top T(x))}.
% \]
% We prefer weighted ERM because it avoids estimating the $p\{x,Y=k\}$'s and it is more robust to model misspecification. \YK{elaborate on robustness to model misspecification}

% \begin{algorithm}
% \caption{ExTRA: Exponentailly tilted reweighted adaptation}\label{alg:DAET}
% \begin{algorithmic}[1]
% \State train classifier for source domain: $\heta_P\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\right]$
% \State fit exponential tilt model:
% \[
% \{\htheta_k\}_{k=1}^K\in\argmax_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\left(\sum_{k=1}^K\big[\heta_P(X)\big]_k\exp(\theta_k^\top T(X))\right)\right]
% \]
% \State train classifier for target domain: $\heta_Q\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\exp(\htheta_Y^\top T(X))\right]$
% \end{algorithmic}
% \end{algorithm}


==> exponential-tilt(ICLR2023)/sections/intro.tex <==
\section{Introduction}

Machine learning models are often deployed in a target domain that differs from the domain in which they were trained and validated in. This leads to the practical challenges of adapting and evaluating the performance of models on a new domain without costly labeling of the dataset of interest. For example, in the Inclusive Images challenge \citep{shankar2017No}, the training data largely consists of images from countries in North America and Western Europe.
If a model trained on this data is presented with images from countries in Africa and Asia, then (i) it is likely to perform poorly, and (ii) its performance in the training (source) domain may not mirror its performance in the target domain. 
However, due to the presence of a small fraction of images from Africa and Asia in the source data, it may be possible to reweigh the source samples to mimic the target domain.

In this paper, we consider the problem of learning a set of importance weights so that the reweighted source samples closely mimic the distribution of the target domain. We pose an exponential tilt model of the distribution shift between the train and the target data and an accompanying method that leverages unlabeled target data to fit the model. Although similar methods are widely used in statistics \cite{rosenbaum1983central} and machine learning \cite{sugiyama2012Density} to train and evaluate models \emph{under covariate shift} (where the decision function/boundary does not change), one of the main benefits of our approach is it allows \emph{concept drift} (where the decision boundary/function are expected to differ) \citep{cai2019Transfer,gama2014survey} between the source and the target domains.
We summarize our contributions below:
\begin{itemize}
\item In Section \ref{sec:exponential-tilt} we develop a model and an accompanying method for learning source importance weights to mimic the distribution of the target domain \emph{without} labeled target samples.
\item In Section \ref{sec:theory} we establish theoretical guarantees on the quality of the weight estimates and their utility in the downstream tasks of fine-tuning and model selection.
\item We demonstrate applications of our method on \waterbirds\ \citep{sagawa2019Distributionally} (Section \ref{sec:waterbird}),  \breeds\ \citep{santurkar2020breeds} (Section \ref{sec:breeds}) and synthetic (Appendix \ref{sec:normal-mixture}) datasets.  
\end{itemize}



==> exponential-tilt(ICLR2023)/sections/linear-independence.tex <==
\subsection{Linear independence}

\paragraph{Exponential tilting} Let $\{p_k(x)\}_{k=1}^K$ be the class conditionals in the training domain, and $q(x)$ be the (marginal) density of the features in the target domain. We wish to show that is a unique set of $\theta_k$'s such that
\[
\sum_{k=1}^Kp_k(x)e^{\theta_k^\top T(x)} = q(x),
\]
where $T(x)$ is a vector of sufficient statistics that includes a constant entry. Suppose there is another set of $\eta_k$'s that satisfies the preceding equation. We must have
\begin{equation}
\sum_{k=1}^Kp_k(x)(e^{\theta_k^\top T(x)} - e^{\eta_k^\top T(x)}) = 0.
\label{eq:difference-zero}
\end{equation}
We assume
\begin{equation}
\{p_k(x)(e^{\theta_k^\top T(x)} - e^{\eta_k^\top T(x)})\}_{k=1}^K\text{ is linearly independent for any $\theta_k$'s and $\eta_k$'s such that $\theta_k \neq \eta_k$.}
\label{eq:linear-independence}
\end{equation}
This implies \eqref{eq:difference-zero} occurs if and only if the terms in the sum are all zero:
\[
p_k(x)(e^{\theta_k^\top T(x)} - e^{\eta_k^\top T(x)}) = 0,\quad k\in[K],
\]
which implies $e^{\theta_k^\top T(x)} = e^{\eta_k^\top T(x)},
$ because $p_k \ne 0$. We appeal to Lemma \ref{lemma:linear-indep} to deduce $\theta_k = \eta_k$.

The linear independence assumption seems restrictive because it requires linear independence for any choice of $\theta_k$'s and $\eta_k$'s, but it is actually mild. For example, if the supports of the $p_k$'s are disjoint, then \eqref{eq:linear-independence} is satisfied. A milder (sufficient) condition is there are points $x_1,\dots,x_K$ such that $p_k(x_k) > 0$ but $p_{l\ne k}(x_k) = 0$ for all $k$. This condition is motivated by the identification restrictions in \cite{gong2016Domain,tachet2020Domain}.

\paragraph{General parametric model} Instead of tilting, consider a general parametric model for the class conditionals in the target domain:
\[
q_k(x) = (A_{\theta_k}p_k)(x),
\]
where $\cA \triangleq \{A_\theta:\theta\in\Theta\}$ is a parameterized family of Markov kernels. If we assume 
\begin{equation}
\{A_{\theta_k}p_k - A_{\eta_k}p_k\}_{k=1}^K\text{ is linearly independent for any $\theta_k$'s and $\eta_k$'s such that $\theta_k\ne\eta_k$},
\label{eq:general-linear-independence}
\end{equation}
then (a version of) the preceding argument shows that the target class conditionals are identifiable. We interpret \eqref{eq:general-linear-independence} is a restriction on the richness of the family of Markov kernels: if there is $\theta$ such that $p_k = A_{\theta}p_l$ for a pair of (distinct) class conditionals, then \eqref{eq:general-linear-independence} fails.

Another way to interpret \eqref{eq:general-linear-independence} is a well-separation condition on the $p_k$'s. t

==> exponential-tilt(ICLR2023)/sections/methods.tex <==
Given that they are identifiable one can estimate the parameters  from the following estimating equation: 
    \[
    E_{Q_X}[f] = \pi_Q E_{P_0}\big[ f(x) e^{\beta_0^\top \Phi(x)} \big] + (1 - \pi_Q) E_{P_1}\big[ f(x) e^{\beta_1^\top \Phi(x)} \big]
    \] Here, the related questions follow. \emph{1. What is a  good choices of $f$? 2. What is the rate of convergence for the parameters? 3. What is the rate of convergence for excess risk? This may involve a non-vanishing error term to capture a model misspecification.}  

==> exponential-tilt(ICLR2023)/sections/proofs.tex <==

\section{Proofs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% PROOF OF KL OBJECTIVE %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rademacher complexity}
\label{supp:rademacher}
We next define the Rademacher complexity \citep{bartlett2002rademacher} that  has been frequently used in  machine learning literature to establish a generalization bound. 
Instead of considering the Rademacher complexity on $\cF$ we define the class of weighted losses $\cG(\ell, \cF) = \{g_f(x, y) = w^\star(x, y) \ell(f(x), y): \ f \in \cF\}$  and for $n \in \bbN$ we define its Rademacher complexity measure as 
\[ \textstyle
    \cR_n(\cG) \triangleq \Ex_{\{(u_i, v_i)\}_{i = 1}^n\stackrel{\IID}{\sim} P} \big[\Ex_{\{\xi_i\}_{i = 1}^n}[\sup_{f \in \cF} \frac1{n} \sum_{i = 1}^n \xi_i \weight^\star(u_i, v_i) \ell \{f(u_i), v_i\}]\big]
\]
where $\{\xi_i\}_{i = 1}^n $ are \IID \

\subsection{Proof of lemma \ref{lemma:KL-distribution-matching}}

If $D$ is the Kulback-Leibler (KL) divergence, then we can rewrite the objective in  \eqref{eq:robust-distribution-matching}  as:
\[
\begin{aligned}
& \Ex_{\hQ_X}\left[\textstyle\log\hq_X\{X\} - \log\Big\{\sum_{k=1}^K\hp\{X,Y=k\}\exp(\theta_k^\top T(X) + \alpha_k)\Big\}\right] \\
&\quad=\textstyle\Ex_{\hQ_X}\left[\textstyle\log\Big\{\sum_{k=1}^K\heta_{P,k}(X)\exp(\theta_k^\top T(X) + \alpha_k\Big\}\right] - \Ex_{\hQ_X} \Big[\log\Big\{\frac{q_X\{x\}}{p_X\{x\}}\Big\}\Big],
\end{aligned}
\] where the term $-\Ex_{\hQ_X} \big[\log\big\{\frac{q_X\{x\}}{p_X\{x\}}\big\}\big]$ in our objective does not involve any tilt parameters and we drop it from our objective. To simplify the notations we define \[
\begin{aligned}
O(\theta, \alpha) &\triangleq \Ex_{\hQ_X}\left[\textstyle\log\Big\{\sum_{k=1}^K\heta_{P,k}(X)\exp(\theta_k^\top T(X) + \alpha_k\Big\}\right]\\
N(\theta, \alpha) &\triangleq \Ex_{\hP} \big[ \exp(\theta_Y^\top T(X) + \alpha_Y) \big]\,.
\end{aligned}
\] 
where $(\theta, \alpha) \in \reals^q$ for $q = K(p+1)$. 
In terms of $O$ and $N$, \eqref{eq:distribution-matching} is
\begin{equation} \label{eq:objs1}
    (\hat \theta , \hat \alpha) = \argmax_{(\theta, \alpha)} \left\{ O(\theta, \alpha)\mid  N(\theta, \alpha) = 1 \right\}.
\end{equation}
Let $F_1 \triangleq \{ (\theta, \alpha)\mid  N(\theta, \alpha) = 1 \}$ be the feasible set. We introduce a change of variables:
\[
c(\theta , \alpha') = (\theta, \alpha(\theta, \alpha'))  ~ \text{ where } ~ \alpha(\theta, \alpha') = \alpha' - 1_K\log(N(\theta, \alpha')).
\] Note that for any $(\theta , \alpha') \in \reals^q,~ c(\theta , \alpha') \in F_1$ because  it holds: 
\[
\begin{aligned}
N(c(\theta, \alpha')) & =  N(\theta, \alpha' - \log(N(\theta, \alpha')) \times 1_K)\\
& = \Ex_{\hP} \big[ \exp(\theta_Y^\top T(X) + \alpha_Y' - \log(N(\theta, \alpha'))) \big]\\
& = \frac{\Ex_{\hP} \big[ \exp(\theta_Y^\top T(X) + \alpha_Y' ) \big]}{N(\theta, \alpha')} = 1\,.
\end{aligned}
\] and the objective value changes to 
\[
\begin{aligned}
O(c(\theta, \alpha')) & = \Ex_{\hQ_X}\left[\textstyle\log\Big\{\sum_{k=1}^K\heta_{P,k}(X)\exp[\theta_k^\top T(X) + \alpha_k'  - \log(N(\theta, \alpha')]\Big\}\right] \\
& = \Ex_{\hQ_X}\left[\textstyle\log\Big\{\sum_{k=1}^K\heta_{P,k}(X)\exp[\theta_k^\top T(X) + \alpha_k'  ]\Big\}\right] - \log(N(\theta, \alpha'))\\
& = O(\theta, \alpha')  - \log(N(\theta, \alpha'))\,.
\end{aligned}
\] 
Defining $F_2 = \{c(\theta, \alpha')\mid (\theta, \alpha')\in \reals^q\}$ we see that $F_1 = F_2$, whose argument follows.  We first notice that $F_2 \subset F_1$ since for any $(\theta , \alpha')\in \reals^q $ it holds $ c(\theta , \alpha') \in F_1$. We also notice that $F_1 \subset F_2$. This is argued by noticing the following: if $(\theta, \alpha') \in F_1$ then $N(\theta,\alpha') = 1$ which implies $c(\theta, \alpha') = (\theta, \alpha')$. 

Here, we summarize the crux of the proof. 
Though there are multiple $(\theta, \alpha')$ that produces the same value of $c(\theta, \alpha')$, each of these $(\theta, \alpha')$'s produce the same value for the objective
\[
O(\theta, \alpha')  - \log(N(\theta, \alpha')) = O(c(\theta, \alpha'))\,,
\] and $c(\theta, \alpha')$ always satisfy the constraint. So, the optimal point $(\theta, \alpha)$ of \eqref{eq:objs1} corresponds to multiple $(\theta, \alpha')$'s and each of them maximizes $O(\theta, \alpha')  - \log(N(\theta, \alpha'))$. Furthermore, we obtain the optimal  $(\theta, \alpha)$ from any of $(\theta, \alpha')$ (which optimizes $O(\theta, \alpha')  - \log(N(\theta, \alpha'))$) using the transformation $c(\theta, \alpha')$. 

The mathematical description of the change of variable follows.
With the change of variable we rewrite \eqref{eq:objs1} as
\[
\begin{aligned}
& (\hat \theta , \hat \alpha) =  c(\hat \theta , \hat \alpha'), ~ (\hat \theta , \hat \alpha')= \argmax_{(\theta, \alpha')} \left\{ O(c(\theta, \alpha'))\mid  N(c(\theta, \alpha')) = 1, (\theta, \alpha')\in \reals^q  \right\}\\
\text{or }& (\hat \theta , \hat \alpha) =  c(\hat \theta , \hat \alpha'), ~ (\hat \theta , \hat \alpha')  = \argmax_{(\theta, \alpha')} \left\{ O(\theta, \alpha') - \log(N(\theta, \alpha')) \mid  (\theta, \alpha') \in \reals^q \right\}
\end{aligned}
\] where the constraint disappear because $N(c(\theta, \alpha')) = 1$ for any $(\theta, \alpha') \in \reals^q$. This completes the proof. 

% \begin{equation}
%     \max\left\{ O(\theta, \alpha')  - \log(N(\theta, \alpha'))\mid  (\theta, \alpha') \right\}
% \end{equation}
% The constraint disappear because  such a change of variable always satisfy the constraint. So, the set $F_2 = \{c(\theta, \alpha')\mid (\theta, \alpha')\}$ is a 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% PROOF OF ANCHOR POINTS %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of proposition \ref{prop:anchor-points}}
\label{supp:prop:anchor-points}

Suppose there are two sets of tilt parameters $(\theta_k, \alpha_k)$'s and $(\eta_k, \beta_k)$'s that satisfy \eqref{eq:distribution-matching}:
\[
q_X\{x\} = \sum_{k=1}^Kp\{x,Y=k\}\exp(\theta_k^\top T(x)+ \alpha_k) = \sum_{k=1}^Kp\{x,Y=k\}\exp(\eta_k^\top T(x) +\beta_k).
\]
For any $x\in\cS_k$, the terms that include $p\{x,Y=l\}$, $l\ne k$ vanish:
\[
p\{x,Y=k\}\exp(\theta_k^\top T(x)+\alpha_k) = p\{x,Y=k\}\exp(\eta_k^\top T(x)+\beta_k).
\]
This implies
\[
\theta_k^\top T(x) + \alpha_k = \eta_k^\top T(x) + \beta_k \text{ for all }x\in\cS_k.
\]
We conclude $\theta_k = \eta_k$ and $\alpha_k = \beta_k$ because $T(\cS_k)$ is  $p$-dimensional, so there are $p$ points $x_1,\dots,x_p\in\cS_k$ such that $T(x_1),\dots,T(x_p)\in\reals^p$ are linearly independent. 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% PROOF OF CONSISTENCY %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\subsection{Proof of Theorem \ref{thm:tilt-concentration}}



For a probabilistic classifier  $\eta: \cX \to \Delta^K$ and the parameter $\coef = (\coef_1^\top , \dots, \coef_K^\top )^\top$
we define the centered logit function $f:\cX \to \reals^K$  as $f_a(x) = \log\{\eta_a(x)\} - \frac 1K \sum_{b = 1}^K \log\{\eta_b(x)\}$. 
We define the functions $u_k(f, \coef) = \eta_a(x) \exp(\coef_k^\top S(x))$, $u_{\cdot} (f, \coef) = \sum_{k=1}^K u_k(f, \coef)$ and $v_k(f, \coef) = u_k(f, \coef)/u_{\cdot}(f, \coef)$, and notice that the objective is
\begin{equation} \textstyle
    \hat L(f, \coef)   = \Ex_{\hQ_X} [\log\{ u_{\cdot}(f, \coef) \}] - \log\{ \Ex_{\hP}[\exp(\coef_y ^\top S(x))] \}\,,
\end{equation}  whereas the true objective is 
\begin{equation} \textstyle
      L^\star( f, \coef)  = \Ex_{Q_X} [\log\{ u_{\cdot}(f, \coef) \}] - \log\{ \Ex_{P}[\exp(\coef^\top_y S(x))] \}\,.
\end{equation}
We see that the first order optimality conditions in estimating $\hat \coef$ are 
\begin{equation} \textstyle \label{eq:optimality-estimation}
\begin{aligned}
 0 & = \partial_{\coef_a} \hat L(\hat f, \hat \coef)\\
 & = \partial_{\coef_a}\big[ \Ex_{\hQ_X} [\log\{ u_{\cdot}(\hat f, \hat \coef) \}] - \log\{ \Ex_{\hP}[\exp( {\hat \coef_y} ^\top S(x))] \}\big]\\
 & = \Ex_{\hQ_X}\big[ \partial_{\coef_a} \{u_{\cdot}(\hat f, \hat \coef)\}/u_{\cdot}(\hat f, \coef) \big] - \frac{\partial_{\coef_a}\{ \Ex_{\hP}[\exp({\hat \coef_y} ^\top S(x))] \}}{ \Ex_{\hP}[\exp({\hat \coef_y} ^\top S(x))]}\\
 & = \Ex_{\hQ_X} [S(x)v_a(\hat f, \hat \coef)] - \Ex_{\hP}[S(x)\exp({\hat \coef_a} ^\top S(x))\bI\{y = a\}] 
\end{aligned}
  \end{equation} where the last inequality holds because $\Ex_{\hP}[\exp(\hcoef_y ^\top S(x))] = 1$. 
Similarly, the first order optimality condition at truth (for $\coef^\star$) are 
 \begin{equation}
     \textstyle \label{eq:optimality-truth}
     \begin{aligned}
     0 &= \partial_{\coef_a}  L^\star( f^\star,  \coef^\star)\\
     &= \Ex_{Q_X} [S(x)v_a( \sf,  \scoef)] - \Ex_{P}[S(x)\exp({\coef_a^\star} ^\top S(x))\bI\{y = a\}]\\
     &= \Ex_{Q_X} [S(x)v_a( \sf,  \scoef)] - \Ex_{P_X}[S(x)\exp({\coef_a^\star} ^\top S(x))\eta_{P, a}^\star(x)]
     \end{aligned}
 \end{equation} We decompose \ref{eq:optimality-estimation} using the Taylor expansion and obtain: 
 \begin{equation} \textstyle
 \label{eq:optimality-theta-hat}
     0 = \partial_{\coef_a} \hL (\sf, \hcoef) + \langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle 
 \end{equation} where $\tilde f$ is a function in the bracket $[f^\star, \hat f]$, \ie\ for every $x$, $\tilde f(x)$ is a number between $\hat f(x)$ and $f^\star(x)$
\paragraph{Bound on $\langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle $:} To bound the term we define $\zeta = \hf - \sf$ and  notice that 
\[
\begin{aligned}
  \langle \zeta, \partial_{f} \partial_{\theta_a} \hL( f, \hcoef)\rangle
 & =\textstyle \sum_{b}\langle \zeta_b, \partial_{f_b} \partial_{\theta_a} \hL( f, \hcoef)\rangle\\
 &=\textstyle \sum_{b}\langle \zeta_b, \partial_{f_b} \{\Ex_{\hQ_X} [S(x)v_a(f, \hat \coef)]\} \rangle \\
 &=\textstyle \sum_{b}\Ex_{\hQ_X}[S(x) \zeta_b(x)  \partial_{f_b}\{v_a(f,  \hat \coef) \} ] \\
 &=\textstyle \sum_{b}\Ex_{\hQ_X}[S(x) \zeta_b(x) v_a(f,  \hcoef) (\delta_{ab} - v_a(f, \hcoef))  ]\,.
\end{aligned}
\] 
% where 
% \[
% \begin{aligned}
%  &  \langle \zeta_b, \partial_{f_b} \{\Ex_{\hQ} [T(x)v_a(f,  \theta)]\} \rangle \\
%  & = \Ex_{\hQ}[T(x) \zeta_b(x)  \partial_{f_b}\{v_a(f,  \theta) \} ]\\
%  & = \Ex_{\hQ}[T(x) \zeta_b(x) v_a(f,  \theta) (\delta_{ab} - v_a(f, \theta))  ]\,,
% \end{aligned}
% \] and 
% \[
% \begin{aligned}
% & \langle \zeta_b, \partial_{f_b} \Big\{\frac{\Ex_{\bbP_m}[T(x)u_a( f,  \theta)]}{\Ex_{\bbP_m}[u_{\cdot} (f,  \theta)]}\Big\} \rangle \\
% & = \frac{1}{\{\Ex_{\bbP_m}[u_{\cdot} (f,  \theta)]\}^2} \Big[\langle \zeta_b, \partial_{f_b} \Ex_{\bbP_m}[T(x)u_a( f,  \theta)] \rangle \times \Ex_{\bbP_m}[u_{\cdot} (f,  \theta)]\\
% & ~~~ - \Ex_{\bbP_m}[T(x)u_a( f,  \theta)] \times \langle \zeta_b, \partial_{f_b} \Ex_{\bbP_m}[u_{\cdot}( f,  \theta)] \rangle\Big]\\
% & = \frac{1}{\{\Ex_{\bbP_m}[u_{\cdot} (f,  \theta)]\}^2} \Big[ \Ex_{\bbP_m}[T(x)\zeta_b(x) u_a( f,  \theta)]  \times \Ex_{\bbP_m}[u_{\cdot} (f,  \theta)] \times \delta_{ab}\\
% & ~~~ - \Ex_{\bbP_m}[T(x)u_a( f,  \theta)] \times  \Ex_{\bbP_m}[\zeta_b(x) u_{b}( f,  \theta)] \Big]
% \end{aligned}
% \] 
The derivative in third equality in the above display is calculated in Lemma \ref{lemma:derivatives}. Here, from Assumption \ref{assump:bounded-covariate} we notice that  $S(x)$ is bounded, \ie, there exists a $c_1>0$ such that $\|S(x)\|_2 \le c_1$ for all $x \in \cX$. This implies the followings:   we have
\[
\begin{aligned} 
\textstyle
\|\Ex_{\hQ_X}[S(x) \zeta_b(x) v_a(f,  \coef) (\delta_{ab} - v_a(f, \coef))  ]\|_2
 \le c_1\Ex_{\hQ_X}[ |\zeta_b(x)| ]
\end{aligned}
\] since $0 \le v_a(f,  \coef) (\delta_{ab} - v_a(f, \coef))\le 1$ and we have 
\[
\begin{aligned}
\textstyle
\|\langle \zeta, \partial_{f} \partial_{\theta_a} \hL( f, \hcoef)\rangle\|_2 \le \sum_b c_1\Ex_{\hQ_X}[ |\zeta_b(x)| ] \le c_1 \sqrt{K} \Ex_{\hQ_X}[ \|\zeta(x)\|_2 ]\,.
\end{aligned}
\]
% (2) we have 
% \[
% \begin{aligned}
% & \frac{1}{\{\Ex_{\bbP_m}[u_{\cdot} (f,  \theta)]\}^2} \Big| \Ex_{\bbP_m}[T(x)\zeta_b(x) u_a( f,  \theta)]  \times \Ex_{\bbP_m}[u_{\cdot} (f,  \theta)] \times \delta_{ab}\\
% & ~~~ - \Ex_{\bbP_m}[T(x)u_a( f,  \theta)] \times  \Ex_{\bbP_m}[\zeta_b(x) u_{b}( f,  \theta)] \Big|\\
% & \le \frac{1}{\{\Ex_{\bbP_m}[u_{\cdot} (f,  \theta)]\}^2} \Big[ c_1\Big\{\sup_{i \in[m]} |\zeta_b(x_{i, P}) |\Big\} \Ex_{\bbP_m}[u_a( f,  \theta)]  \times \Ex_{\bbP_m}[u_{\cdot} (f,  \theta)] \\
% & ~~~ +c_1 \Ex_{\bbP_m}[u_a( f,  \theta)] \times  \Big\{\sup_{i \in[m]} |\zeta_b(x_{i, P}) |\Big\} \times \Ex_{\bbP_m}[u_{b}( f,  \theta)] \Big]\\
% & \le 2c_1 \sup_{i \in[m]} |\zeta_b(x_{i, P}) |
% \end{aligned}
% \]
It follows from Assumption \ref{assmp:source-classifier}: with probability at least $ 1- \delta$ it holds   $\sup_{i \in[n_Q]} \|\hf(x_{Q, i}) - \sf(x_{Q,i})\|_2 \le c_2 r_{n_P} \sqrt{\log(n_Q)\log\{1/\delta\}}$, we conclude that  
\begin{equation}
    |\langle \hf - \sf, \partial_{f} \partial_{\theta_a} \hL( f, \theta)\rangle| \le \sqrt{K} c_1 c_2 r_{n_P} \sqrt{\log(n_Q)\log\{1/\delta\}}
\end{equation} holds with probability at least $ 1- \delta$. 

\paragraph{The term $\partial_{\coef_a} \hL(\sf, \hcoef)$}
We use strong convexity \ref{assmp:strong-convexity} and convergence of the loss that \[\sup_{\xi \in K}|\hat L(f^\star, \coef) -   L^\star(f^\star, \coef)| \stackrel{n_P, n_Q \to \infty}{\longrightarrow} 0\] for any compact $K$ in \citet[Corollary 3.2.3.]{vaart2000Weak} to conclude that $\hcoef \to \scoef$ in probability and hence $\hcoef$ is a consistent estimator for $\scoef$.


Following the consistency of $\hcoef$  we see that for sufficiently large $n_P, n_Q$ we have $\|\hcoef - \scoef\|_2 \le \delta_\coef$ ($\delta_\coef$ is chosen according to Lemma \ref{lemma:lb-normalizer}) with probability at least $ 1 -\delta$ and on the event it holds: $\|\hcoef\|_2 \le \|\scoef\|_2 + \delta_\coef$. We define empirical process 
\begin{equation}\label{eq:emp-1st-derivative}
    Z_{a, n_P, n_Q} = \sup_{\|\coef\|_2\le \|\scoef\|_2 + 1} \|\partial_{\coef_a}\hL(\sf, \coef) - \partial_{\coef_a}\sL(\sf, \coef)\|_2
\end{equation}
for which we shall provide a high probability upper bound. We denote $Z_{a, n_P, n_Q}(\coef) = \partial_{\coef_a}\hL(\sf, \coef) - \partial_{\coef_a}\sL(\sf, \coef)$ and notice that 
\[
\begin{aligned}
 & \partial_{\coef_a} \hL(\sf, \coef) - \partial_{\coef_a}\sL(\sf, \coef)\\
& = \underbrace{\Ex_{\hQ_X} [S(x)v_a(\sf,  \coef)] - \Ex_{Q_X} [S(x)v_a(\sf,  \coef)]}_{\triangleq \bA(\coef)}\\
& ~~~~ \underbrace{ -  \frac{\Ex_{\hP}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]}{\Ex_{\hP}[\exp( \coef_y ^\top S(x))]} +  \frac{\Ex_{P}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]}{\Ex_{P}[\exp( \coef_y ^\top S(x))]} }_{\triangleq \bB(\coef)} = \bA(\coef) + \bB(\coef)
\end{aligned}
\]
where to bound $\bA(\coef)$ we notice that $S(x_{Q, i})v_a(\sf,  \coef)$ are \IID\ and bounded by $c_1$ ($\|S(x)v_a(\sf,  \coef)\| \le \|S(x)\|_2 \le c_1$ for all $x\in \cX$) and hence sub-gaussian. We apply Hoeffding's concentration inequality for a sample mean of \IID\  sub-gaussian random variables and obtain a constant $c_2>0$ such that for any $\delta>0$ with probability at least $1 - \delta$ it holds
\[ \textstyle
\bA(\coef) = \Ex_{\hQ_X} [S(x)v_a(\sf,  \coef)] - \Ex_{Q_X} [S(x)v_a(\sf,  \coef)] \le c_1 c_2 \sqrt{\frac{\log (1/\delta)}{n_Q}}\,.
\] Using a chaining argument over an $\ell_2$ ball of radius $\|\scoef\|_2 + \delta_\coef$ we  obtain a uniform bound as the following: there exists a constant $c_2>0$ such that for any $\delta>0$ with probability at least $1 - \delta$ it holds
\begin{equation}
    \textstyle \label{eq:bound.A}
\sup_{\coef: \|\coef \|_2 \le \|\scoef\|_2 + \delta_\coef}\bA(\coef)  \le c_1 c_3  \sqrt{\frac{K(p+1)\log (1/\delta)}{n_Q}}\,.
\end{equation}
To bound $\bB$ we first define 
\[
\begin{aligned}
\bB.1(\coef, n_P) \triangleq & ~\Ex_{\hP}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}] - \Ex_{P}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]\\
\bB.2(\coef, n_P) \triangleq &~ \Ex_{\hP}[\exp( \coef_a ^\top S(x))] - \Ex_{P}[\exp( \coef_a ^\top S(x))]
\end{aligned}
\]
and  notice that both the random variables $\{ S(x_{P, i})\exp( \coef_a ^\top S(x_{P, i}))\bI\{y_{P, i} = a\} \}_{i = 1}^{n_P}$ and $\{ \exp( \coef_a ^\top S(x_{P, i})) \}_{i = 1}^{n_P}$ are bounded for all $\|\coef \|_2 \le \|\scoef\|_2 + \delta_\coef$. Similarly as before we obtain constant $c_4, c_5 > 0$ such that the following hold with probability at least $1- \delta$:
\begin{equation} \label{eq:sup-con-b1b2}
    \begin{aligned}
 \sup_{\coef: \|\coef \|_2 \le \|\scoef\|_2 + \delta_\coef} \big|\bB.1(\coef, n_P)\big|
& \le\textstyle c_4  \sqrt{\frac{K(p+1)\log (1/\delta)}{n_P}}\\
 \sup_{\coef: \|\coef \|_2 \le \|\scoef\|_2 + \delta_\coef} \big|\bB.2(\coef, n_P)\big|
& \le\textstyle c_5  \sqrt{\frac{K(p+1)\log (1/\delta)}{n_P}}\,.
\end{aligned}
\end{equation}
In Lemma \ref{lemma:lb-normalizer} we notice that
\begin{equation}\label{eq:lb-normalizer}
    \inf_{\coef: \|\coef \|_2 \le \|\scoef\|_2 + \delta_\coef} \Ex_{P}[\exp( \coef_y ^\top S(x))] \ge \frac 12\,.
\end{equation}
Gathering all the inequalities  in $\bB$ we obtain
\[
\begin{aligned}
\bB(\coef) & = -  \frac{\Ex_{\hP}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]}{\Ex_{\hP}[\exp( \coef_y ^\top S(x))]} +  \frac{\Ex_{P}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]}{\Ex_{P}[\exp( \coef_y ^\top S(x))]}\\
& = -  \frac{\Ex_{P}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}] +\bB.1(\coef, n_P) }{\Ex_{P}[\exp( \coef_y ^\top S(x))] + \bB.2(\coef, n_P)} +  \frac{\Ex_{P}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]}{\Ex_{P}[\exp( \coef_y ^\top S(x))]}\\
& = \frac{-\bB.1(\coef, n_P)\Ex_{P}[\exp( \coef_a ^\top S(x))] + \bB.2(\coef, n_P)\Ex_{P}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]}{\Big\{\Ex_{P}[\exp( \coef_y ^\top S(x))] + \bB.2(\coef, n_P)\Big\}\Ex_{P}[\exp( \coef_y ^\top S(x))]}
\end{aligned}
\] and this implies 
\[
\begin{aligned}
|\bB(\coef)| & \le  \frac{\|\bB.1(\coef, n_P)\|_2\Ex_{P}[\exp( \coef_a ^\top S(x))] + |\bB.2(\coef, n_P)|\|\Ex_{P}[S(x)\exp( \coef_a ^\top S(x))\bI\{y = a\}]\|_2}{\Big\{\Ex_{P}[\exp( \coef_y ^\top S(x))] - |\bB.2(\coef, n_P)|\Big\}\Ex_{P}[\exp( \coef_y ^\top S(x))]}
\end{aligned}
\] where we use \eqref{eq:sup-con-b1b2} and \eqref{eq:lb-normalizer} to obtain a constant $c_6>0$ such that with probability at least $1 - \delta$ it holds
\begin{equation}\textstyle\label{eq:bound.B}
    \sup_{\coef: \|\coef \|_2 \le \|\scoef\|_2 + \delta_\coef} |\bB(\coef)| \le c_6 \sqrt{\frac{K(p+1)\log (1/\delta)}{n_P}}\,.
\end{equation}
We now combine \eqref{eq:bound.A} and \eqref{eq:bound.B} and obtain a constant $c_7>0$ such that with probability at least $1 - 2\delta$ we have 
\begin{equation} \textstyle\label{eq:emp-ub}
    Z_{a, n_P, n_Q} \le c_7 \left\{\sqrt{\frac{K(p+1)\log (1/\delta)}{n_P}} + \sqrt{\frac{K(p+1)\log (1/\delta)}{n_Q}}\right\}\,.
\end{equation}

% Here, we notice the following: $T(x)v_a(\sf,  \coef)$, $T(x)u_a(\sf,  \coef)$ and $T(x)u_{\cdot}(\sf,  \coef)$ are bounded over a bounded support and hence sub-gaussian and from sub-gaussian concentration it follows: defining $z_{a, n}^{(1)} = (\Ex_{\bbQ_n} - \Ex_{\bbQ})[T(x)v_a(\sf,  \coef)]$,  $z_{a, m}^{(2)} = (\Ex_{\bbP_m} - \Ex_{\bbP})[T(x)u_a(\sf,  \coef)]$ and $z_{ m}^{(3)} = (\Ex_{\bbP_m} - \Ex_{\bbP})[T(x)u_{\cdot}(\sf,  \coef)]$ there exists constants $c_3, c_4, c_5>0$ such that for any $\delta > 0$ it holds:
%     \[
%     \|z_{a, n}^{(1)}\|_2 \le c_3 \sqrt{\frac{ \log(1/\delta)}{n}}, ~ \|z_{a, m}^{(2)}\|_2 \le c_4 \sqrt{\frac{ \log(1/\delta)}{m}}, ~ |z_{a, m}^{(3)}| \le c_5 \sqrt{\frac{ \log(1/\delta)}{m}}
%     \] with probability at least $ 1- \delta$. We define the event as $\cE(\bA)$. 
% We notice in $\bA$ that 
% \[
% \begin{aligned}
% & \Ex_{\bbQ_n} [T(x)v_a(\sf,  \coef)] - \frac{\Ex_{\bbP_m}[T(x)u_a( \sf,  \coef)]}{\Ex_{\bbP_m}[u_{\cdot} ( \sf,  \coef)]}  \\
% & = \Ex_{\bbQ} [T(x)v_a(\sf,  \coef)] + z_{a, n}^{(1)} - \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] + z_{a, m}^{(2)}}{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]+ z_{a, m}^{(3)}}\\
% & = \Ex_{\bbQ} [T(x)v_a(\sf,  \coef)]  - \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] }{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]} \\
% & ~~ + z_{a, n}^{(1)}+ \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] }{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]} -  \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] + z_{a, m}^{(2)}}{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]+ z_{a, m}^{(3)}}
% \end{aligned}
% \] where we notice that 
% \[
% \begin{aligned}
% & \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] }{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]} -  \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] + z_{a, m}^{(2)}}{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]+ z_{a, m}^{(3)}} \\
% & = \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] z_{a, m}^{(3)} - \Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]z_{a, m}^{(2)} }{\{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]\}\{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]+ z_{a, m}^{(3)}\}}\,.
% \end{aligned}
% \] On the event $\cE(\bA)$ we notice that $ \|z_{a, n}^{(1)}\|_2 \le c_3 \sqrt{\frac{ \log(1/\delta)}{n}}$ and since  $\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)] = 1$ (which we establish in Lemma \ref{lemma:true-normalization}) we further notice that 
% \[
% \begin{aligned}
% & \left \|\frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] z_{a, m}^{(3)} - \Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]z_{a, m}^{(2)} }{\{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]\}\{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]+ z_{a, m}^{(3)}\}} \right\|_2 \\
% & \le \frac{\|\Ex_{\bbP}[T(x)u_a( \sf,  \coef)]\|_2 |z_{a, m}^{(3)}|+  \|z_{a, m}^{(2)}\|_2 }{\kappa (\kappa - |z_{a, m}^{(3)}|)}\\
% & \le \frac{c_6  c_5 \sqrt{\frac{ \log(1/\delta)}{m}}+  c_4 \sqrt{\frac{ \log(1/\delta)}{m}} }{\kappa^2 - c_5 \kappa \sqrt{\frac{ \log(1/\delta)}{m}}}\\
% & \le 2c_6  c_5 \kappa^{-2} \sqrt{\frac{ \log(1/\delta)}{m}}+  2c_4\kappa^{-2} \sqrt{\frac{ \log(1/\delta)}{m}}
% \end{aligned}
% \] where for some $c_6>0$ we have  $\|\Ex_{\bbP}[T(x)u_a( \sf,  \coef)]\|_2 \le c_6$ and the inequality in the last line holds for sufficiently large $m$ since $c_5 \sqrt{\frac{ \log(1/\delta)}{m}} \le \frac\kappa 2$ for sufficiently large $m$. We now see that 
% \[
% \bA = \Ex_{\bbQ} [T(x)v_a(\sf,  \coef)]  - \frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] }{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]} + z_{a, m, n}(\coef)
% \] where For sufficiently large $m$  on the event $\cE(\bA)$ it holds:
% \[
% \begin{aligned}
% \|z_{a, m, n}(\coef)\|_2 &\le \|z_{a, n}^{(1)}\|_2 + \left \|\frac{\Ex_{\bbP}[T(x)u_a( \sf,  \coef)] z_{a, m}^{(3)} - \Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]z_{a, m}^{(2)} }{\{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]\}\{\Ex_{\bbP}[u_{\cdot} ( \sf,  \coef)]+ z_{a, m}^{(3)}\}} \right\|_2\\
% &\le c_3 \sqrt{\frac{ \log(1/\delta)}{n}} + 2c_6 c_5\kappa^{-2} \sqrt{\frac{ \log(1/\delta)}{m}}+  2c_4\kappa^{-2} \sqrt{\frac{ \log(1/\delta)}{m}}\\
% & \le c_7 \Big\{\sqrt{\frac{ \log(1/\delta)}{m}} + \sqrt{\frac{ \log(1/\delta)}{n}}\Big\}
% \end{aligned}
% \] for some $c_7>0$. Noticing that $z_{a, m, n}(\coef)$ is a Lipschitz function on $\coef \in B(0, \|\scoef\|_2 + 1)$ we see from Lemma ?? that there exists a $c_8>0$ such that  with probability at least $1 - \delta$ the following holds:
% \[
% \|Z_{a, m, n}\|_2 \le c_8\Big\{\sqrt{\frac{ \log(1/\delta)}{m}} + \sqrt{\frac{ \log(1/\delta)}{n}}\Big\}
% \]



Returning to the first order optimality condition \eqref{eq:optimality-theta-hat} for estimating $\hcoef$ 
we notice that 
\[
\begin{aligned}
 0 & = \textstyle\sum_{a} (\hcoef_a - \scoef_a)^\top \big\{\partial_{\coef_a} \hL (\sf, \hcoef) + \langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\}\\
 & = \textstyle\sum_{a} (\hcoef_a - \scoef_a)^\top \partial_{\coef_a} \sL (\sf, \hcoef) + \sum_{a} (\hcoef_a - \scoef_a)^\top  \big\{Z_{a, n_P, n_Q}(\hcoef) + \langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\}\\
 & = \textstyle(\hcoef - \scoef) ^\top \partial_{\coef} \sL (\sf, \hcoef) + \sum_{a} (\hcoef_a - \scoef_a)^\top  \big\{Z_{a, n_P, n_Q}(\hcoef) + \langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\}
\end{aligned}
\]


We combine it with the first ordder optimality condition for $\scoef$ \eqref{eq:optimality-truth}
to obtain 
\[
\begin{aligned}
(\hcoef - \scoef) ^\top \big\{\partial_{\coef} \sL (\sf, \hcoef) - \partial_{\coef} \sL (\sf, \scoef)\big\}\\
+ \textstyle\sum_{a} (\hcoef_a - \scoef_a)^\top  \big\{Z_{a, n_P, n_Q}(\hcoef) + \langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\} = 0
\end{aligned}
\]
which can be rewritten as 
\begin{equation} \label{eq:eqA.24}
  \textstyle  (\hcoef - \scoef) ^\top \big\{\partial_{\coef} \sL (\sf, \hcoef) - \partial_{\coef} \sL (\sf, \scoef)\big\} = - \sum_{a} (\hcoef_a - \scoef_a)^\top  \big\{Z_{a, n_P, n_Q}(\hcoef) + \langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\}\,.
\end{equation} Using the strong convexity assumption at $\scoef$ we obtain that the left hand side in the above equation is lower bounded as 
\begin{equation} \label{eq:lhs}
    (\hcoef - \scoef) ^\top \big\{\partial_{\coef} \sL (\sf, \hcoef) - \partial_{\coef} \sL (\sf, \scoef)\big\} \ge \strongconvexity \|\hcoef - \scoef\|_2^2 \,.
\end{equation}

Let $\cE$ be the event on which the following hold:
\begin{enumerate}
    \item $\|\hcoef - \scoef\|_2 \le \delta_\coef$, 
    \item $|\langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL(\tilde  f, \hat  \coef)\rangle| \le \sqrt{K}c_1c_2 r_{n_P} \sqrt{\log(n_Q)\log\{1/\delta\}}$ for all $a$, 
    \item $Z_{a, n_P, n_Q} \le c_7\Big\{\sqrt{\frac{ K(p+1) \log(1/\delta)}{n_P}} + \sqrt{\frac{K(p+1) \log(1/\delta)}{n_Q}}\Big\}$ for all $a$. 
\end{enumerate}
We notice that the event $\cE$ has probability $1 - (2 K + 1)\delta$. 
Under the event there exists a  $c_9>0$ such that  the right hand side in \eqref{eq:eqA.24} is upper bounded as 
\begin{equation} \label{eq:rhs}
    \begin{aligned}
& \textstyle\left | - \sum_{a} (\hcoef_a - \scoef_a)^\top  \big\{Z_{a, n_P, n_Q}(\hcoef) + \langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\}\right|\\
& \le \textstyle\sum_{a} \|\hcoef_a - \scoef_a\|_2 \Big\{\|Z_{a, n_P, n_Q}(\hcoef)\|_2 + \big\|\langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\|_2 \Big\}\\
& \le\textstyle \sum_{a} \|\hcoef_a - \scoef_a\|_2 \Big\{Z_{a, n_P, n_Q} + \big\|\langle \hf - \sf, \partial_{f} \partial_{\coef_a} \hL( \tf, \hcoef)\rangle\big\|_2 \Big\}\\
& \le \textstyle \sum_{a} \|\hcoef_a - \scoef_a\|_2 c_{9}  \Big\{r_{n_P} \sqrt{\log(n_Q)\log\{1/\delta\}} + \sqrt{\frac{ K(p+1)\log(1/\delta)}{n_P}} + \sqrt{\frac{K(p+1) \log(1/\delta)}{n_Q}}\Big\} \\
& \le \textstyle c_{9}  \Big\{r_{n_P} \sqrt{\log\{n_Q/\delta\}} + \sqrt{\frac{ K(p+1)\log(1/\delta)}{n_P}} + \sqrt{\frac{K(p+1) \log(1/\delta)}{n_Q}}\Big\} \sqrt{K} \|\hcoef - \scoef\|_2 
\end{aligned}
\end{equation}
 Combining the bounds \eqref{eq:lhs} and \eqref{eq:rhs} for left and right hand sides we obtain a $c_{10}>0$ such that on the event $\cE$ it holds 
 \[\textstyle\|\hcoef - \scoef\|_2 \le c_{10}\Big\{r_{n_P} \sqrt{\log(n_Q)\log\{1/\delta\}} + \sqrt{\frac{K(p+1) \log(1/\delta)}{n_P}} + \sqrt{\frac{K(p+1) \log(1/\delta)}{n_Q}}\Big\}\,. \]
 
 Having a concentration on $\hcoef$ we now notice that \[
 \begin{aligned}
 & \|\hat \weight - \weight^\star\|_{1, P} \\
 & = \textstyle\int \big|\exp(\hcoef_y^\top S(x)) - \exp({\scoef_y}^\top S(x))\big| p_X(x)dx\\
 & = \textstyle\int |(\hcoef_y - \scoef_y)^\top S(x)| \exp(\coef_x) p_X(x)dx
 \end{aligned}
 \]
 where $\coef_x$ is a number between $\hcoef_y^\top S(x)$ and ${\scoef_y}^\top S(x)$. On the event $\cE$ we notice that $\|\hcoef\|_2 \le \|\scoef\|_2 + \delta_\coef$ and hence it holds: $|\hcoef_y^\top S(x)|\le \|\hcoef_y\|_2 \|S(x)\|_2 \le \|\hcoef\|_2 \|S(x)\|_2 \le c_1 (\|\scoef\|_2 + \delta_\coef)$. Furthermore, we notice that $|{\scoef_y}^\top S(x)|\le \|\scoef\|_2 \|S(x)\|_2 \le c_1\|\scoef\|_2$, which implies $|\coef_x| \le c_1 (\|\scoef\|_2 + \delta_\coef)$. Returning to the integral we obtain that on the event $\cE$ it holds: 
 \[
 \begin{aligned}
 &\textstyle \int |(\hcoef_y - \scoef_y)^\top S(x)| \exp(\coef_x) p_X(x)dx\\
 & \le\textstyle \|\hcoef_y - \scoef_y\|_2 \int \|S(x)\|_2\exp\{c_1 (\|\scoef\|_2 + \delta_\coef)\} p_X(x)dx \\
 & \le \|\hcoef - \scoef\|_2 c_1 \exp\{c_1 (\|\scoef\|_2 + \delta_\coef)\}\\
 & \le\textstyle c_{11}\Big\{r_{n_P} \sqrt{\log(n_Q)\log\{1/\delta\}} + \sqrt{\frac{K(p+1) \log(1/\delta)}{n_P}} + \sqrt{\frac{K(p+1) \log(1/\delta)}{n_Q}}\Big\}
 \end{aligned}
 \] for some $c_{11}>0$, which holds with probability at least $ 1- (2K + 1)\delta$. 

\begin{lemma}
\label{lemma:lb-normalizer}
There exists $\delta_\xi>0$ such that \[
\inf_{\coef: \|\coef \|_2 \le \|\scoef\|_2 + \delta_\coef} \Ex_{P}[\exp( \coef_y ^\top S(x))] \ge \frac 12\,.
\]
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:lb-normalizer}]
  To establish a bound on $\Ex_{P}[\exp( \coef_y ^\top S(x))] - \Ex_{P}[\exp( {\scoef_y} ^\top S(x))]$ for any $\|\coef - \scoef\|_2 \le \delta_\coef$ we notice that \[
 \begin{aligned}
 & |\Ex_{P}[\exp( \coef_y ^\top S(x))] - \Ex_{P}[\exp( {\scoef_y} ^\top S(x))]| \\
 & = \textstyle\int \big|\exp(\coef_y^\top S(x)) - \exp({\scoef_y}^\top S(x))\big| p_X(x)dx\\
 & = \textstyle\int |(\coef_y - \scoef_y)^\top S(x)| \exp(\coef_x) p_X(x)dx
 \end{aligned}
 \]
 where $\coef_x$ is a number between $\coef_y^\top S(x)$ and ${\scoef_y}^\top S(x)$. We notice that $\|\coef\|_2 \le \|\scoef\|_2 + \delta_\coef$ and hence it holds: $|\coef_y^\top S(x)|\le \|\coef_y\|_2 \|S(x)\|_2 \le \|\coef\|_2 \|S(x)\|_2 \le c_1 (\|\scoef\|_2 + \delta_\coef)$. Furthermore, we notice that $|{\scoef_y}^\top S(x)|\le \|\scoef\|_2 \|S(x)\|_2 \le c_1\|\scoef\|_2$, which implies $|\coef_x| \le c_1 (\|\scoef\|_2 + \delta_\coef)$. Returning to the integral we obtain 
 \[
 \begin{aligned}
 &\textstyle \int |(\coef_y - \scoef_y)^\top S(x)| \exp(\coef_x) p_X(x)dx\\
 & \le\textstyle \|\coef_y - \scoef_y\|_2 \int \|S(x)\|_2\exp\{c_1 (\|\coef\|_2 + \delta_\coef)\} p_X(x)dx \\
 & \le \delta_\coef c_1 \exp\{c_1 (\|\scoef\|_2 + \delta_\coef)\}\,.
 \end{aligned}
 \] We choose $\delta_\coef>0$ small enough such that $\delta_\coef c_1 \exp\{c_1 (\|\scoef\|_2 + \delta_\coef)\} \le 1/2$.  Since $\Ex_{P}[\exp( {\scoef_y} ^\top S(x))] = 1$ we obtain that for any $\coef$ with $\|\coef - \scoef\|_2 \le 1/2$ we have 
 \[
 \begin{aligned}
 \textstyle\Ex_{P}[\exp( \coef_y ^\top S(x))] \ge \Ex_{P}[\exp( {\scoef_y} ^\top S(x))] - |\Ex_{P}[\exp( \coef_y ^\top S(x))] - \Ex_{P}[\exp( {\scoef_y} ^\top S(x))]| \ge \frac 12\,.
 \end{aligned}
 \] This implies the lemma.

\end{proof}

\begin{lemma}[Derivatives] \label{lemma:derivatives}
The following holds:
\begin{enumerate}
    \item $\partial_{\theta_b} u_a(f, \theta) = T(x)u_a(f, \theta) \delta_{a,b}$, $\partial_{\theta_b} u_{\cdot}(f, \theta) = T(x)u_b(f, \theta) $ and $\partial_{\theta_b} v_a(f, \theta) = T(x)v_a(f, \theta)\{\delta_{a, b} - v_b(f, \theta)\}$. 
    \item $\partial_{f_b} \eta_a = \eta_a (\delta_{a, b} - \eta_b)$, $\partial_{f_b} \{u_a(f, \theta)\} = (\delta_{a, b} - \eta_b)u_a(f, \theta)$, $\partial_{f_b} \{u_{\cdot}(f, \theta)\} = u_b(f, \theta) - \eta_b u_{\cdot}(f, \theta)$ and $\partial_{f_b} \{v_a(f, \theta)\} = v_a(f, \theta) (\delta_{a, b} - v_b(f, \theta))$. 
\end{enumerate}
\end{lemma}

\begin{proof}[Proof of lemma \ref{lemma:derivatives}]
We calculate the derivatives one by one. 
\paragraph{1:} We notice that 
\[
\begin{aligned}
\partial_{\theta_b} u_a(f, \theta)  &= \partial_{\theta_b} \{\eta_a(x) \exp(\theta_a^\top T(x))\}\\
& = \eta_a(x) \exp(\theta_a^\top T(x)) T(x) \delta_{a, b} = T(x)u_a(f, \theta) \delta_{a,b}
\end{aligned}
\] and that 
\[
\textstyle\partial_{\theta_b} u_{\cdot}(f, \theta) = \sum_{a = 1}^K T(x)u_a(f, \theta) \delta_{a,b} = T(x)u_b(f, \theta)
\] which finally implies
\[
\begin{aligned}
\partial_{\theta_b} v_a(f, \theta) &=\textstyle \frac{\partial_{\theta_b} \{u_a(f, \theta)\} u_{\cdot }(f, \theta) - \partial_{\theta_b} \{u_{\cdot}(f, \theta)\} u_{a }(f, \theta) }{\{u_{\cdot} (f, \theta)\}^2}\\
& =\textstyle \frac{T(x)u_a(f, \theta) \delta_{a,b} u_{\cdot }(f, \theta) - T(x)u_b(f, \theta) u_{a }(f, \theta) }{\{u_{\cdot} (f, \theta)\}^2}\\
& = T(x) \{u_a / u_{\cdot}\} \{\delta_{a, b} - u_a / u_{\cdot}\} = T(x) v_a (\delta_{a, b} - v_a)
\end{aligned}
\]

\paragraph{2:} Here \[
\begin{aligned}
\partial_{f_b} \eta_a  = \textstyle\partial_{f_b} \left\{\frac{e^{f_a}}{\sum_{j} e^{f_j}} \right\} = \textstyle\frac{\delta_{a, b} e^{f_a}\sum_{j} e^{f_j} - e^{f_a} e^{f_b} }{\Big\{\sum_{j} e^{f_j}\Big\}^2} = \eta_a (\delta_{a, b} -\eta_b)\,,
\end{aligned}
\] 
\[
\begin{aligned}
\partial_{f_b} \{u_a(f, \theta)\} & = \partial_{f_b} \{\eta_a\} \exp(\theta_a^\top T(x)) \\
& = \eta_a (\delta_{a, b} -\eta_b)\exp(\theta_a^\top T(x)) = (\delta_{a, b} -\eta_b)u_a(f, \theta)\,,
\end{aligned}
\]
\[ \textstyle
\partial_{f_b} \{u_{\cdot}(f, \theta)\}  = \sum_{a} (\delta_{a, b} -\eta_b)u_a(f, \theta) = u_{b}(f, \theta) - \eta_b u_{\cdot}(f, \theta)
\] and finally,
\[
\begin{aligned}
\partial_{f_b} \{v_a(f, \theta)\} & = \frac{ \{\partial_{f_b} u_a(f, \theta)\} u_{\cdot}(f, \theta) -  \{\partial_{f_b} u_{\cdot}(f, \theta)\} u_{a}(f, \theta) }{\{u_{\cdot}(f, \theta)\}^2}\\
& = \frac{ (\delta_{a, b} -\eta_b)u_a(f, \theta) u_{\cdot}(f, \theta) -  \{u_{b}(f, \theta) - \eta_b u_{\cdot}(f, \theta)\} u_{a}(f, \theta) }{\{u_{\cdot}(f, \theta)\}^2}\\
& = (u_a / u_{\cdot}) \{ \delta_{a, b} u_{\cdot} - \cancel{\eta_b u_{\cdot}} - u_a  +\cancel{\eta_b u_{\cdot}}  \}/ u_{\cdot}\\
& =  (u_a / u_{\cdot}) \{ \delta_{a, b}  - (u_a/u_{\cdot})   \} = v_a \{ \delta_{a, b} - v_a \}
\end{aligned}
\]
\end{proof}


% \begin{lemma}\label{lemma:sup-convergence}
% Let $X_1, \dots, X_n \in \cX$ are \IID\ random vectors from distribution $P$. For a function $f : \cX \times \reals^d$ let $beta \mapsto f(\dots, \beta)$ be a Lipschitz function, \ie\ there exists an $L>0$ such that for any $\beta_1, \beta_2 \in \reals^d$
% \[\textstyle
% \sup_{x\in \cX} |f(x, \beta_1) - f(x, \beta_2)| \le L \|\beta_1 - \beta_2 \|_2 \,.
% \] Then for any $M>0$ there exist a $c_M>0$ such that for any $\delta>0$ with probability at least $1 - \delta$ it holds
% \[\textstyle
% \sup_{\|\beta\|_2 \le M}\big|\Ex_{\hP}[f(X, \beta)] - \Ex_{P}[f(X, \beta)] \big| \le c_M \sqrt{\frac{d\log(1/\delta)}{n}}\,.
% \]
% \end{lemma}

% \begin{proof}[Proof of Lemma \ref{lemma:sup-convergence}]
% Without loss of generality assume that $\Ex_{P}[f(X, \beta)] = 0$. 
% Let $\cN$ be a $1/2$-net  of  $B(0, M)$ a ball of radius $M$ with respect to $\|\cdot \|_2$-norm which satisfy $|\cN | \le (5M)^d$ (see \cite[Lemma 7.6]{duchi2016lecture}). Then for any $\beta \in \cS^{d-1}$ there exists  a $\beta'$ such that $\|\beta - \beta'\|_2 \le 1/2$ and the following holds: 
% \[
% \begin{aligned}
% |E_{\hP}[f(X, \beta)] | &=  |E_{\hP}[f(X, \beta')] + E_{\hP}[f(X, \beta) - f(X, \beta')] |\\
% &\le |E_{\hP}[f(X, \beta')] | + L\| {\beta - \beta'} \|_2
% &\le |{\coef'} ^\top x | + \frac{\| x \|_2}2
% \end{aligned}
% \] We take a supremum over $\theta \in \cS^{d-1}$ on the left side and over $\theta'\in \cN$ on the right side and obtain 
% \[
% \begin{aligned}
% &  \|x \|_2 = \sup_{\theta \in \cS^{d-1}}  |\coef ^\top x | \le \sup_{\theta'\in \cN}  |{\coef'} ^\top x | + \frac{\| x \|_2}2
% & \text{or, } \frac{\| x \|_2}2 \le \sup_{\theta'\in \cN}  |{\coef'} ^\top x |\,.
% \end{aligned}
% \] Now \[
% \begin{aligned}
% \Pr(\|x\|_2 > t) & \le \Pr \big( 2 \sup_{\theta'\in \cN}  |{\coef'} ^\top x |>t \big)\\
% & \le \sum_{\theta'\in \cN} \Pr(|{\coef'} ^\top x | > t/2) \\
% & \le 5^d e^{- t^2 / (4\zeta^2)} \\
% & \le e^{- \frac{t^2 - cd}{4\zeta^2}}
% \end{aligned}
% \] for some  $c> 0$ which is independent of $d$. Noticing that $t^2 - cd \ge \frac{t^2}{d}$ holds for any $ t > \frac{\sqrt{c}d}{\sqrt{d-1}}$ we now have 
% \[
% \begin{aligned}
% & \Pr(\|x\|_2 > t)  \le e^{- \frac{t^2 }{4d\zeta^2}}, ~ t > \frac{\sqrt{c}d}{\sqrt{d-1}}\\
%  \text{or, } & \Pr(\|x\|_2 > t) \le e^{- \frac{t^2 }{4d\zeta^2}}, ~ t >  \sqrt{cd}\\
%  \text{or, } & \Pr(\|x\|_2 > t) \le e^{\frac{c}{4\zeta^2} }e^{- \frac{t^2 }{4d\zeta^2}}, ~ t >  0
% \end{aligned}
% \] where the last one holds because $e^{- \frac{t^2 }{4d\zeta^2}} \le e^{\frac{c}{4\zeta^2} }e^{- \frac{t^2 }{4d\zeta^2}}$ for $t > \sqrt{cd}$ and $e^{\frac{c}{4\zeta^2} }e^{- \frac{t^2 }{4d\zeta^2}} \ge  1$ for $t \le \sqrt{cd}$. 

% \end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% PROOF OF UNIQUENESS %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{proof}[Proof of Lemma \ref{lemma:uniqueness}]
% We notice that 
% \[
% \textstyle 
% \sum_{k = 1}^K \eta_{P, k}^\star(x) \exp\{{\coef_k}^\top S(x)\} = \sum_{k = 1}^K \frac{p\{x, Y = k\}}{p_X(x)} \exp\{{\coef_k}^\top S(x)\} 
% \] which implies 
% \[
% \begin{aligned}
% & \klloss(\eta_P^\star, \coef)\\
% & =  \Ex_{Q_X}[\log \{ \sum_{k = 1}^K \frac{p\{x, Y = k\}}{p_X(x)} \exp\{{\coef_k}^\top S(x)\}  \}] - \log [\Ex_{P_X} \{ \sum_{k = 1}^K \frac{p\{x, Y = k\}}{p_X(x)} \exp\{{\coef_k}^\top S(x)\}  \}]\\
% & =  \Ex_{Q_X}[\log \{ \sum_{k = 1}^K \frac{p\{x, Y = k\}}{p_X(x)} \exp\{{\coef_k}^\top S(x)\}  \}] - \log [\int  \{ \sum_{k = 1}^K p\{x, Y = k\} \exp\{{\coef_k}^\top S(x)\} dx  \}] \\
% & = \Ex_{Q_X} \left[\log \left\{\frac{\sum_{k = 1}^K p\{x, Y = k\} \exp\{{\coef_k}^\top S(x)}{\int  \{ \sum_{k = 1}^K p\{x, Y = k\} \exp\{{\coef_k}^\top S(x)\} dx}\right\}\right] - \Ex_{Q_X}[\log p_X(x)]
% \end{aligned}
% \] and 
% \[ \textstyle
% \klloss(\eta_P^\star, \scoef)
%  = \Ex_{Q_X}[\log(q_X(x))] - \Ex_{Q_X}[\log(p_X(x))]
% \] which implies 

% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% PROOF OF GENERALIZATION %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Lemma \ref{lemma:generalization-bound}}

We start by decomposing the loss difference in the left hand side of equation \eqref{eq:gen-bound}. 
\begin{equation}
    \begin{aligned}
    \cL_Q(\hat f_{\hat \weight}) - \cL_Q(f^\star) = \cL_P(\hat f, \weight^\star) - \cL_P(f^\star, \weight^\star)\\
    = \textstyle\underbrace{\cL_P(\hat f, \weight^\star) - \cL_{\hP}(\hat f, \weight^\star)}_{(a)} + \underbrace{\cL_{\hP}(\hat f, \weight^\star) - \cL_{\hP}(\hat f, \hat \weight)}_{(b)} + \underbrace{\cL_{\hP}(\hat f, \hat \weight) - \cL_{\hP}( f^*, \hat \weight)}_{\le 0}\\
    \textstyle + \underbrace{\cL_{\hP}( f^*, \hat \weight) - \cL_{\hP}( f^*,  \weight^\star)}_{(c)} + \underbrace{\cL_{\hP}( f^*,  \weight^\star) - \cL_P( f^*,  \weight^\star)}_{(d)}\,,
    \end{aligned}
\end{equation} where we write $\hat f_{\hat \weight} \equiv \hat f$. 

\paragraph{Uniform bound on (a)} To control (a) in \eqref{eq:gen-bound} we establish a concentration bound on the following generalization error
\[
\begin{aligned}
\sup_{f \in \cF} \big\{ \cL_P( f, \weight^\star) - \cL_{\hP}( f, \weight^\star) \big\} \\
=\textstyle \sup_{f \in \cF} \Big\{ \Ex\big[g_f(X, Y)\big] -\frac1 {\nsource} \sum_{i = 1}^{\nsource} g_f(X_{P, i}, Y_{P, i}) \Big\}
\triangleq F(z_{1:\nsource})\,,
\end{aligned}
\] where, for $i \ge 1$ we denote $z_{1:i} = (z_1, \dots, z_i)$ and  $z_i = (X_{P, i}, Y_{P, i})$.  First, we use a modification of McDiarmid concentration inequality to bound $F(z_{1:\nsource})$
in terms of its expectation and a $O(1/\sqrt{\nsource})$ term, as elucidated in the following lemma. 
\begin{lemma}
\label{lemma:mcdiarmid}
There exists a constant $c_1>0$ such that with probability at least $1-\delta$ the following holds
\begin{equation}
\label{eq:conc-mcdirmid}
  \textstyle  F(z_{1:\nsource}) \le \Ex\big[F(z_{1:\nsource})\big] + c_1\sqrt{\frac{\log(1/\delta)}{\nsource}}\,.
\end{equation}
\end{lemma}
Next, we use a symmetrization argument (see \cite[Chapter 2, Lemma 2.3.1]{wellner2013weak} ) to bound the expectation $\Ex\big[F(z_{1:\nsource})\big]$ by the Rademacher complexity of the hypothesis class $\cG$, \ie, 
\begin{equation}
\label{eq:symmetrization}
    \Ex\big[F(z_{1:\nsource})\big] \le 2 \cR_{\nsource} (\cG)\,.
\end{equation}
Combining \eqref{eq:conc-mcdirmid} and \eqref{eq:symmetrization} we obtain
\begin{equation}
  \textstyle  (a) = \cL_P(\hat f, \weight^\star) - \cL_{\hP}(\hat f, \weight^\star) \le 2 \cR_{\nsource}(\cG) +   c_1\sqrt{\frac{\log(1/\delta)}{\nsource}}\,,\label{eq:bound-a}
\end{equation} with probability at least $ 1- \delta$. 

\paragraph{Bound on (b) and (c)} Denoting $z_i = (X_{P, i}, Y_{P, i})$ and $\ell_f(z_i) = \ell(f(X_{P,i}), Y_{P, i})$ we  notice that 
for any $f\in \cF$ we have 
\[
\begin{aligned}
  \textstyle ~~\big|\cL_{\hP}( f, \weight^\star) - \cL_{\hP}( f, \hat \weight)\big|
  & = \textstyle\Big|\frac1{\nsource}\sum_{i = 1}^{\nsource}\big\{ \hat \weight(z_i) - \weight^\star (z_i) \big\} \ell_f(z_i)\Big|\\
  & \le\textstyle \frac1{\nsource}\sum_{i = 1}^{\nsource}\big|\big\{ \hat \weight(z_i) - \weight^\star (z_i) \big\} \ell_f(z_i)\big| \le\textstyle \frac{\|\ell\|_\infty}{\nsource}\sum_{i = 1}^{\nsource}\big| \hat \weight(z_i) - \weight^\star (z_i) \big|\,.
\end{aligned}
\] Since $\hat \weight(z) - \weight^\star (z)$ is a sub-gaussian random variable, we use sub-gaussian concentration to establish that for some constant $c_2>0$ \begin{equation}
  \textstyle  \text{for any }f \in \cF, ~~\big|\cL_{\hP}( f, \weight^\star) - \cL_{\hP}( f, \hat \weight)\big| \le \|\ell\|_\infty \Big\{ \Ex_{z_1}\big[|\hat w(z_1) - w^\star (z_1)|\big] + c_2 \sqrt{\frac{\log(1/\delta)}{\nsource}} \Big\} \label{eq:bound-bc}
\end{equation}
 with probability at least $1 - \delta$. This provides a simultaneous bound (on the same probability event) for both (b) and (c) with $f = \hat f$ and $f = f^\star$. 

\paragraph{Bound on (d)} We note that 
\[
\begin{aligned}
 \textstyle ~~ \cL_{\hP}( f^*,  \weight^\star) - \cL_P( f^*,  \weight^\star) = \frac{1}{\nsource}\sum_{i = 1}^{\nsource} \weight^\star (z_i) \ell_{f^\star} (z_i) - \Ex_P\big\{\weight^\star (z_1) \ell_{f^\star} (z_1)\big\}\,,
\end{aligned}
\] where $\{\weight^\star (z_i) \ell_{f^\star} (z_i)\}_{i = 1}^{\nsource}$ are \IID\ sub-gaussian random variables. Using Hoeffding concentration bound we conclude that there exists a constant $c_3>0$ such that for any $\delta>0$ the following holds with probability at least $1 - \delta$
\begin{equation}
\label{eq:bound-d}
 \textstyle   \frac{1}{\nsource}\sum_{i = 1}^{\nsource} \weight^\star (z_i) \ell_{f^\star} (z_i) - \Ex_P\big\{\weight^\star (z_1) \ell_{f^\star} (z_1)\big\} \le c_3 \sqrt{\frac{\log(1/\delta)}{\nsource}}\,.
\end{equation} 
Finally, using \eqref{eq:bound-a} on (a) (which is true on an event of probability $\ge 1 - \delta$), \eqref{eq:bound-bc} on (b) and (c) (simultaneously true on an event of probability $\ge 1- \delta$), and \eqref{eq:bound-d} on (d) (holds on an event of probability $\ge 1- \delta$) we conclude that with probability at least $1 - 3\delta$ the following holds
\begin{equation}
   \textstyle \cL_Q(\hat f_{\hat w}) -  \cL_Q(f^\star) \le  2 \cR_n(\cG) + \|\ell\|_\infty \cdot \Ex_{z_1}\big[|\hat \weight(z_1) - \weight^\star (z_1)|\big] + c_4 \sqrt{\frac{\log(1/\delta)}{\nsource}} 
\end{equation} where $c_4 = c_1 + \|\ell\|_\infty c_2 + c_3$. 



\begin{proof}[Proof of Lemma \ref{lemma:mcdiarmid}] For the simplicity of notations we drop the subscript from $\nsource$ and denote the sample size simply by $n$. 
For $i \le n$ we define $\Ex_{i:n}$ as the expectation with respect to the random variables $z_i, \dots, z_n$, and for $i > n$ we define $\Ex_{i:n}\big[F(z_{1:n})\big] = F(z_{1:n})$  and notice that
\begin{equation}
\label{eq:martingale-sum}
  \textstyle  F(z_{1:n}) - \Ex\big[F(z_{1:n})\big] = \sum_{i = 1}^{n} \Big\{ \Ex_{(i+1):n}\big[F(z_{1:n})\big] - \Ex_{{i:n}}\big[F(z_{1:n})\big] \Big\}\,.
\end{equation}
Here, 
\begin{equation}
\label{eq:martingale-diff}
    \begin{aligned}
& ~~ \Ex_{(i+1):n}\big[F(z_{1:n})\big] - \Ex_{{i:n}}\big[F(z_{1:n})\big]\\ 
& = \Ex_{(i+1):n} \Big\{F(z_{1:n}) - \Ex_{z_i}\big[F(z_{1:n})\big]\Big\}\\
& = \Ex_{(i+1):n} \Big\{F(z_1, \dots, z_{i-1}, z_i, z_{i+1}, \dots, z_n) - \Ex_{z_i'}\big[F(z_1, \dots, z_{i-1}, z_i', z_{i+1}, \dots, z_n)\big]\Big\}\\
& = \Ex_{(i+1):n} \Ex_{z_i'} \Big\{F(z_1, \dots, z_{i-1}, z_i, z_{i+1}, \dots, z_n) - F(z_1, \dots, z_{i-1}, z_i', z_{i+1}, \dots, z_n)\Big\}
\end{aligned}
\end{equation}
 where, $z_i'$ is an \IID\ copy of $z_i$. We notice that 
\begin{equation}
\label{eq:fluctuation-bound}
    \begin{aligned}
& ~~ F(z_1, \dots, z_{i-1}, z_i, z_{i+1}, \dots, z_n) - F(z_1, \dots, z_{i-1}, z_i', z_{i+1}, \dots, z_n) \\
& = \textstyle\sup_{f \in \cF} \Big\{ \Ex\big[g_f(z_1)\big] -\frac1 {n} \sum_{i = 1}^{n} g_f(z_i) \Big\}\\
& ~~~~~~~~- \sup_{f \in \cF} \Big\{ \Ex\big[g_f(z_1)\big] -\frac1 {n} \sum_{i = 1}^{n} g_f(z_i) +\frac 1n g_f(z_i') - \frac1n g_f(z_i) \Big\}\\
& \le \textstyle\sup_{f \in \cF} \Big\{ - \frac 1n g_f(z_i') + \frac1n g_f(z_i) \Big\}
\end{aligned}
\end{equation}
 where the last inequality is obtained by setting $A_f = \Ex\big[g_f(z_1)\big] -\frac1 {n} \sum_{i = 1}^{n} g_f(z_i)$ and $B_f = \frac 1n g_f(z_i') - \frac1n g_f(z_i)$ in the following stream of inequalities
\[
\begin{aligned}
 \sup_{f\in \cF} \{A_f\} - \sup_{f\in \cF} \{A_f+ B_f\} 
& = \textstyle\sup_{f\in \cF} \{A_f+B_f - B_f\} - \sup_{f\in \cF} \{A_f+ B_f\} \\
& \le \textstyle\sup_{f\in \cF} \{A_f+B_f\} + \sup_{f\in \cF} \{-B_f\} - \sup_{f\in \cF} \{A_f+ B_f\}\\
& = \sup_{f\in \cF} \{-B_f\}\,,
\end{aligned}
\]
and that 
\begin{equation}
\label{eq:sup-diff-bound}
   \begin{aligned}
 \textstyle\sup_{f \in \cF} \Big\{ - \frac 1n g_f(z_i') + \frac1n g_f(z_i) \Big\}
& \textstyle\le \frac 1n \Big\{ \sup_{f \in \cF} |g_f(z'_i)| + \sup_{f \in \cF} |g_f(z_i)|\Big\}\\
& = \textstyle\frac 1n \Big\{ w^\star(z_i')\sup_{f \in \cF} |\ell(z_i')| + w^\star(z_i)\sup_{f \in \cF} |\ell(z_i')|\Big\}\\
& \le \textstyle\frac{\|\ell\|_\infty}{n}\big\{ w^\star(z_i') + w^\star(z_i)\big\}\,,
\end{aligned} 
\end{equation} where $\ell(z) = \ell(f(x), y)$. 
We use inequalities \eqref{eq:fluctuation-bound} and \eqref{eq:sup-diff-bound} in \eqref{eq:martingale-diff} and get the following
\begin{equation}
\label{eq:martingale-diff-ub}
\begin{aligned}
 \Ex_{(i+1):n}\big[F(z_{1:n})\big] - \Ex_{{i:n}}\big[F(z_{1:n})\big] &\le \frac{\|\ell\|_\infty}{n}\big\{ \Ex_{z_i'} [w^\star(z_i')] + w^\star(z_i)\big\}\,.
\end{aligned}
   \end{equation}
Now, we use \eqref{eq:martingale-sum} and \eqref{eq:martingale-diff-ub} to bound the moment generating function of $F(z_{1:n}) - \Ex[F(z_{1:n})]$ as seen in the following inequalities. For $\lambda > 0$
\begin{equation}
\label{eq:mgf-bound}
\begin{aligned}
  & ~~   \Ex\Big\{ \exp\Big(\lambda\big\{F(z_{1:n}) - \Ex[F(z_{1:n})]\big\}\Big)\Big\}\\
 & = \Ex\Big\{ \exp\Big(\lambda\sum_{i = 1}^n\big\{\Ex_{(i+1):n}\big[F(z_{1:n})\big] - \Ex_{{i:n}}\big[F(z_{1:n})\big]\big\}\Big)\Big\}\\
 & \le \Ex\Big\{ \exp\Big(\lambda\sum_{i = 1}^n\frac{\|\ell\|_\infty}{n}\big\{ \Ex [w^\star(z_i')] + w^\star(z_i)\big\}\Big)\Big\}\\
 & \le \Ex\Big\{ \exp\Big(\lambda\sum_{i = 1}^n\frac{\|\ell\|_\infty}{n}\big\{ w^\star(z_i')+ w^\star(z_i)\big\}\Big)\Big\}, ~~ \text{since} ~~ e^{\Ex\{X\}} \le \Ex\big\{e^X\big\}\\
 & =  \prod_{i = 1}^n\Ex\Big\{ \exp\Big(\frac{\lambda \|\ell\|_\infty}{n} w^\star(z_i)\Big)\Big\} \Ex\Big\{ \exp\Big(\frac{\lambda \|\ell\|_\infty}{n} w^\star(z_i')\Big)\Big\}\\
 & \le  \prod_{i = 1}^n \exp\Big(\frac{2c\lambda^2 \|\ell\|_\infty^2}{n^2} \Big) = \exp\Big( \frac{2c\lambda^2 \|\ell\|_\infty^2}{n} \Big)\,.
\end{aligned}
\end{equation} 
Following the bound on moment generating function in \eqref{eq:mgf-bound} we get 
\[
\begin{aligned}
  & ~~\Pr\big\{F(z_{1:n}) - \Ex[F(z_{1:n})] > t\big\}\\
  &\le e^{-\lambda t} \Ex\Big\{ \exp\Big(\lambda\big\{F(z_{1:n}) - \Ex[F(z_{1:n})]\big\}\Big)\Big\}\\
  & = \exp\Big(-\lambda t + \frac{2c\lambda^2 \|\ell\|_\infty^2}{n} \Big)\,,
\end{aligned}
\] where letting $\lambda = nt /(4c \|\ell\|_\infty^2)$ we obtain
\[
\Pr\big\{F(z_{1:n}) - \Ex[F(z_{1:n})] > t\big\} \le \exp \Big( -\frac{nt^2}{8c \|\ell\|_\infty^2} \Big)\,,
\] and letting $t = \|\ell\|_\infty\sqrt{8c\log(1/\delta)/n}$ we establish the lemma with $C = \|\ell\|_\infty \sqrt{8c}$.

\end{proof}

% \begin{proof}[Proof of Lemma \ref{lemma:convexity-at-truth}]
% We define the following functions:
% \begin{equation}\textstyle
% \begin{aligned}
%   A_k(\eta, \Theta; x) = [\eta(x)]_k \exp(\theta_k^\top T(x)), ~~
%   A(\eta, \Theta; x) = \sum_{k = 1}^K A_k(\eta, \Theta; x)\\
%   \Psi_k(\eta, \Theta; x) = \frac{A_k(\eta, \Theta; x)}{A(\eta, \Theta; x)}, ~~
%   \Psi(\eta, \Theta; x) = (\Psi_1(\eta, \Theta; x), \dots, \Psi_K(\eta, \Theta; x))^\top\\
%   A^\star_k(x) = A_k(\eta_P^\star, \Theta^\star; x), A^\star(x) = A(\eta_P^\star, \Theta^\star; x), \Psi_k^\star(x) = \Psi_k(\eta_P^\star, \Theta^\star; x), \Psi^\star(x) = \Psi(\eta_P^\star, \Theta^\star; x)
% \end{aligned}
% \end{equation} and notice that 
% $\klloss(\eta, \Theta, \mu) = \Ex_{\mu} \big[\log\{A(\eta, \Theta; x)\}\big] - \log\big\{ \Ex_{\bbP_X} [A(\eta, \Theta; x)] \big\}$ and $d\bbQ_x = A^\star(x) d \bbP_x$. The first and second order partial derivatives of the loss are
% \begin{equation}
%     \begin{aligned}
%       \partial_{\theta_k} \klloss(\eta, \Theta, \mu) = \Ex_{\mu}\Big[ \frac{T(x) A_k(\eta, \Theta; x)}{A(\eta, \Theta; x)} \Big] - \frac{\Ex_{\bbP_x}[T(x) A_k(\eta, \Theta; x)]}{\Ex_{\bbP_x}[A(\eta, \Theta; x)]}\\
%       = \Ex_{\mu}\big[ T(x)\Psi_k(\eta, \Theta; x) \big] - \frac{\Ex_{\bbP_x}[T(x) A_k(\eta, \Theta; x)]}{\Ex_{\bbP_x}[A(\eta, \Theta; x)]}\,,\\
%       \partial_{\theta_k}\partial_{\theta_{k'}} \klloss(\eta, \Theta, \mu) = \Ex_{\mu}\big[ T(x)T(x)^\top\Psi_k(\eta, \Theta; x) \big\{\delta_{k = k'} -\Psi_k(\eta, \Theta; x) \big\} \big]\\
%       - \frac{\Ex_{\bbP_x} \big[ T(x)T(x)^\top A_k(\eta, \Theta; x) \big]}{\Ex_{\bbP_x} \big[  A(\eta, \Theta; x) \big]} \delta_{k = k'} \\
%       + \frac{\Ex_{\bbP_x} \big[ T(x) A_k(\eta, \Theta; x) \big] \Ex_{\bbP_x} \big[ T(x)^\top  A_{k'}(\eta, \Theta; x) \big]}{\big\{\Ex_{\bbP_x} \big[  A(\eta, \Theta; x) \big]\big\}^2}
%     \end{aligned}
% \end{equation} and for any $U = [u_1, \dots, u_K] \in \reals^{(d+1) \times K}$ we see that 
% \[\textstyle
% \begin{aligned}
%   &  \Vec(U) ^\top \nabla^2_{\Theta} \klloss(\eta_P^\star, \Theta^\star, \bbQ_x) \Vec(U) \\
%   & = \sum_{k, k' = 1}^{K} \Ex_{\bbQ_x}\big[ u_k^\top T(x)T(x)^\top u_{k'}\Psi_k(\eta_P^\star, \Theta^\star; x) \big\{\delta_{k = k'} -\Psi_k(\eta_P^\star, \Theta^\star; x) \big\} \big]\\
%   & ~~~ - \sum_{k, k' = 1}^{K} \frac{\Ex_{\bbP_x} \big[ u_k^\top T(x)T(x)^\top u_{k'} A_k(\eta_P^\star, \Theta^\star; x) \big]}{\Ex_{\bbP_x} \big[  A(\eta_P^\star, \Theta^\star; x) \big]} \delta_{k = k'} \\
%   & ~~~ + \sum_{k, k' = 1}^{K} \frac{\Ex_{\bbP_x} \big[ u_k^\top T(x) A_k(\eta_P^\star, \Theta^\star; x) \big] \Ex_{\bbP_x} \big[ T(x)^\top u_{k'}  A_{k'}(\eta_P^\star, \Theta^\star; x) \big]}{\big\{\Ex_{\bbP_x} \big[  A(\eta_P^\star, \Theta^\star; x) \big]\big\}^2}\\
%   & = \sum_{k = 1}^{K} \Ex_{\bbQ_x}\big[ \{u_k^\top T(x)\}^2\Psi_k^\star(x)  \big] - \Ex_{\bbQ_x}\Big[\Big\{\sum_{k = 1}^{K} u_k^\top T(x)\Psi_k^\star(x)  \Big\}^2\Big]\\
%   & ~~~ -  \frac{\sum_{k = 1}^K\Ex_{\bbP_x} \big[ \{u_k^\top T(x)\}^2 A_k^\star( x) \big]}{\Ex_{\bbP_x} \big[  A^\star( x) \big]}  + \Bigg\{ \frac{\sum_{k = 1}^{K}\Ex_{\bbP_x} \big[ u_k^\top T(x) A_k^\star( x) \big] }{\Ex_{\bbP_x} \big[  A^\star( x) \big]}\Bigg\}^2\\
%   & = \cancel{\sum_{k = 1}^{K} \Ex_{\bbP_x}\big[ \{u_k^\top T(x)\}^2 A_k^\star (x)  \big]} - \Ex_{\bbQ_x}\Big[\Big\{\sum_{k = 1}^{K} u_k^\top T(x)\Psi_k^\star(x)  \Big\}^2\Big]\\
%   & ~~~ -  \cancel{\sum_{k = 1}^K\Ex_{\bbP_x} \big[ \{u_k^\top T(x)\}^2 A_k^\star( x) \big]}  + \Big\{ \sum_{k = 1}^{K}\Ex_{\bbP_x} \big[ u_k^\top T(x) A_k^\star( x) \big] \Big\}^2\\
% & ~~~~~~~ \text{since} ~ \Psi_k^\star(x)d\bbQ_x = A_k^\star (x)d\bbP_x ~ \text{and} ~ \Ex_{\bbP_x}[A^\star(x)] = \Ex_{\bbQ_x}[1] = 1,\\
% & = - \Ex_{\bbP_x}\Big[\frac{1}{A^\star(x)}\Big\{\sum_{k = 1}^{K} u_k^\top T(x)A_k^\star(x)  \Big\}^2\Big] + \Big\{ \sum_{k = 1}^{K}\Ex_{\bbP_x} \big[ u_k^\top T(x) A_k^\star( x) \big] \Big\}^2\\
% & = - \Ex_{\bbQ_x}\Big[\frac{1}{A^\star(x)^2}\Big\{\sum_{k = 1}^{K} u_k^\top T(x)A_k^\star(x)  \Big\}^2\Big] + \Big\{ \sum_{k = 1}^{K}\Ex_{\bbP_x} \big[ u_k^\top T(x) A_k^\star( x)/A^\star(x) \big] \Big\}^2\\
% & = - \operatorname{var}_{\bbQ_x} \Big[\frac{1}{A^\star(x)}\sum_{k = 1}^{K} u_k^\top T(x)A_k^\star(x)  \Big]\\
% & = - \operatorname{var}_{\bbQ_x} \Big[\sum_{k = 1}^{K} u_k^\top T(x)\Psi_k^\star(x)  \Big] < 0
% \end{aligned}
% \] 

% \end{proof}






% \begin{lemma}
% \label{lemma:true-normalization}
% There exists a $\kappa>0$ such that 
% \[ \textstyle
% \inf_{\|\theta \|\le \|\stheta\|_2 + 1}\Ex_{\bbP}[u_{\cdot} ( \sf,  \theta)] \ge \kappa\,.
% \]
% \end{lemma}

% \begin{proof}[Proof of Lemma \ref{lemma:true-normalization}]
% Here we notice that 
% \[
% \begin{aligned}
% & \Ex_{\bbP}[u_{\cdot} ( \sf,  \theta)]\\
% & =  \Ex_{\bbP}\Big[\sum_{a}u_{a} ( \sf,  \theta)\Big]\\
% & = \Ex_{\bbP}\Big[\sum_{a}\eta_{P, a}^\star(x)\exp(\stheta^\top T(x))\Big]\\
% & = \Ex_{\bbP}\Big[\sum_{a}\frac{p\{Y = k, x\}}{p_X(x)}\exp(\stheta^\top T(x))\Big]\\
% & = \int \sum_a \frac{q\{Y = k, x\}}{p_X(x)} p_X(x)dx\\
% & = \int q_X(x)dx = 1
% \end{aligned}
% \]

% \end{proof}

==> exponential-tilt(ICLR2023)/sections/related-work.tex <==
\vspace{-0.4cm}
\section{Related work}



\textbf{Out-of-distribution generalization} is essential for safe deployment of ML models. There are two prevalent problem settings: domain generalization and subpopulation shift \citep{koh2020WILDS}. Domain generalization typically assumes access to several datasets during training that are related to the same task, but differ in their domain or environment \citep{blanchard2011Generalizing,muandet2013Domain}. The goal is to learn a predictor that can generalize to unseen related datasets via learning invariant representations \citep{ganin2016Domainadversarial,sun2016Deep}, invariant risk minimization \citep{arjovsky2019Invariant,krueger2021out}, or meta-learning \citep{dou2019Domain}.
Domain generalization is a very challenging problem and recent benchmark studies demonstrate that corresponding methods rarely improve over vanilla empirical risk minimization (ERM) on the source data unless given access to labeled target data for model selection \citep{gulrajani2020Search,koh2020WILDS}.

Subpopulation shift setting assumes that both train and test data consist of the same groups with different group fractions. This setting is typically approached via distributionally robust optimization (DRO) to maximize worst group performance \citep{duchi2016Statistics,sagawa2019Distributionally}, various reweighing strategies \citep{shimodaira2000Improving,byrd2019What,sagawa2020Investigation,idrissi2021simple}. These methods require group annotations which could be expensive to obtain in practice. Several methods were proposed to sidestep this limitation, however they still rely on a validation set with group annotations for model selection to obtain good performance \citep{hashimoto2018Fairness,liu2021Just,zhai2021DORO,creager2021Environment}. Our method is most appropriate for the subpopulation shift setting (see Section \ref{sec:exponential-tilt}), however it differs in that it does not require group annotations, but requires unlabeled target data.

\textbf{Model selection} on out-of-distribution (OOD) data is an important and challenging problem as noted by several authors \citep{gulrajani2020Search,koh2020WILDS,zhai2021DORO,creager2021Environment}.
\citet{xu2022estimation,chen2021mandoline} propose solutions specific to covariate shift based on parametric bootstrap and reweighing; \citet{garg2022leveraging,guillory2021predicting,yu2022predicting} align model confidence and accuracy with a threshold; \citet{jiang2021assessing,chen2021detecting} train several models and use their ensembles or disagreement. Our importance weighting approach is computationally simpler than the latter and is more flexible in comparison to the former, as it allows for concept drift and can be used in downstream tasks beyond model selection as we demonstrate both theoretically and empirically.



\textbf{Domain adaptation} is another closely related problem setting. Domain adaptation (DA) methods require access to labeled source and unlabeled target domains during training and aim to improve target performance via a combination of distribution matching \citep{ganin2016Domainadversarial,sun2016Deep,shen2018wasserstein}, self-training \citep{shu2018DIRTT,kumar2020Understanding}, data augmentation \citep{cai2021Theory,ruan2021optimal}, and other regularizers. DA methods are typically challenging to train and require retraining for every new target domain. On the other hand, our importance weights are easy to learn for a new domain allowing for efficient fine-tuning, similar to test-time adaptation methods \citep{sun2020TestTime,wang2020Tent,zhang2020Adaptive}, which adjust the model based on the target unlabeled samples. Our importance weights can also be used to define additional regularizers to enhance existing DA methods.


\textbf{Importance weighting} has often been used in the domain adaptation literature on label shift \citep{lipton2018Detecting,azizzadenesheli2019Regularized,maity2022minimax} and covariate shift \citep{sugiyama2007covariate,hashemi2018weighted} but the application has been lacking in the area of concept drift models \citep{cai2019Transfer,maity2021linear}, due to the reason that it is generally impossible to estimate the  weights without seeing labeled data from the target. In this paper, we introduce an exponential tilt model which accommodates concept drift while allowing us to estimate the importance weights for the distribution shift. 

==> exponential-tilt(ICLR2023)/sections/setup.tex <==
\section{The exponential tilt model}
\label{sec:exponential-tilt}
\paragraph{Notation} We consider a $K$-class classification problem. Let $\cX \in \reals^d$ and $\cY\triangleq[K]$ be the space of inputs and set of possible labels, and $P$ and $Q$ be probability distributions on $\cX\times\cY$ for the source and target domains correspondingly.
% We consider $P$ as the distribution of samples in the source domain and $Q$ as that in the target domain.
A (probabilistic) classifier is a map $f:\cX\to\Delta^{K-1}$.
% , where $\Delta^{K-1}$.
% is the probability simplex in $\reals^K$.
We define $p\{x, Y = k\}$ as the weighted source class conditional density, \ie\ $p\{x, Y = k\} = p\{x\mid Y = k\} \times P\{Y = k\}$,  where $p\{x \mid Y = k\}$ is the density of the source feature distribution in class $k$ and $P\{Y = k\}$ is the class probability in source. We similarly define $q\{x , Y = k\}$ for target. 

We consider the problem of learning importance weights on samples from a source domain so that the weighted source samples mimic the target distribution. We assume that the learner has access to labeled samples $\{(X_{P,i},Y_{P,i})\}_{i=1}^{n_P}$ from the source domain and and unlabeled samples $\{X_{Q,i}\}_{i=1}^{n_Q}$ from the target domain. The learner's goal is to estimate a weight function $\weight(x, y)>0$ such that
\begin{equation}
\Ex\left[\weight(X_P,Y_P)g(X_P,Y_P)\right] \approx \Ex\big[g(X_Q,Y_Q)\big]\text{ for all (reasonable) }g: \cX \times \cY \to \reals.
\label{eq:true-weighted-expectation}
\end{equation}
Ideally, $\weight = \frac{dQ}{dP}$ is the likelihood ratio between the source and target domains (this leads to equality in \eqref{eq:true-weighted-expectation}), but learning this weight function is generally impossible without labeled samples from the target domain \citep{david2010Impossibility}. Thus we must impose additional restrictions on the domains.

\paragraph{The exponential tilt model} We assume that there is a vector of sufficient statistics $T:\cX \to \reals^p$ and the parameters \{$\theta_k \in \reals^p$, $\alpha_k\in \reals\}_{k=1}^K$ such that 
\begin{equation}
\textstyle\log\frac{q\{x,Y=k\}}{p\{x,Y=k\}} = \theta_k^\top T(x) + \alpha_k\text{ for all }k\in[K];
\label{eq:exponential-tilt}
\end{equation}
\ie\ $q\{x,Y=k\}$ is a member of the exponential family with base measure $p\{x,Y=k\}$ and sufficient statistics $T$. 
We call \eqref{eq:exponential-tilt} the \textbf{exponential tilt} model. It implies the importance weights between the source and target samples are
\[
\weight(x,y) = \exp(\theta_y^\top T(x) +  \alpha_y).
\]
\paragraph{Model motivation}
The exponential tilt model is motivated by the rich theory of exponential families in statistics. In machine learning, it was used for learning with noisy labels and for improving worst-group performance when group annotations are available \citep{li2020tilted,li2021tilted}. It is also closely related to several common models in transfer learning and domain adaptation. In particular, it implies there is a linear concept drift between the source and target domains. It also extends the widely used \textbf{covariate shift} \citep{sugiyama2012Machine} and \textbf{label shift} models \citep{alexandari2020EM,lipton2018Detecting,azizzadenesheli2019Regularized,maity2022minimax,garg2020Unified} of distribution shifts. It extends the covariate shift model because the exponential tilt model permits (linear in $T(X)$) \textbf{concept drifts} between the source and target domains; it extends the label shift model because it allows the class conditionals to differ between the source and target domains. It does, however, come with a limitation: implicit in the model is the assumption that there is some amount of overlap between the source and target domains. In the subpopulation shift setting, this assumption is always satisfied, while in domain generalization it may be violated if the new domain drastically differs from the source data (see Appendix \ref{sec:normal-mixture} for a synthetic data example).


\paragraph{Choosing $T$} 
% We comment on the choice of the sufficient statistics $T$ under the subpopulation shift setting. 
The goal of $T$ is to identify the common subpopulations across domains, such that 
\[(X_P,Y_P)\mid\{T(X_P) = t, Y_P = k\}\overset{d}{\approx}(X_Q,Y_Q)\mid\{T(X_Q) = t, Y_P = k\}.\]
If $T$ segments the source domain into its subpopulations (\ie\ the subpopulations are $\{(x, y)\in\cX\times \cY\mid T(x) = t, y = k\}$ for different values of $t$'s and $k$'s), then it is possible to achieve perfect reweighing of the source domain with the exponential tilt model: the weight of the $\{T(X) = t, Y = k\}$ subpopulation is $\exp(\theta_k^\top t+\alpha_k)$. However, in practice, such a $T$ that perfectly segments the subpopulations may not exist (\eg\ the subpopulations may overlap) or is very hard to learn (\eg\ we don't have prior knowledge of the subpopulations to guide $T$).

If no prior knowledge of the domains is available, we can use a neural network to parameterize $T$ and learn its weights along with the tilt parameters, or simply use a pre-trained feature extractor as $T$, 
which we demonstrate to be sufficiently effective in our empirical studies.
We also study the effects of misspecification of $T$ using a synthetic dataset example in Appendix \ref{sec:normal-mixture}.



==> exponential-tilt(ICLR2023)/sections/theory.tex <==
\section{Theoretical properties of distribution matching}

\subsection{Identifiability of the exponential tilt model}
\label{sec:identifiability}
To show that the $\theta_k$'s are identifiable from \eqref{eq:distribution-matching}, we must show that there is a unique solution to \eqref{eq:distribution-matching}. Unfortunately, this is impossible without additional assumptions. For example, consider a linear discriminant analysis (LDA) problem in which the class conditionals drift between the source and target domains:
\[
\begin{aligned}
p\{x,Y=k\} &= \pi_k\phi(x-\mu_{P,k}) \\
q\{x,Y=k\} &= \pi_k\phi(x-\mu_{Q,k})
\end{aligned},
\]
where $\phi$ is the standard MVN density. Here the $\pi_k\in(0,1)$ are the class proportions in both source and target domains, while the $\mu_{P,k}$'s (resp.\ the $\mu_{Q,k}$'s) are the class conditional means in the source (resp.\ target) domain. We see that this problem satisfies the exponential tilt model with $T(x) = (1,x)$:
\[
\log\frac{q\{x,Y=k\}}{p\{x,Y=k\}} = (\mu_{Q,k} - \mu_{P,k})^\top x .
\]
Unfortunately, this instance of the exponential tilt model is not identifiable; any permutation of the class labels $\sigma:[K]\to[K]$ also leads to the same (marginal) distribution of inputs:
\[
\begin{aligned}
&\sum_{k=1}^Kp\{x,Y=k\}\exp\left(\textstyle(\mu_{Q,k} - \mu_{P,k})^\top x + \frac12\|\mu_{P,k}\|_2^2 - \frac12\|\mu_{Q,k}\|_2^2\right) \\
&\quad= \sum_{k=1}^Kp\{x,Y=\sigma(k)\}\exp\left(\textstyle(\mu_{Q,k} - \mu_{P,\sigma(k)})^\top x + \frac12\|\mu_{P,\sigma(k)}\|_2^2 - \frac12\|\mu_{Q,k}\|_2^2\right).
\end{aligned}
\]
From this example, we see that the non-identifiability of the exponential tilt model is closely related to the label switching problem in clustering. Intuitively, the exponential tilt model in the preceding example is too flexible because it can tilt any $p\{x,Y=k\}$ to $q\{x,Y=l\}$. Thus there is ambiguity in which $p\{x,Y=k\}$ tilts to which $q\{x,Y=l\}$. In the rest of this subsection, we present two identification restrictions that guarantee the exponential tile model is identifiable.

\subsubsection{Anchor sets} 

A standard identification restriction in related work on domain adaptation is a clustering assumption. For example, \citet{tachet2020Domain} assume there is a partition of $\cX$ into disjoint sets $\cX_k$ such that $\supp(P\{\cdot\mid Y=k\}),\supp(Q\{\cdot\mid Y=k\}) \subset \cX_k$ for all $k\in[K]$. This assumption is strong: it implies there is a perfect classifier in the source and target domains. Here we consider a weaker version of the clustering assumption: there are sets $\cS_k$ such that
\[
P\{Y=k\mid X\in\cS_k\} = Q\{Y=k\mid X\in\cS_k\} = 1.
\]
We note that the $\cS_k$'s can be much smaller than the $\cX_k$'s; this permits the supports of $P\{\cdot\mid Y=k\}$ and $P\{\cdot\mid Y=l\}$ to overlap. 

\begin{definition}[anchor set]
\label{def:anchor-set}
A set $\cS\subset\cX$ is an \textbf{anchor set} if $p\{x,Y=k\} > 0$ and $p\{x,Y=l\} = 0$, $l\ne k$ for all $x\in\cS$.
\end{definition}

% In terms of the regression function (in the source domain) $\eta_P$, an anchor set for the $k$-th class is a set of points such that $\big[\eta_P(x)\big]_k = 1$.

\begin{proposition}[identifiability from anchor sets]
\label{prop:anchor-points} 
If there are anchor sets $\cS_k$ for all $K$ classes (in the source domain) and $T(\cS_k)$ is $d$-dimensional, then there is at most one set of $\theta_k$'s that satisfy \eqref{eq:distribution-matching}.
\end{proposition}

\begin{proof}
Suppose there are two sets of tilt parameters $\theta_k$'s and $\eta_k$'s that satisfy \eqref{eq:distribution-matching}:
\[
q_X\{x\} = \sum_{k=1}^Kp\{x,Y=k\}\exp(\theta_k^\top T(x)) = \sum_{k=1}^Kp\{x,Y=k\}\exp(\eta_k^\top T(x)).
\]
For any $x\in\cS_k$, the terms that include $p\{x,Y=l\}$, $l\ne k$ vanish:
\[
p\{x,Y=k\}\exp(\theta_k^\top T(x)) = p\{x,Y=k\}\exp(\eta_k^\top T(x)).
\]
This implies
\[
\theta_k^\top T(x) = \eta_k^\top T(x)\text{ for all }x\in\cS_k.
\]
We conclude $\theta_k = \eta_k$ because $T(\cS_k)$ is  $d$-dimensional, so there are $d$ points $x_1,\dots,x_d\in\cS_k$ such that $T(x_1),\dots,T(x_d)\in\reals^d$ are linearly independent. 
\end{proof}

This identification restriction is also closely related to the linear independence assumption in \citet{gong2016Domain}. Inspecting the proof of proposition \ref{prop:anchor-points}, we see that the anchor set assumption implies linear independence of $\{p_k(x)\exp(\theta_k^\top T(x))\}_{k=1}^K$ for any set of $\theta_k$'s.


\subsubsection{Invariant inputs/Anchor variables} 

In many applications, certain inputs are known to be invariant between the source and target domains. \my{really?}


\section{Generalization bound}
In this section we establish a generalization bound for the proposed domain adaptation method via exponential tilt. To begin with we define and recall some notations. 

\paragraph{Notations and definitions}
Recall that we consider a classification setup, \ie,  $\cY = [K]$  and $\ell: \reals^{K} \times \cY \to \reals$ is the appropriate 
loss for classification that we use in Algorithm \ref{alg:DAET}. We denote $\reals_{\ge 0}$ as the set of all non-negative real numbers and $\cF$ as the hypothesis class for all the classifiers. For an $f \in \cF$ and a weight function $\weight: \cX \to \reals_{\ge 0}^K $ we denote $\weight(x, j)$ as the $j$-th co-ordinate of $\weight(x)$ and define the weighted loss function and it's empirical version on source data as: 
\[ \textstyle
\cL_P(f, w) = \Ex_{(x, y) \sim P} [\weight(x, y)\ell(f(x), y)], ~ \hat \cL_P (f, w) = \frac 1 {\nsource} \sum_{i = 1}^\nsource  \weight(x_{P, i}, y_{P, i})\ell\{f(x_{P, i}), y_{P, i}\}\,.
\] We also define the loss function on the target data as: 
\[
\cL_Q(f) = \Ex_{(x, y) \sim Q} \big[\ell(f(x), y)\big]\,.
\] 
If $\{(\alpha_k^\star, \theta_k^\star)\}_{k = 1}^K$ is the true value of the tilt parameters in  \eqref{eq:exponential-tilt}, \ie, the following holds:
\[ \textstyle
  q\{x, Y = k\} = p\{x, Y = k\} \exp\{\alpha_k^\star + (\theta_k^\star)^\top T(x)\}; \ k \in [K]\,,
\] then defining $\weight^\star(x, k) = \exp\{\alpha_k^\star + (\theta_k^\star)^\top T(x)  \}$ as the true weight function we notice that  $\cL_P(f, \weight^\star) = \cL_Q(f)$ as we show in the  following display:
\[ \textstyle
\begin{aligned}
\cL_P(f, \weight^\star) 
 & = \int \sum_{y= 1}^K \weight^\star (x, y) \ell\{f(x), y\} p\{x, Y = y\} dx\\
 & = \int \sum_{y= 1}^K  \ell\{f(x), y\} q\{x, Y = y\} dx=\cL_Q(f)\,.
\end{aligned}
\] 

We next define the Rademacher complexity that  has been frequently used in  machine learning literature to establish a generalization bound. 
Instead of considering the Rademacher complexity on $\cF$ we define the class of weighted losses $\cG(\ell, \cF) = \{g_f(x, y) = w^\star(x, y) \ell(f(x), y): \ f \in \cF\}$  and for $n \in \bbN$ we define it's Rademacher complexity measure as 
\[ \textstyle
    \cR_n(\cG) \triangleq \Ex_{\{(u_i, v_i)\}_{i = 1}^n\stackrel{\IID}{\sim} P} \big[\Ex_{\{\xi_i\}_{i = 1}^n}[\sup_{f \in \cF} \frac1{n} \sum_{i = 1}^n \xi_i \weight^\star(u_i, v_i) \ell \{f(u_i), v_i\}]\big]
\]
where $\{\xi_i\}_{i = 1}^n $ are \IID \ symmetric Rademacher random variables. 
To establish our generalization bound we need the following  assumption on the loss function.

\begin{assumption}
\label{assump:bounded-loss}
The loss function $\ell$ is bounded, \ie, there exists an $B>0$ such that for any $f\in \cF$, $x \in \cX$ and $y \in [K]$ it holds: $|\ell\{f(x), y\}| \le B$. 
\end{assumption}

With the above definitions and the assumption we're now ready to establish our generalization bound. 

\begin{theorem}
\label{th:generalization-bound} For a weight function $\weight$ and the source samples $\{(x_{i, P}, y_{i, P})\}_{i = 1}^\nsource$ of size $\nsource$ let $\hat f_{\weight} = \argmin_{f\in\cF} \hat \cL_P(f, \weight)$. There exists a constant $c> 0$ such that  the following generalization bound holds with probability at least $1 -\delta$
\begin{equation}\textstyle
\label{eq:gen-bound}
    \cL_Q(\hat f_{ \weight}) - \min_{f\in\cF}\cL_Q (f) \le  2 \cR_m(\cG) + B  \| \weight - w^\star \|_{1, P} + c \sqrt{\frac{\log(1/\delta)}{m}} \,.
\end{equation}
\end{theorem}

From the above bound we notice that a  weight function $\weight$ with small $\|\omega - \omega^\star \|_{1, P}$  is crucial to have a classifier on target population with a small generalization bound. In the next subsection we study the property of the weight function $\hat \omega$ with $\hat \omega(x, k) = \exp\{ \hat \alpha_k + {\hat \theta_k}^\top T(x) \}$ where $\{(\hat \alpha_k, \hat \theta_k)\}_{k = 1}^K$ are obtained from Algorithm \ref{alg:DAET} and establish a rate of convergence for $\|\hat \omega - \omega^\star \|_{1, P}$. 

% We let $\ell$ to be the loss function under consideration and  denote the hypothesis class of classifiers as $\cF$. 
% For a weight function $w(x) = (w(x, 1), \dots , w(x, K))^\top$ and a classifier $f \in \cF$ let us define the weighted loss function and it's empirical version as the followings, 
% \begin{equation}
% \label{eq:weighted-loss}
% \begin{aligned}
% \cL(f, w, P) = \Ex_{(X, Y) \sim P} \big[w(X, Y)\ell(f(X), Y)\big]\,,\\
% \hat \cL(f, w) \equiv \cL(f, w, \hat P)  = \frac 1{n_P} \sum_{i = 1}^{n_P} w(X_i^{(P)}, Y_i^{(P)})\ell(f(X_i^{(P)}), Y_i^{(P)})\,.
% \end{aligned}
%     \end{equation} We also define the target loss function as
%     \begin{equation}
%     \label{eq:true-loss}
%     \cL_\star(f) =    \Ex_{(X, Y) \sim Q} \big[\ell(f(X), Y)\big] \,.
%     \end{equation}
%     Let $\{(\alpha_k^\star, \theta_k^\star)\}_{k= 1}^K$ be the true values of the tilt parameters, \ie, the followings hold:
%     \begin{equation}
%         q\{x, Y = k\} = p\{x, Y = k\} \exp\big(\alpha_k^\star + (\theta_k^\star)^\top T(x)  \big); \ k \in [K]\,.
%     \end{equation} We define the true weight function $w^\star$ as 
%     \begin{equation}
% \begin{aligned}
% w^\star(x) = (w^\star(x, 1), \dots, w^\star(x, K))^\top\,, \\
% w_k^\star(x) = \exp\big(\alpha_k^\star + (\theta_k^\star)^\top T(x)  \big); \ k \in [K]\,.
% \end{aligned}
%          \end{equation} One may notice that weighted loss function \eqref{eq:weighted-loss} at the true weight function $w^\star$ is the target loss function, as suggested by the following calculations:
% \[\textstyle
% \begin{aligned}
% \cL(f, w^\star, P) &= \Ex_{(X, Y) \in P} \big[ w^\star (X, Y) \ell(f(X), Y) \big] \\
% & = \int \sum_{k= 1}^K w^\star (x, k) \ell(f(x), k) p\{x, Y = k\} dx\\
% & = \int \sum_{k= 1}^K  \ell(f(x), k) q\{x, Y = k\} dx=\cL_\star(f)\,.
% \end{aligned}
% \] We define the set $\cG(\ell, \cF) = \{g_f(x, y) = w^\star(x, y) \ell(f(x), y): \ f \in \cF\}$ and it's Rademacher complexity measure
% \begin{equation}
%     \label{eq:rademacher}
%     \cR_n(\cG) \triangleq \Ex_{(X_i, Y_i)\sim P: i\in [n]} \Big[\Ex_{\xi_i:i\in [n]}\Big[\sup_{f \in \cF} \frac1{n} \sum_{i = 1}^n \xi_i w^\star(X_i, Y_i) \ell (f(X_i), Y_i)\Big]\Big]
% \end{equation}
%  with $\xi_i: i\in [n]$ are \IID\ Rademacher random variables. 





\subsection{Estimation of the tilt parameters and the weight function}
Here, for notational simplicity, we define $\coef_k = (\alpha_k, \theta_k^\top )^\top$'s
as the tilt parameters, $\coef_k^\star = (\alpha_k^\star, {\theta_k^\star}^\top )^\top$'s as their true values, $S(x) = (1, T(x)^\top )^\top $ as the sufficient statistics for exponential tilt and $\coef = (\coef_1^\top, \dots, \coef_K^\top)^\top\in \reals^{K(d+1)}$ as the long vector containing  all the tilt parameters. 
We recall from Algorithm \ref{alg:DAET} that estimation of the tilt parameters $\coef$ requires a classifier $\hat \eta_P$ on the source data. So, we define our objective for estimating $\coef$ through a generic  classifier $\eta : \cX \rightarrow \Delta^{K}$. Denoting $\eta_k(x)$ as the $k$-th co-ordinate of $\eta(x)$ we define the expected log-likelihood objective as:
\[
\textstyle
\klloss(\eta, \coef) = \Ex_{Q_X}[\log \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}] - \log [\Ex_{P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}]\,,
\] and its empirical version as 
\[
\textstyle
\hat \klloss(\eta, \coef) = \Ex_{\hat Q_X}[\log \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}] - \log [\Ex_{\hat P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}]\,.
\] The term   $\log [\Ex_{P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}]$ in the log-likelihood objective works as a normalizer: for any $\eta : \cX \to \Delta^K$ the function $[ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) ]/[\Ex_{P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}] $ is a density over the support $\cX$ with respect to the base measure $P_X$. Furthermore, plugging in the Bayes classifier $\eta^\star_P$ (defined as $\eta^\star_{P, k}(x) = p\{x, Y = k\}/p_X(x)$) and  $\scoef$ we realize that the quantity $\sum_{k = 1}^K \eta_{P, k}^\star(x) \exp(\coef_k^\top S(x))$ is a density with respect to the base measure $P_X$, as we explain in the following display: 
\[\textstyle
\sum_{k = 1}^K \eta_{P, k}^\star(x) \exp\{{\coef_k^\star}^\top S(x)\} = \sum_{k = 1}^K \frac{p\{x, Y = k\}}{p_X(x)} \exp\{{\coef_k^\star}^\top S(x)\} =  \frac{\sum_{k = 1}^K q\{x, Y = k\}}{p_X(x)} = \frac{q_X(x)}{p_X(x)}
\]
and hence it holds $\Ex_{P_X} \{ \sum_{k = 1}^K \eta_{P, k}^\star(x) \exp\{{\coef_k^\star}^\top S(x)\} = 1$. In the next lemma we establish that $\scoef$ is the unique maximizer of $\klloss(\eta_P^\star, \coef)$, which is crucial for establishing that $\hcoef$ converges to $\scoef$. 

\begin{lemma}\label{lemma:uniqueness}
$\coef \mapsto \klloss(\eta_P^\star, \coef)$ is uniquely maximized at $\scoef$. 
\end{lemma}



We next make the assumption that is standard in establishing consistency of MLE. 

\begin{assumption}
\label{assmp:strong-convexity}
The loss $\coef \mapsto -\klloss(\eta^\star_P, \coef)$ is  strongly convex at $\scoef$, \ie, there exists a constant $\strongconvexity>0$ such that for any $\coef$ it holds:
\[
-\klloss(\eta^\star_P, \coef) \ge -\klloss(\eta^\star_P, \scoef) - \partial_\coef\klloss(\eta^\star_P, \scoef)  ^\top (\coef - \scoef) +\frac{\mu}{2}\|\coef - \scoef\|_2^2\,. 
\]
\end{assumption}
We note that the assumption is a restriction on the distribution $Q_X$ rather than the objective itself. For technical convenience we next assume that the feature space is bounded. 


\begin{assumption} \label{assump:bounded-covariate}
$\cX$ is bounded, \ie, there exists  an $M>0$ such that $\cX \subset B(0, M)$.
\end{assumption}

Recall, from Algorithm \ref{alg:DAET}, that we need a fitted source classifier $\hat \eta_P$  to estimate the tilt parameter: $\scoef$ is estimated by maximizing $\klloss(\hat \eta_P, \coef)$ rather than the unknown $\klloss(\eta_P^\star, \coef)$. While analyzing the convergence $\hcoef$ we need to control the difference  $\klloss(\hat \eta_P, \coef) - \klloss(\eta_P^\star, \coef)$, which requires the pre-activated logit functions for $\hat \eta_P$ to be close to $\eta_P^\star$. Though the pre-activation logit functions are not unique for a classifier as \[
\textstyle
\frac{\exp(f_k(x))}{\sum_{j = 1}^K \exp(f_j(x))} = \frac{\exp(f_k(x)+a(x))}{\sum_{j = 1}^K \exp(f_j(x) +a(x))}
\] holds  for any $f: \cX \to \reals^K$ and $a:\cX\to \reals$, we notice that the centered logit function of the classifier is unique, \ie, 
\[ \textstyle
\frac{\exp(f_k(x))}{\sum_{j = 1}^K \exp(f_j(x))} =  \eta(x), ~ \sum_{j = 1}^K{f_j(x)} = 0  \Longleftrightarrow f_k(x) = \log\{\eta_k(x)\} - \frac1K \sum_{j = 1}^K \log\{\eta_j(x)\}\,.\]
We next assume that the centered logit for $\hat \eta_P$ convegres to the one for $\eta_P^\star $. 

\begin{assumption}
\label{assmp:source-classifier}
Let $f_{k}^\star(x) = \log\{\eta_{P, k}^\star(x)\} - \frac 1K \sum_{j = 1}^K \log\{\eta_{P, j}^\star(x)\}$. We assume that there exist an estimator $\{\hat f _k(x)\}_{k =1 }^K$ for $\{f^\star_k(x)\}_{k = 1}^K$ such that the following holds: there exists a constant $c>0$ such that  for almost surely $[\bbP_X]$  it holds
\[
\Pr(\|\hat f(x) - f^\star(x)\|_{2} > t) \le \exp(-c t^2 /r_m^2), ~ t > 0\,.
\]
\end{assumption}



Having such an estimator we construct $\hat \eta_P$ as $\hat \eta_{P, k}(x) = \exp(\hat f_k(x))/\{\sum_{j = 1}^K \exp(\hat f_j(x))\}$, which we shall use in Algorithm \ref{alg:DAET} to estimate $\hcoef$and set the weights $\hat \weight$ as $\hat \weight(x, k) = \exp\{\hcoef_k^\top S(x)\}$.  With the above assumptions we're ready to establish the concentration for $\hcoef - \scoef$ and  $\hat \weight - \weight^\star$.
\begin{lemma} \label{lemma:tilt-concentration}
Let the assumptions \ref{assmp:strong-convexity}, \ref{assump:bounded-covariate} and \ref{assmp:source-classifier} hold. For the sample sizes $m, n$ define $\alpha_{m, n} = r_m \sqrt{\log(m+n)}+ m ^{-1/2} + n^{-1/2}$. There exists constants $k_1, k_2>0$ such that with probability at least the following hold:
\[
\|\htheta - \stheta \|_2 \le k_1 \alpha_{m, n}\sqrt{\log(1/\delta)}, \text{ and } \|\hat \weight - \weight^\star\|_{1, P} \le k_2 \alpha_{m, n}\sqrt{\log(1/\delta)}. 
\]
\end{lemma}

\begin{corollary}
Combining the results in Theorem \ref{th:generalization-bound} and Lemma \ref{lemma:tilt-concentration} we conclude that there exists a $k_3>0$ such that  with probability at least $1 - (2K + 2)\delta$ the following holds:
\[
\cL_Q(\hat f_{\hat w}) - \min_{f}\cL_Q (f) \le  2 \cR_m(\cG) + k_3 \alpha_{m,n}\sqrt{\log(1/\delta)}\,.
\]
\end{corollary}

\my{summarize the implications of theoretical results}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/estimation.tex <==
\section{Estimation of the exponential tilt parameters}

In this section we present a method for estimating the tilt parameters.  Throughout the section we assume that the condition \ref{assmp:non-linear} is satisfied and the tilt parameters in \eqref{eq:exponential-tilt} are uniquely identified.



% There are several ways one can estimate the tilt parameters, a  popular approach is matching the distributions, where one can minimize a distribution between $q_X$ and the exponentially tilted mixture \eqref{eq:rep1}. In the following  subsection we consider the simple approach of moment matching. 

% \subsection{Moment matching approach}
% We estimate the tilt parameters by matching some moments for target marginal $q_X$ and source class conditionals $p_0$ and $p_1$. Specifically, for a suitably chosen $f(x)$ we solve the equation 
% \begin{equation}
%     \label{eq:moment-matching}
%     E_{\hat Q_X} [f(x)] = \hat \pi_Q E_{\hat P_1}\left[f(x) e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[f(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right]
%     \end{equation} to get the estimates $\hat \pi_Q, \hat \beta_0$ and $\hat \beta_1$. In the traditional moment matching setup we consider $f = 1, \Phi^{\otimes 1}(x) \Phi(x), \Phi^{\otimes 2}(x) = \Phi(x)\Phi(x)^\top, \dots $ to get the sufficiently many independent equations to estimate the parameters. More explicitly saying the parameters as estimated from the following independent equations: 
%     \begin{equation}
%         \begin{aligned}
%         1 = \hat \pi_Q E_{\hat P_1}\left[ e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[ e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right],\\
%         E_{\hat Q_X} [\Phi(x)] = \hat \pi_Q E_{\hat P_1}\left[\Phi(x) e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[\Phi(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right],\\
%         E_{\hat Q_X} [\Phi(x)\Phi(x)^\top] = \hat \pi_Q E_{\hat P_1}\left[\Phi(x)\Phi(x)^\top e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[\Phi(x)\Phi(x)^\top e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right],
%         \end{aligned}
%     \end{equation} where we note that any one of the three equations cannot be derived from the other two equations. 
    
    
    
    
%     A couple of questions immediately one might ask  are the followings:  What is the rate of convergence for the estimates and how does it depend on $f$? What would be a \emph{good} choice of $f$? To answers these question we decompose the right hand side of the equation \eqref{eq:moment-matching}. Here, we note that 
%     \begin{equation}
%         \begin{aligned}
% &  \hat \pi_Q E_{\hat P_1}\left[f(x) e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}\right] + (1-\hat \pi_Q) E_{\hat P_0}\left[f(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right]\\
% & =  \underbrace{\pi_Q E_{ P_1}\left[f(x) e^{ \alpha_1 + \beta_1^\top \Phi(x)}\right] + (1- \pi_Q) E_{ P_0}\left[f(x) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right]}_{(1)} \\
%  & ~~ + \underbrace{(1 - \hat \pi_Q) \big( E_{\hat P_0} - E_{P_0} \big) \left[f(x) e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}\right]}_{(2.a)} + \underbrace{\hat \pi_Q \big( E_{\hat P_1} - E_{P_1} \big) \left[f(x) e^{\hat \alpha_1 + \hat \beta_1^\top
%  \Phi(x)}\right]}_{(2.b)} \\ 
%  & ~~ + \underbrace{(1 - \hat \pi_Q) E_{P_0} \left[f(x) \Big(e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}- e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\Big)\right]}_{(3.a)} \\
%  & ~~ +  \underbrace{\hat \pi_Q E_{P_1} \left[f(x) \Big(e^{\hat \alpha_1 + \hat \beta_1^\top \Phi(x)}- e^{ \alpha_1 +  \beta_1^\top \Phi(x)}\Big)\right]}_{(3.b)} \\
%  & ~~ + \underbrace{(\hat \pi_Q - \pi_Q) \left(E_{ P_1}\left[f(x) e^{ \alpha_1 + \beta_1^\top \Phi(x)}\right] -  E_{ P_0}\left[ f(x) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right]\right)}_{(4)}\,.
%         \end{aligned}
%     \end{equation}
    
    
% We start by observing that (1) is equal to $E_{Q_X}[f(x)]$ which is the population mean of the left hand side in equation \eqref{eq:moment-matching}. Hence, taking (1) in the other side would make the left hand side 
% \[(5)\triangleq E_{\hat Q_X}[f(x)] - E_{Q_X}[f(x)] \,,\] which is small in limit.   
% The magnitude of the  term $E_{ P_1}\left[f(x) e^{ \alpha_1 + \beta_1^\top \Phi(x)}\right] -  E_{ P_0}\left[ f(x) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right] = E_{ Q_1}[f(x)] - E_{ Q_0}[f(x)]$ in (4) contributes in the rate of convergence of $\hat \pi_Q - \pi_Q$, in a way that a bigger magnitude of $E_{ Q_1}[f(x)] - E_{ Q_0}[f(x)]$ would make $\hat \pi_Q - \pi_Q$ converge faster. So we require $E_{ Q_1}[f(x)] - E_{ Q_0}[f(x)]$ to be as big as possible in some norm. With the first order Taylor expansion on (3.a) we have \[
% \begin{aligned}
% & E_{P_0} \left[f(x) \Big(e^{\hat \alpha_0 + \hat \beta_0^\top \Phi(x)}- e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\Big)\right]\\
% & \approx E_{P_0} \left[f(x)\big((\hat \alpha_0 - \alpha_0 ) + (\hat \beta_0 - \beta_0)^\top \Phi(x)\big) e^{ \alpha_0 +  \beta_0^\top \Phi(x)}\right]\\
% & = E_{Q_0} \left[f(x)\big((\hat \alpha_0 - \alpha_0 ) + (\hat \beta_0 - \beta_0)^\top \Phi(x)\big)\right]\,.
% \end{aligned}
% \] This implies that we require the magnitudes of $E_{Q_0}[f(x)]$ and $E_{Q_0}[\Phi(x)f(x)]$ to be as large as possible and similarly from (3.b) we require the magnitudes of $E_{Q_1}[f(x)]$ and $E_{Q_1}[\Phi(x)f(x)]$ to be as large as possible. The  error in estimation arises from (2.a), (2.b) and (5) and the error is higher for larger $\|f\|_\infty$. This contradicts with the requirement that larger magnitude of  $E_{Q_0}[f(x)\Phi(x)]$ and $E_{Q_1}[f(x)\Phi(x)]$ is better for estimation of $\hat \beta_0$ and $\hat \beta_1$. So, we fix some $L>0$ and try to find the best possible choice of $f$ with $\|f\|_\infty = L. $

\subsection{Maximum likelihood approach}

% Here one can consider maximizing the likelihood for the semi-supervised data. We denote $\eta_P(x)\triangleq P(y = 1|x) = \frac{\pi_P p_1(x)}{\pi_P p_1(x) + (1-\pi_P) p_0(x)}$ as the source regression function. With the labeled data for source and unlabeled data for target the likelihood is
% \begin{equation}
% \begin{aligned}
%  \cL & = \prod_{i = 1}^m \big(\pi_P p_1(x_i^{(P)})\big)^{y_i^{(P)}}\big((1-\pi_P) p_0(x_i^{(P)})\big)^{1-y_i^{(P)}}\\
%  & ~~~ \times \prod_{i=1}^n \left( \pi_Qp_1(x_i^{(Q)})e^{\alpha_1 + \beta_1^\top \Phi(x_i^{(Q)})} + (1-\pi_Q)p_0(x_i^{(Q)})e^{\alpha_0 + \beta_0^\top \Phi(x_i^{(Q)})}\right)\,.
% \end{aligned}
%   \end{equation}
%   Denoting $\tilde q (x) \triangleq \pi_Qp_1(x_i^{(Q)})e^{\alpha_1 + \beta_1^\top \Phi(x_i^{(Q)})} + (1-\pi_Q)p_0(x_i^{(Q)})e^{\alpha_0 + \beta_0^\top \Phi(x_i^{(Q)})}$ we see that maximizing the likelihood loss is equivalent to minimizing the following loss:
   
%   \[
%  \big[  \text{Classification loss with } \{(x_i^{(P)}, y_i^{(P)})\}_{i = 1}^m \big]+ \text{KL} (\hat Q_X || \tilde Q_X ). 
%   \]

Given the source class conditionals $p_j(x)$, the transfer parameters $ \{(\beta_j, \pi_j)\}_{j = 1}^K$ and the tilt transformation $T$ the likelihood for the target data $\{x_i\}_{i = m+1 }^{m + n}$ is 
\begin{equation}
    \label{eq:likelihood-target}
    \cL\Big((\beta_j, \pi_j)\big\vert x_i; ~ i = m+1, \dots, m+n \Big) = \prod_{i = m+1}^{m+n} \Bigg\{\sum_{j = 1}^K  \frac{\pi_j} {\alpha_j}  p_j(x_i) e^{\beta_j ^\top T(x)} \Bigg\}
\end{equation} where $\alpha_j = \int p_j(x_i) e^{\beta_j ^\top T(x)}$. The unknown $p_j$'s are replaced by estimates $\hat p_j$'s obtained from the source data and the likelihood is maximized to estimate the transfer parameters. 

\begin{equation}
    \label{eq:mle}
  \{(\hat \beta_j, \hat \pi_j)\}_{j = 1}^K  = \underset{\{(\beta_j, \pi_j)\}_{j = 1}^K}{\argmin} - \sum_{i = m+1}^{m+n}\log \Bigg\{\sum_{j = 1}^K  \frac{\pi_j} {\hat \alpha_j}  \hat p_j(x_i) e^{\beta_j ^\top T(x)} \Bigg\},
\end{equation} where $\hat \alpha_j = \int \hat p_j(x_i) e^{\beta_j ^\top T(x)}$.


\subsection{Self-training approach}
The self-training approach minimizes the average entropy to estimate the tilt parameters. We notice that the exponentially tilted model implies the log odds difference between source and target is a linear function of $T(x)$: \begin{equation}
\begin{aligned}
&\textsc{logit}_j^{(Q)}(x) - \textsc{logit}_k^{(Q)}(x)\\  &=\log\Bigg(\frac{ \pi_j^{(Q)} q_j(x) }{ \pi_k^{(Q)} q_k(x) }\Bigg)\\
 &= \log\Bigg(\frac{\pi_j^{(P)} p_j(x)}{\pi_k^{(P)} p_k(x)}\Bigg) + (\beta_j - \beta_k)^\top T(x) - (\alpha_j - \alpha_k)\\ & ~~~~ + \log \Bigg(\frac{ \pi_j^{(Q)}  }{ \pi_k^{(Q)}}\Bigg)- \log \Bigg(\frac{ \pi_j^{(P)}  }{ \pi_k^{(P)}}\Bigg)\\
 & = \big\{\textsc{logit}_j^{(P)}(x) + \beta_j^\top T(x) + \gamma_j\big\}  -\big\{ \textsc{logit}_k^{(P)}(x) + \beta_k^\top T(x) + \gamma_k\big\}
\end{aligned}
   \end{equation} But the above may not imply \begin{equation}
        \textsc{logit}_j^{(Q)}(x)  =   \textsc{logit}_j^{(P)}(x) + \beta_j^\top T(x) + \gamma_j\,.
   \end{equation} So, we consider a modification of logits which satisfies  the restriction that \begin{equation}
       \sum_j \textsc{logit}_j^{(P)}(x) = 0, ~~~ \text{ for all}~~ x\,,
   \end{equation} which is satisfied by the unique modification that 
   \begin{equation}
       \textsc{c-logit}_j^{(P)}(x) \gets \textsc{logit}_j^{(P)}(x) - \frac{1}{K}\sum_k \textsc{logit}_k^{(P)}(x)
   \end{equation} and the followings are satisfied. \begin{equation}\begin{aligned}
   \textsc{c-logit}_j^{(Q)}(x)  =   \textsc{c-logit}_j^{(P)}(x) + \big\{\beta_j - \frac1 K \sum_k \beta_k \big\}^\top T(x) + \big\{\gamma_j - \frac1K \sum_K \gamma_K\big\},\\
   q(y = j|x; \beta_k, \gamma_k; k \in 1, \dots, K) = \frac{e^{\textsc{c-logit}_j^{(Q)}(x)}}{\sum_k e^{\textsc{c-logit}_k^{(Q)}(x)}}.
   \end{aligned}
      \end{equation} 
Finally, denoting $\beta \equiv (\beta_1, \dots, \beta_K)^\top\in \reals^{K \times \text{dim}(T(x))}$ and $\gamma = (\gamma_1, \dots,\gamma_K)^\top \in \reals^K$ the  parameters are estimated by minimizing the loss
\begin{equation}
   (\hat \beta, \hat \gamma) \equiv \underset{\beta^\top 1_K = 0, \gamma^\top 1_K = 0}{\mathrm{argmin}} \bbE_{\widehat Q_X}\Big[ -\sum_{j= 1}^K q(y = j | x; \beta, \gamma) \log \{q(y = j | x; \beta, \gamma)\}\Big]
\end{equation} and the final classifier is obtained as \begin{equation}
  \hat y(x) \equiv  \argmax_{j} \{\textsc{c-logit}_j^{(Q)}(x)  =   \textsc{c-logit}_j^{(P)}(x) + \hat \beta_j^\top T(x) + \hat \gamma_j\}
\end{equation}
\textcolor{blue}{Write down the LDA proof of self-training}

\begin{theorem}
Self-training for balanced-LDA works. 
\end{theorem}

\begin{proof}
For a classifier $\sigma(x^\top w)$ the self-training loss function is 
\begin{equation}
    L(w) = E_{Q_X}\big[ - \sigma(x^\top w) \log \big( \sigma(x^\top w) \big) - \big(1 - \sigma(x^\top w )\big) \log \big( 1- \sigma(x^\top w)  \big)\big]
     \end{equation}
Assuming the data is being generated from the LDA model, \ie,  $Q_X \sim \frac 12 N(\mu, I) + \frac12 N(-\mu, I)$ we show that \begin{equation}
    \Bigg(I - \frac{\mu \mu^\top }{\|\mu\|_2^2}\Bigg) \nabla_{w} L(\mu) = 0
\end{equation} We start by noticing that 
\[
\begin{aligned}
\nabla_{w} L(w) & = E_{Q_X}\Bigg[ - \log \bigg(\frac{\sigma(x^\top w)}{1- \sigma(x^\top w)} \bigg) \sigma(x^\top w) \big(1- \sigma(x^\top w)\big) x\Bigg]\\
&= E_{Q_X}\Bigg[ -  \sigma(x^\top w) \big(1- \sigma(x^\top w)\big) xx^\top \Bigg]w\,,
\end{aligned}
\] and 
\[
E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) xx^\top \Bigg]\mu = E_{N(-\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) xx^\top \Bigg]\mu\,.
\] This implies 
\[
\nabla_w L(\mu) = E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) xx^\top \Bigg]\mu
\] 
Denoting $P_{\mu}^\perp = I - \frac{\mu \mu^\top }{\|\mu\|_2^2}$ we notice that for a random variable $x \sim N(\mu, I)$ the following holds: (1) $P_\mu ^\perp x \perp \!\!\! \perp \mu^\top x$ and (2) $E\big[P_{\mu}^\perp x\big] = 0$. This two facts imply
\[
\begin{aligned}
\Bigg(I - \frac{\mu \mu^\top }{\|\mu\|_2^2}\Bigg) \nabla_{w} L(\mu) &= E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) P_\mu^\perp x x^\top\mu \Bigg] \\
&= E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) x^\top\mu \Bigg] E_{N(\mu, I)}\Big[  P_\mu^\perp x  \Big]
& = 0\,.
\end{aligned}
\]
The fact that $P_\mu \perp \nabla_{w} L(\mu) = 0 $ implies $\nabla_{w} L(\mu) = c\mu$ for some $c\in \reals$. Again 
\[
\begin{aligned}
\nabla_{w} L(\mu) &= E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) P_\mu^\perp x x^\top\mu \Bigg]\\
& ~~~+ E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big) \frac{\mu \mu^\top}{\|\mu\|_2^2} x x^\top\mu \Bigg] \\
& = E_{N(\mu, I)}\Bigg[ -  \sigma(x^\top \mu) \big(1- \sigma(x^\top \mu)\big)   (x^\top\mu)^2 \Bigg]\frac{\mu }{\|\mu\|_2^2} \\
& = -\lambda \mu\,,
\end{aligned}
\] where $\lambda>0$. The fact that  $\nabla_{w} L(w) + \lambda w$ is gradient of the regularized loss $L(w) + \frac{\lambda}{2}\|w\|_2^2$ and  $\nabla_{w} L(\mu) + \lambda \mu = 0$ implies $\mu$ is the unique minimizer in an $\ell_2$-ball. For a different $\lambda$ we can replace $\mu$ by $\delta \mu$ for some $\delta>0$ resulting 
\[
\begin{aligned}
\nabla_{w} L(\delta\mu) &= E_{N(\mu, I)}\Bigg[ -  \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)   \delta ^2 (x^\top\mu)^2 \Bigg]\frac{\delta \mu }{\delta^2 \|\mu\|_2^2}\\
& = E_{N(\mu, I)}\Bigg[ -  \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)    (x^\top\mu)^2 \Bigg]\frac{\delta \mu }{ \|\mu\|_2^2}
\end{aligned}
\] where $\delta$ is adjusted accordingly to get $\lambda = \frac{1}{ \|\mu\|_2^2} E_{N(\mu, I)}\Bigg[   \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)    (x^\top\mu)^2 \Bigg]$. Since, 
\[
\begin{aligned}
& \frac{1}{ \|\mu\|_2^2} E_{N(\mu, I)}\Bigg[   \sigma(\delta x^\top \mu) \big(1- \sigma(\delta x^\top \mu)\big)    (x^\top\mu)^2 \Bigg]\\
& = E_{N(1, 1)}\Big[   \sigma(\delta' g) \big(1- \sigma(\delta' g )\big)    g^2 \Big], ~~ \delta' \triangleq \delta \|\mu\|_2 \\
& \le \frac 14 E_{N(1, 1)}\big[       g^2 \big] = \frac 12\,.
\end{aligned}
\] So, we have to set $\lambda < \frac 12$. 
\end{proof}

==> sections/exp-tilt.tex <==
\section{Transfer through exponential tilting}

We consider a problem of domain adaptation in binary classification setup. Let $\cX\subset  \reals^f$ be the space of feature vectors. We assume that the source and target populations are distributed as $P$ and $Q$ respectively, where $P$ and $Q$ are probability distributions on the space $\cX\times \{0, 1\}$.  Assume that we have $m$ many \IID\ labeled observations  $\{(x_i, y_i)\}_{i=1}^m  $ from $P$ and  $n$ \IID\ unlabeled observations $ \{x_i\}_{i = m+1}^{m +n} $ from the target distribution $Q$. Denoting $D = \{(x_i, y_i)\}_{i=1}^m  \cup \{x_i\}_{i = m+1}^{m +n} $ as the full dataset we see that $D \sim P^{\otimes m} \otimes Q_X^{\otimes n}$ where $Q_X$ is the marginal of $x$ under $Q$ distribution.   The task at hand is to construct a classifier for the target population. 


We restrict ourselves to the setup of exponentially tilted transfers. We assume that the class conditional distributions for $P$ and $Q$ are continuous with densities $p_0$, $p_1$ and $q_0$, $q_1$, respectively. Furthermore, we assume that the class conditional densities for target are exponential tilts to the corresponding class conditional densities for source. More specifically, given a transformation $\Phi(x)\in \reals^d$ and some $\beta_0, \beta_1 \in \reals^d$ we have the followings: 
\begin{equation}
    \label{eq:exponential-tilt}
\text{For } y \in \{0, 1\}  ~~~~~   q_y(x) = p_y(x) e^{\alpha_y + \beta_y ^\top \Phi(x)} \text{  where  }  \alpha_y = - \log \left(\int p_y(x) e^{ \beta_y ^\top \Phi(x)} dx \right).
\end{equation}
 In the above tilt the constant $\alpha_y$ is set  to make $q_y$ a valid density, \ie, $\int q_y(x)dx = 1$. 
 
 This type of exponential tilting has a natural connection to the linearly adjusted posterior drift model \cite{maity2021linear} though logistic link function. Denoting $\gamma$ as the logistic link ($\gamma(x) = \log\{x/(1-x)\}$) and $\pi_Q$ and $\pi_P$ as the proportion of having $y = 1$ in the $P$  and $Q$ distribution, respectively,  we notice that \eqref{eq:exponential-tilt} implies 
 \begin{equation}
 \label{eq:target-classifier}
     \begin{aligned}
 \gamma(Q(y = 1| x)) &= \log\left(\frac{q_1(x)}{q_0(x)}\right) + \gamma(\pi_Q)\\
 & = \log\left(\frac{p_1(x)}{p_0(x)}\right) + (\alpha_1 - \alpha_0) + (\beta_1 - \beta_0)^\top \Phi(x) + \gamma(\pi_Q)\\
 & = \gamma(P(y = 1| x)) - \gamma(\pi_P) + (\alpha_1 - \alpha_0) + (\beta_1 - \beta_0)^\top \Phi(x) + \gamma(\pi_Q)\,. 
 \end{aligned}
 \end{equation}
  The calculation in the above display implies that after a logistic transformation, the regression function (conditional probability of having $y = 1$ given that we observe the feature value $x$) for target distribution is just a linear shift of the source regression function. This is the exact modelling assumption in linearly adjusted posterior drift setup when the link function is logistic link \citep[see][Equation (1.1)]{maity2021linear}.
  
  Unlike [1], this paper deals with the more challenging setting 
 
 
\subsection{Identifiability of exponential tilting}
Recalling the calculations in display \eqref{eq:target-classifier} we see that  construction of the target classifier requires us to estimate the the following quantities: $P(y = 1| x)$,  $\pi_P$,  $\alpha_1 - \alpha_0$, $\beta_1 - \beta_0$ and $ \pi_Q.$ Given the labeled source data one can estimate  $P(y = 1| x)$ and $\pi_P$. So the question remains \emph{how do we estimate $\alpha_1 - \alpha_0$, $\beta_1 - \beta_0$ and $ \pi_Q$}? A first step toward estimating of these quantities is unique identification of them. We see that from the labeled data from source one can potentially  estimate the $P$ distribution, but in absence of the target labels the best one can do is to estimate $q_X$. Furthermore, these are the maximal information one can hope to estimate from the data at hand, meaning without additional information on $P$ and $Q_X$ the data $D$ is a \emph{minimal sufficient statistics} for them.   Hence, we ask the following question. 
\begin{quote}
   \textbf{Question}: Given the distributions $P$ and $q_X$ when are the quantities $\alpha_1 - \alpha_0$, $\beta_1 - \beta_0$ and $ \pi_Q$ uniquely identifiable? 
\end{quote}
The rest of this subsection is dedicated to answering this question. We start with noticing that under \eqref{eq:exponential-tilt} the marginal density $q_X$ can be written as 
\begin{equation}
\label{eq:rep1}
  q_X(x) = (1-\pi_Q) p_0(x) e^{\alpha_0 +\beta_0 ^\top \Phi(x)}   + \pi_Q p_1(x) e^{\alpha_1 +\beta_1 ^\top \Phi(x)}\,. 
\end{equation} and by absorbing $\pi_Q$ in $\alpha_1$ and $1-\pi_Q$ in $\alpha_0$ we have 
\begin{equation}
\label{eq:rep2}
    q_X(x) = p_0(x) e^{a_0 +\beta_0 ^\top \Phi(x)}   +  p_1(x) e^{a_1 +\beta_1 ^\top \Phi(x)}\,,
\end{equation} for some $a_0, a_1 \in \reals$. With this two representations one might ask whether these two representations are equivalent, in the sense that is it possible to recover one representation from another.  The following lemma establish that. 
\begin{lemma}
\label{lemma:eqiv-rep}
We have the equivalence between the representations \eqref{eq:rep1} and \eqref{eq:rep2}, \ie, \begin{enumerate}
    \item \eqref{eq:rep1} implies \eqref{eq:rep2} with $a_1 = \alpha_1 + \log(\pi_Q)$ and $a_0 = \alpha_0 + \log(1-\pi_Q)$, and 
    \item \eqref{eq:rep2} implies \eqref{eq:rep1} with $\alpha_y = - \log \left(\int p_y(x) e^{ \beta_y ^\top \Phi(x)} dx \right)$ for $y = 0$ and $1$ and $\pi_Q = e^{a_1 - \alpha_1} = 1 - e^{a_0 - \alpha_0}$. 
\end{enumerate}
\end{lemma}
We stick to the representation in \eqref{eq:rep2} and from the transformed target regression function in display \eqref{eq:target-classifier} we only need to identify $a_1 - a_0 = \alpha_1 - \alpha_0 + \log(\pi_Q) - \log(1 - \pi_Q)$ and $\beta_1 - \beta_0$.  Next  we consider  a condition on the density ratio $\frac{p_1(x)}{p_0(x)}$
with is  necessary and sufficient for unique identification of the parameters $a_0$, $a_1$, $\beta_0$ and $\beta_1$. Later we establish that this condition is also necessary and sufficient for unique identification of $a_1 - a_0 $ and $\beta_1 - \beta_0$. We start with the required conditions, where we assume: 

\begin{assumption}
\label{assmp:range}
    For every $v, w \in \reals^d$ and $M>0$ there exists $x_1, x_2 \in \cX$ such that the followings hold: (1) $\|\Phi(x_1)\|_2 \le \frac1 M \le M \le \|\Phi(x_2)\|_2$, and (2) $v^\top \Phi(x_1) w^\top \Phi(x_1) < 0$ and $v^\top \Phi(x_2) w^\top \Phi(x_2) < 0$. 
\end{assumption}

\begin{assumption}
    \label{assmp:non-linear}
    For any $\theta_0,  \delta_0\in \reals$, $\alpha>0$ and $\theta,  \delta \in\reals^d$   we have an $x$ such that 
    \[p_1(x) e^{\theta_0 + \theta^\top \Phi(x)}\left(e^{\delta_0 + \delta^\top \Phi(x)} - 1\right) \neq  p_0(x) \left(e^{\alpha\delta_0 + \alpha\delta^\top \Phi(x)} - 1\right)\,. \]
    \end{assumption}
    Next we show that this condition is necessary and sufficient for uniquely identifying the parameters $a_0$, $a_1$, $\beta_0$ and $\beta_1$.
    
    
   \begin{lemma}
   
   Assume that a solution of the  equation \eqref{eq:rep2} exists and the range of $\Phi(x)$ satisfies the assumption \ref{assmp:range}.  The solution is unique if and only if the assumption \ref{assmp:non-linear} holds. \label{lemma:uniqueness}
   \end{lemma}
   
   The above Lemma asserts that we have a unique target regression function.
   \[
   \eta_Q(x) = \frac{p_1(x) e^{a_1 + \beta_1^\top \Phi(x)}}{p_1(x) e^{a_1 + \beta_1^\top \Phi(x)} + p_0(x) e^{a_0 + \beta_0^\top \Phi(x)}}\,.
   \]
   But we note that to have a unique target regression function we only need $a_1 - a_0$ and $\beta_1 - \beta_0$ to be uniquely identified. In the next lemma we establish these two requirements are equivalent. 
   
   \begin{lemma}
   \label{lemma:unique-reg-fn}
   Assume that a solution of the  equation \eqref{eq:rep2} exists and the range of $\Phi(x)$ satisfies the assumption \ref{assmp:range}. The quantities $a_1 - a_0$ and $\beta_1 - \beta_0$ are unique if and only if the solution of the  equation \eqref{eq:rep2} is unique. 
   \end{lemma}

\subsection{The case of LDA model}
Here, we consider the case of linear discrimination (LDA) model where the decision boundary is linear. For $j \in \{0, 1\}$ let us assume that $p_j(x) \equiv N(\mu_j^{(P)}, \Sigma)$ and $q_j(x) \equiv N(\mu_j^{(Q)}, \Sigma)$, where $\mu_j^{(P)}, \mu_j^{(Q)} \in \reals^d$ and $\Sigma\in \reals^{d \times d }$ is a positive definite matrix. Noticing that $\log(q_j/p_j) = x^\top \Sigma^{-1} (\mu_j^{(Q)} - \mu_j^{(P)}) + \alpha_j, ~ \alpha_j \in \reals$ the minimal requirement of a linear transformation $\Phi$ is that $\text{Row-space}(\Phi) \supseteq \text{Span}(\Sigma^{-1} (\mu_0^{(Q)} - \mu_0^{(P)}), \Sigma^{-1} (\mu_1^{(Q)} - \mu_1^{(P)}))$. Furthermore,  the fact that $ \log  (p_1/p_0) = x^\top \Sigma^{-1} (\mu_0^{(P)} - \mu_1^{(P)}) + C$ implies $\Sigma^{-1} (\mu_0^{(P)} - \mu_1^{(P)}) \notin \text{Row-space}(\Phi)$. These are necessary and sufficient conditions for the assumption \ref{assmp:non-linear} to be satisfied.  

\subsection{The cases of non-identifiability}

One of the cases that is excluded by the condition \ref{assmp:non-linear} is linear decision boundary (with respect to $\Phi(x)$) for $P$. This is a very popular modeling assumption for the classification task and perhaps the most well-known example of such linear decision boundary is the linear discrimination model, \ie, the class conditionals for source are distributed as normal with different means and the same variance. Given a $P$ it is possible to figure out the means and the commons variance and hence the class conditionals. The exponential tilting model \eqref{eq:exponential-tilt} implies that the target distribution also satisfies the linear discrimination model with the same common variance as the source. But the exponential tilting \ref{eq:exponential-tilt} has the flexibility of covering all the linear discrimination models with a specific variance. With the only available knowledge of $q_X$ from the target, the best possible task one can hope to do is clustering on $q_X$.   With the clustering task in mind, it is possible to identify and estimate these cluster densities for the target, which are the target class conditional densities up to a permutation.  But identifying and estimating the cluster densities is only a part of the task toward building a target classifier, one also needs to know which cluster corresponds to which class, and figuring out this correspondence is not possible without the target labels. So, building a target classifier for this specific case of linear discrimination with exponential tilting requires target labels.  

We end this subsection with an example of linear discrimination model which falls under the condition \ref{eq:exponential-tilt} and hence can be tackled even in absence of the target labels. We assume that the feature $\Phi(x)$ has two independent components, \ie, $\Phi(x) = (\Phi_1(x)^\top, \Phi_2(x)^\top)^\top, ~~ \Phi_1(x)\in \reals^{d_1},  \Phi_2(x) \in  \reals^{d_2}, $ and there does not exists a matrix $A\in \reals^{d_2 \times d_1}$ such that  $\Phi_2(x) = A \Phi_1(x) $ for all $x$. We also assume that  the exponential tilting condition \eqref{eq:exponential-tilt} is satisfied with $\Phi_1(x)$ and that  the source decision boundary is linear in terms of $\Phi(x)$ with a non-trivial component for $\Phi_2(x)$, \ie, there exists $\beta_0\in \reals, \beta_1 \in \reals^{d_1}$ and $\beta_2 \in \reals^{d_2}$ such that
\begin{equation}
    \log\left(\frac{p_1(x)}{p_0(x)}\right) = \beta_0 + \beta_1 ^\top \Phi_1(x) + \beta_2 ^\top \Phi_2(x), ~~~~ \beta_2 \neq 0\,.
\end{equation} Then the condition \ref{assmp:non-linear} is satisfied except some special cases when for some $\delta_0, \theta_0 \in \reals$, $\alpha>0$ and $\theta_1, \beta_1 \in \reals^{d_1}$ and any $x$ we have
\[
\beta_2^\top \Phi_2(x) = \theta_0 + \theta_1 ^\top \Phi_1(x) +  \log\left(\frac{e^{\alpha\delta_0 + \alpha\delta_1^\top \Phi_1(x)} - 1}{e^{\delta_0 + \delta_1^\top \Phi_1(x)} - 1}\right)\,.
\]


\subsection{The case of exponential family distributions} 

% In this subsection we provide an interpretation for the condition \ref{assmp:non-linear} when the class conditional distributions in source and target are from exponential family of distributions. With the definition $\cE(T) = \{p_\beta(x) = \exp(\beta^\top T(x)- \beta_0): \beta_0 = \int \exp(\beta^\top T(x)), ~\beta \in \reals^d\}$ where $T: \cX \to \reals^d$ is a feature map, we assume that $p_j(x) \in \cE(T_j^{(P)})$ and $ q_j(x)\in \cE(T_j^{(Q)})$ for $ j = 0, 1. $ Let $A(x)$ is the transformation used in exponentially tilted adaptation. Then the following conditions are necessary. The condition that 
% \begin{equation}
%     \text{Span} \Big\{ (\beta_j^{(Q)})^\top T_j^{(Q)}(x) - (\beta_j^{(P)})^\top T_j^{(P)}(x);~ j = 0, 1 \Big\} \subseteq \text{Span}\big\{A(x)\big\}
% \end{equation} ensures that $A(x)$ is enough for for adaptation. Furthermore, the condition that 
% \begin{equation}
%     (\beta_1^{(P)})^\top T_1^{(P)}(x) - (\beta_0^{(P)})^\top T_0^{(P)}(x) \notin \text{Span}\big\{A(x)\big\}
% \end{equation} is required to maintain identifiability of the transfer.   


In this subsection, we assume that the source and target class conditionals are from the exponential family. With statistic $T(x) \in \reals^d$ the exponential family of distributions has the following collection of  distributions: 
\begin{equation}
    p_\beta(x) = \frac 1 {\beta_0}\exp(\beta^\top T(x)); ~~ \beta_0 = \int \exp(\beta^\top T(x)), ~\beta \in \reals^d\,.
\end{equation} For national simplicity we let $T(x) = x$ from hereon. The following theorem provides identification for the multi-class transfer. 
\begin{theorem}
\label{th:multi-class-exponential}
Suppose $p_j(x), ~ q_j(x); ~ j = 1, 2, \dots, K$ are exponential family distributions with statistic $x$ and the following are satisfied. 
\begin{enumerate}
    \item $\text{span}  \Big\{ \log\big(\frac{q_j(x)}{p_j(x)}\big); ~ j = 1, \dots, K  \Big\} \subseteq \text{span} \big\{T(x), 1\big\}$.
    \item There does not exist a pair $(j, k)$, a vector $u \in \reals^{|T(x)|}$, and a scalar $v\in \reals$ such that $\frac{p_j(x)}{p_k(x)} = e^{u^\top T(x) + v}$. 
\end{enumerate} Then there exists a unique solution to the equation 
\begin{equation}
\label{eq:target-marginal-multi}
    \sum_{j = 1}^K p_j(x) \alpha_j e^{\beta_j^\top T(x) 
    } = q_X(x)\,,
\end{equation} such that $\alpha_j \ge 0$. The conditions are also necessary for existence of unique solution. 
\end{theorem}

\begin{corollary}[LDA with linear transformation]
Suppose the class conditionals satisfies LDA model for source and target distribution with same covariance matrix. More specifically, we assume  $p_j(x) \sim N(\mu_j, \Sigma)$ and $q_j(x) \sim N(\xi_j, \Sigma)$ for some $\{\mu_j, \xi_j\}_{j = 1}^K \subseteq \reals^d$ and $\Sigma \in \reals^{d \times d}$. Furthermore, we also assume the transformation $T(x)$ is linear. Then the conditions in the Theorem \ref{th:multi-class-exponential} simplifies to the following ones. 
\begin{enumerate}
    \item $\text{span}  \Big\{ \Sigma^{-1}(\xi_j - \mu_j); ~ j = 1, \dots, K  \Big\} \subseteq \text{row-space} \big\{T\big\}$.
    \item There does not exist  $1 \le j \neq k \le K$ such that $\Sigma^{-1}(\mu_j - \mu_k) \notin \text{row-space} \big\{T\big\}$, or equivalently, the projection of the vectors $\big\{\Sigma^{-1}\mu_j\big\}_{j = 1}^K$ in the orthogonal space to $\text{row-space} \big\{T\big\}$ are distinct. 
\end{enumerate} The first condition ensures that the transformation $T$ is sufficient for transferring source class conditional densities to target ones  by the exponential tilt adjustment. The second condition is important for the unique identification, which ensures that after the transformation $T'$ which is orthogonal to $T$ (\ie, each row of $T'$ is orthogonal to each row of $T$) the class conditional distributions in the source are distinct. Furthermore, condition 1. that distribution of $T'(x)|y = j$ is the same between source and target. So the feature $T'(x)$ can be viewed as an invariant one across source and target. 

If some the feature co-ordinates has same class conditional distributions across source and target populations, along with some discriminating power for the labels (\eg, $P(x_1|y = j) = Q(x_1 | y = j)$ and $P(x_1 | y = j)$'s are different) then one can set $T$ to be the transformations in the remaining co-ordinates (in previous example $T$ is the matrix obtained after deleting the first row of identity matrix). One may think that since the invariant coordinates have some discriminating power for labels, they can be used to build a classifier which would also work for the target distribution. The exponential tilt correction can recover the target Bayes classifier and result in a better predictive accuracy. 
\end{corollary}

==> sections/exponential-tilt.tex <==
\section{Domain adaptation via exponential tilting}


At a high-level, the proposed method for domain adaptation consists of two steps:
\begin{enumerate}
\item \textbf{fit exponential tilt model:} estimate the parameters $\theta_k$'s in the exponential tilt model by matching the tilted (marginal) distribution of the inputs from the source domain with that of the inputs from the target domain;
\item \textbf{train classifier for target domain:} construct/train a classifier for the target domain by plugging in the estimates of $q\{x,Y=k\}$ into \eqref{eq:target-regression-function} or weighted empirical risk minimization (ERM).
\end{enumerate}
We elaborate on the two steps in the rest of this section and summarize the method in algorithm \ref{alg:DAET}.

\paragraph{Fit exponential tilt model} In the first step, we estimate the parameters of the exponential tilt model by distribution matching. This step is based on the observation that under the exponential tilt model \eqref{eq:exponential-tilt}
\begin{equation}
q_X\{x\} = \sum_{k=1}^Kp\{x,Y=k\}w_k\exp(\theta_k^\top T(x) - a_k(\theta_k)),
\label{eq:distribution-matching}
\end{equation}
where $q_X$ is the (marginal) density of the inputs in the source domain. It is possible obtain an estimate $\hq_X$ of $q_X$ from the unlabeled samples $\{X_i\}_{i=n_s+1}^{n_s+n_t}$ and estimates $\hp\{x,Y=k\}$ of the $p\{x,Y=k\}$'s from the labeled samples $\{(X_i,Y_i)\}_{i=1}^{n_s}$. This suggests we find $\theta_k$'s such that  
\[
\sum_{k=1}^K\hp\{x,Y=k\}w_k\exp(\theta_k^\top T(x) - a_k(\theta_k)) \approx \hq_X\{x\}.
\]
A more robust approach is to minimize the discrepancy between the two sides with respect to the $\theta_k$'s:
\begin{equation}
\{\htheta_k\}_{k=1}^K \in \argmin_{\{\theta_k\}_{k=1}^K}D\left(\textstyle\hq_X\{x\}\|\sum_{k=1}^K\hp\{x,Y=k\}w_k\exp(\theta_k^\top T(x) - a_k(\theta_k))\right),
\label{eq:robust-distribution-matching}
\end{equation}
where $D$ is a discrepancy between probability distributions on $\cX$. For example if $D$ is the Kulback-Leibler (KL) divergence, then \eqref{eq:robust-distribution-matching} is
\begin{equation}
\begin{aligned}
\{\htheta_k\}_{k=1}^K &\in \argmin_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\hq_X\{X\} - \log\left(\sum_{k=1}^K\hp\{X,Y=k\}\exp(\theta_k^\top T(X) - a_k(\theta_k))\right)\right] \\
% &=\argmin_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\hq_X\{X\} - \log\hp_X\{X\} - \log\left(\sum_{k=1}^K\big[\heta_P(X)\big]_k\exp(\theta_k^\top T(X))\right)\right] \\
&\equiv\argmax_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\left(\sum_{k=1}^K\big[\heta_P(X)\big]_k\exp(\theta_k^\top T(X) - a_k(\theta_k))\right)\right],
\end{aligned}
\label{eq:KL-distribution-matching}
\end{equation}
where $\hQ_X$ is the empirical distribution of the (unlabeled) samples from the target domain and $\heta_P:\cX\to\Delta^{K-1}$ is an estimate of the regression function in the source domain:
\[
\big[\eta_P(x)\big]_k \triangleq P\{Y=k\mid X=x\}.
\]
One benefit of minimizing the KL divergence is the learner does not need to estimate the $p\{x,Y=k\}$'s; they merely need to train a discriminative model to estimate $\eta_P$ from the (labeled) samples from the source domain. In other words, the learner does not needs to train generative models. 

% \YK{Subha's convex method here}

We note that the consistency of \eqref{eq:robust-distribution-matching} depends on the identifiability of the $\theta_k$'s from  \eqref{eq:distribution-matching}; \ie\ the uniqueness of the $\theta_k$'s that satisfy \eqref{eq:distribution-matching}. As long as the $\theta_k$'s are identifiable, then \eqref{eq:robust-distribution-matching} provides consistent estimates of the $\theta_k$'s. Unfortunately, without additional assumptions on the $p\{x,Y=k\}$'s and $T$, the $\theta_k$'s are generally unidentifiable from \eqref{eq:distribution-matching} (see section \ref{sec:identifiability} for an example). We elaborate on the identifiability of the exponential tilt model in section \ref{sec:identifiability}.

\paragraph{Train classifier for target domain} Armed with estimates $\htheta_k$'s of the $\theta_k$'s, we train a classifier for the target domain by weighted ERM in the second step:
\begin{equation}
\heta_Q\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\exp(\htheta_Y^\top T(X))\right],
\label{eq:weighted-ERM}
\end{equation}
where $\ell$ is a loss function. The weight function in \eqref{eq:weighted-ERM} is chosen so that expected value of the cost function in \eqref{eq:weighted-ERM} is exactly the risk in the target domain:
\[
\begin{aligned}
\Ex_P\left[\ell(f(X),Y)\exp(\theta_Y^\top T(X))\right] &= \sum_{k=1}^K\Ex_P\left[\ell(f(X),k)\exp(\theta_k^\top T(X))\ones\{Y=k\}\right] \\
&= \sum_{k=1}^K\Ex_Q\left[\ell(f(X),k)\ones\{Y=k\}\right] \\
&= \Ex_Q\left[\ell(f(X),Y)\right],
\end{aligned}
\]
where we recalled $q\{x,Y=k\} = p\{x,Y=k\}\exp(\theta_k^\top T(x))$ in the second step. Alternatively, it is also possible to plug in estimates of the $p\{x,Y=k\}$'s and the $\theta_k$'s into $\eta_Q$ to obtain
\[
\heta_Q(x) \gets \frac{\hp\{x,Y=k\}\exp(\theta_k^\top T(x))}{\sum_{l=1}^K\hp\{x,Y=l\}\exp(\theta_l^\top T(x))}.
\]
We prefer weighted ERM because it avoids estimating the $p\{x,Y=k\}$'s and it is more robust to model misspecification. \YK{elaborate on robustness to model misspecification}

\begin{algorithm}
\caption{ExTRA: Exponentailly tilted reweighted adaptation}\label{alg:DAET}
\begin{algorithmic}[1]
\State train classifier for source domain: $\heta_P\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\right]$
\State fit exponential tilt model:
\[
\{\htheta_k\}_{k=1}^K\in\argmax_{\{\theta_k\}_{k=1}^K}\Ex_{\hQ_X}\left[\textstyle\log\left(\sum_{k=1}^K\big[\heta_P(X)\big]_k\exp(\theta_k^\top T(X))\right)\right]
\]
\State train classifier for target domain: $\heta_Q\in\argmin_{f\in\cF}\Ex_{\hP}\left[\ell(f(X),Y)\exp(\htheta_Y^\top T(X))\right]$
\end{algorithmic}
\end{algorithm}


==> sections/expt.tex <==
\section{Experiments}

\subsection{LDA}
We evaluate the performance of the exponentially tilted approach on a simulated data from LDA model. The source ($P$) distribution is a mixture of the two classes ($y = \pm 1$) with probability for class $y = -1$ being $0.75$ , and the class conditional distributions are $x | y \sim N\big((y, y)^\top, I_2\big), ~ y = \pm 1$. The target ($Q$) is also a mixture of two classes with equal probability for the two classes and the class conditional distributions $x | y \sim N\big((-y, y)^\top, I_2\big), ~ y = \pm 1$.    The data-points are plotted in Figure \ref{fig:LDA} along with the decision boundaries. The boundary with unlabeled target distribution is obtained using the exponentially tilted model where the tilt parameters (with $T(x) = x_1$) are calculated from the MLE approach \eqref{eq:mle}.
\begin{figure}
 \vspace{.05in}
\centering
\includegraphics[width=\linewidth]{plots/LDA.pdf}
\vspace{-.3in}
\caption{}
%  \vspace{-.05in}
\label{fig:LDA}
\end{figure}

==> sections/linear-independence.tex <==
\subsection{Linear independence}

\paragraph{Exponential tilting} Let $\{p_k(x)\}_{k=1}^K$ be the class conditionals in the training domain, and $q(x)$ be the (marginal) density of the features in the target domain. We wish to show that is a unique set of $\theta_k$'s such that
\[
\sum_{k=1}^Kp_k(x)e^{\theta_k^\top T(x)} = q(x),
\]
where $T(x)$ is a vector of sufficient statistics that includes a constant entry. Suppose there is another set of $\eta_k$'s that satisfies the preceding equation. We must have
\begin{equation}
\sum_{k=1}^Kp_k(x)(e^{\theta_k^\top T(x)} - e^{\eta_k^\top T(x)}) = 0.
\label{eq:difference-zero}
\end{equation}
We assume
\begin{equation}
\{p_k(x)(e^{\theta_k^\top T(x)} - e^{\eta_k^\top T(x)})\}_{k=1}^K\text{ is linearly independent for any $\theta_k$'s and $\eta_k$'s such that $\theta_k \neq \eta_k$.}
\label{eq:linear-independence}
\end{equation}
This implies \eqref{eq:difference-zero} occurs if and only if the terms in the sum are all zero:
\[
p_k(x)(e^{\theta_k^\top T(x)} - e^{\eta_k^\top T(x)}) = 0,\quad k\in[K],
\]
which implies $e^{\theta_k^\top T(x)} = e^{\eta_k^\top T(x)},
$ because $p_k \ne 0$. We appeal to Lemma \ref{lemma:linear-indep} to deduce $\theta_k = \eta_k$.

The linear independence assumption seems restrictive because it requires linear independence for any choice of $\theta_k$'s and $\eta_k$'s, but it is actually mild. For example, if the supports of the $p_k$'s are disjoint, then \eqref{eq:linear-independence} is satisfied. A milder (sufficient) condition is there are points $x_1,\dots,x_K$ such that $p_k(x_k) > 0$ but $p_{l\ne k}(x_k) = 0$ for all $k$. This condition is motivated by the identification restrictions in \cite{gong2016Domain,tachet2020Domain}.

\paragraph{General parametric model} Instead of tilting, consider a general parametric model for the class conditionals in the target domain:
\[
q_k(x) = (A_{\theta_k}p_k)(x),
\]
where $\cA \triangleq \{A_\theta:\theta\in\Theta\}$ is a parameterized family of Markov kernels. If we assume 
\begin{equation}
\{A_{\theta_k}p_k - A_{\eta_k}p_k\}_{k=1}^K\text{ is linearly independent for any $\theta_k$'s and $\eta_k$'s such that $\theta_k\ne\eta_k$},
\label{eq:general-linear-independence}
\end{equation}
then (a version of) the preceding argument shows that the target class conditionals are identifiable. We interpret \eqref{eq:general-linear-independence} is a restriction on the richness of the family of Markov kernels: if there is $\theta$ such that $p_k = A_{\theta}p_l$ for a pair of (distinct) class conditionals, then \eqref{eq:general-linear-independence} fails.

Another way to interpret \eqref{eq:general-linear-independence} is a well-separation condition on the $p_k$'s. t

==> sections/methods.tex <==
Given that they are identifiable one can estimate the parameters  from the following estimating equation: 
    \[
    E_{Q_X}[f] = \pi_Q E_{P_0}\big[ f(x) e^{\beta_0^\top \Phi(x)} \big] + (1 - \pi_Q) E_{P_1}\big[ f(x) e^{\beta_1^\top \Phi(x)} \big]
    \] Here, the related questions follow. \emph{1. What is a  good choices of $f$? 2. What is the rate of convergence for the parameters? 3. What is the rate of convergence for excess risk? This may involve a non-vanishing error term to capture a model misspecification.}  

==> sections/theory.tex <==
\section{Theoretical properties of distribution matching}

\subsection{Identifiability of the exponential tilt model}
\label{sec:identifiability}
To show that the $\theta_k$'s are identifiable from \eqref{eq:distribution-matching}, we must show that there is a unique solution to \eqref{eq:distribution-matching}. Unfortunately, this is impossible without additional assumptions. For example, consider a linear discriminant analysis (LDA) problem in which the class conditionals drift between the source and target domains:
\[
\begin{aligned}
p\{x,Y=k\} &= \pi_k\phi(x-\mu_{P,k}) \\
q\{x,Y=k\} &= \pi_k\phi(x-\mu_{Q,k})
\end{aligned},
\]
where $\phi$ is the standard MVN density. Here the $\pi_k\in(0,1)$ are the class proportions in both source and target domains, while the $\mu_{P,k}$'s (resp.\ the $\mu_{Q,k}$'s) are the class conditional means in the source (resp.\ target) domain. We see that this problem satisfies the exponential tilt model with $T(x) = (1,x)$:
\[
\log\frac{q\{x,Y=k\}}{p\{x,Y=k\}} = (\mu_{Q,k} - \mu_{P,k})^\top x .
\]
Unfortunately, this instance of the exponential tilt model is not identifiable; any permutation of the class labels $\sigma:[K]\to[K]$ also leads to the same (marginal) distribution of inputs:
\[
\begin{aligned}
&\sum_{k=1}^Kp\{x,Y=k\}\exp\left(\textstyle(\mu_{Q,k} - \mu_{P,k})^\top x + \frac12\|\mu_{P,k}\|_2^2 - \frac12\|\mu_{Q,k}\|_2^2\right) \\
&\quad= \sum_{k=1}^Kp\{x,Y=\sigma(k)\}\exp\left(\textstyle(\mu_{Q,k} - \mu_{P,\sigma(k)})^\top x + \frac12\|\mu_{P,\sigma(k)}\|_2^2 - \frac12\|\mu_{Q,k}\|_2^2\right).
\end{aligned}
\]
From this example, we see that the non-identifiability of the exponential tilt model is closely related to the label switching problem in clustering. Intuitively, the exponential tilt model in the preceding example is too flexible because it can tilt any $p\{x,Y=k\}$ to $q\{x,Y=l\}$. Thus there is ambiguity in which $p\{x,Y=k\}$ tilts to which $q\{x,Y=l\}$. In the rest of this subsection, we present two identification restrictions that guarantee the exponential tile model is identifiable.

\subsubsection{Anchor sets} 

A standard identification restriction in related work on domain adaptation is a clustering assumption. For example, \citet{tachet2020Domain} assume there is a partition of $\cX$ into disjoint sets $\cX_k$ such that $\supp(P\{\cdot\mid Y=k\}),\supp(Q\{\cdot\mid Y=k\}) \subset \cX_k$ for all $k\in[K]$. This assumption is strong: it implies there is a perfect classifier in the source and target domains. Here we consider a weaker version of the clustering assumption: there are sets $\cS_k$ such that
\[
P\{Y=k\mid X\in\cS_k\} = Q\{Y=k\mid X\in\cS_k\} = 1.
\]
We note that the $\cS_k$'s can be much smaller than the $\cX_k$'s; this permits the supports of $P\{\cdot\mid Y=k\}$ and $P\{\cdot\mid Y=l\}$ to overlap. 

\begin{definition}[anchor set]
\label{def:anchor-set}
A set $\cS\subset\cX$ is an \textbf{anchor set} if $p\{x,Y=k\} > 0$ and $p\{x,Y=l\} = 0$, $l\ne k$ for all $x\in\cS$.
\end{definition}

% In terms of the regression function (in the source domain) $\eta_P$, an anchor set for the $k$-th class is a set of points such that $\big[\eta_P(x)\big]_k = 1$.

\begin{proposition}[identifiability from anchor sets]
\label{prop:anchor-points} 
If there are anchor sets $\cS_k$ for all $K$ classes (in the source domain) and $T(\cS_k)$ is $d$-dimensional, then there is at most one set of $\theta_k$'s that satisfy \eqref{eq:distribution-matching}.
\end{proposition}

\begin{proof}
Suppose there are two sets of tilt parameters $\theta_k$'s and $\eta_k$'s that satisfy \eqref{eq:distribution-matching}:
\[
q_X\{x\} = \sum_{k=1}^Kp\{x,Y=k\}\exp(\theta_k^\top T(x)) = \sum_{k=1}^Kp\{x,Y=k\}\exp(\eta_k^\top T(x)).
\]
For any $x\in\cS_k$, the terms that include $p\{x,Y=l\}$, $l\ne k$ vanish:
\[
p\{x,Y=k\}\exp(\theta_k^\top T(x)) = p\{x,Y=k\}\exp(\eta_k^\top T(x)).
\]
This implies
\[
\theta_k^\top T(x) = \eta_k^\top T(x)\text{ for all }x\in\cS_k.
\]
We conclude $\theta_k = \eta_k$ because $T(\cS_k)$ is  $d$-dimensional, so there are $d$ points $x_1,\dots,x_d\in\cS_k$ such that $T(x_1),\dots,T(x_d)\in\reals^d$ are linearly independent. 
\end{proof}

This identification restriction is also closely related to the linear independence assumption in \citet{gong2016Domain}. Inspecting the proof of proposition \ref{prop:anchor-points}, we see that the anchor set assumption implies linear independence of $\{p_k(x)\exp(\theta_k^\top T(x))\}_{k=1}^K$ for any set of $\theta_k$'s.


\subsubsection{Invariant inputs/Anchor variables} 

In many applications, certain inputs are known to be invariant between the source and target domains. \my{really?}


\section{Generalization bound}
In this section we establish a generalization bound for the proposed domain adaptation method via exponential tilt. To begin with we define and recall some notations. 

\paragraph{Notations and definitions}
Recall that we consider a classification setup, \ie,  $\cY = [K]$  and $\ell: \reals^{K} \times \cY \to \reals$ is the appropriate 
loss for classification that we use in Algorithm \ref{alg:DAET}. We denote $\reals_{\ge 0}$ as the set of all non-negative real numbers and $\cF$ as the hypothesis class for all the classifiers. For an $f \in \cF$ and a weight function $\weight: \cX \to \reals_{\ge 0}^K $ we denote $\weight(x, j)$ as the $j$-th co-ordinate of $\weight(x)$ and define the weighted loss function and it's empirical version on source data as: 
\[ \textstyle
\cL_P(f, w) = \Ex_{(x, y) \sim P} [\weight(x, y)\ell(f(x), y)], ~ \hat \cL_P (f, w) = \frac 1 {\nsource} \sum_{i = 1}^\nsource  \weight(x_{P, i}, y_{P, i})\ell\{f(x_{P, i}), y_{P, i}\}\,.
\] We also define the loss function on the target data as: 
\[
\cL_Q(f) = \Ex_{(x, y) \sim Q} \big[\ell(f(x), y)\big]\,.
\] 
If $\{(\alpha_k^\star, \theta_k^\star)\}_{k = 1}^K$ is the true value of the tilt parameters in  \eqref{eq:exponential-tilt}, \ie, the following holds:
\[ \textstyle
  q\{x, Y = k\} = p\{x, Y = k\} \exp\{\alpha_k^\star + (\theta_k^\star)^\top T(x)\}; \ k \in [K]\,,
\] then defining $\weight^\star(x, k) = \exp\{\alpha_k^\star + (\theta_k^\star)^\top T(x)  \}$ as the true weight function we notice that  $\cL_P(f, \weight^\star) = \cL_Q(f)$ as we show in the  following display:
\[ \textstyle
\begin{aligned}
\cL_P(f, \weight^\star) 
 & = \int \sum_{y= 1}^K \weight^\star (x, y) \ell\{f(x), y\} p\{x, Y = y\} dx\\
 & = \int \sum_{y= 1}^K  \ell\{f(x), y\} q\{x, Y = y\} dx=\cL_Q(f)\,.
\end{aligned}
\] 

We next define the Rademacher complexity that  has been frequently used in  machine learning literature to establish a generalization bound. 
Instead of considering the Rademacher complexity on $\cF$ we define the class of weighted losses $\cG(\ell, \cF) = \{g_f(x, y) = w^\star(x, y) \ell(f(x), y): \ f \in \cF\}$  and for $n \in \bbN$ we define it's Rademacher complexity measure as 
\[ \textstyle
    \cR_n(\cG) \triangleq \Ex_{\{(u_i, v_i)\}_{i = 1}^n\stackrel{\IID}{\sim} P} \big[\Ex_{\{\xi_i\}_{i = 1}^n}[\sup_{f \in \cF} \frac1{n} \sum_{i = 1}^n \xi_i \weight^\star(u_i, v_i) \ell \{f(u_i), v_i\}]\big]
\]
where $\{\xi_i\}_{i = 1}^n $ are \IID \ symmetric Rademacher random variables. 
To establish our generalization bound we need the following  assumption on the loss function.

\begin{assumption}
\label{assump:bounded-loss}
The loss function $\ell$ is bounded, \ie, there exists an $B>0$ such that for any $f\in \cF$, $x \in \cX$ and $y \in [K]$ it holds: $|\ell\{f(x), y\}| \le B$. 
\end{assumption}

With the above definitions and the assumption we're now ready to establish our generalization bound. 

\begin{theorem}
\label{th:generalization-bound} For a weight function $\weight$ and the source samples $\{(x_{i, P}, y_{i, P})\}_{i = 1}^\nsource$ of size $\nsource$ let $\hat f_{\weight} = \argmin_{f\in\cF} \hat \cL_P(f, \weight)$. There exists a constant $c> 0$ such that  the following generalization bound holds with probability at least $1 -\delta$
\begin{equation}\textstyle
\label{eq:gen-bound}
    \cL_Q(\hat f_{ \weight}) - \min_{f\in\cF}\cL_Q (f) \le  2 \cR_m(\cG) + B  \| \weight - w^\star \|_{1, P} + c \sqrt{\frac{\log(1/\delta)}{m}} \,.
\end{equation}
\end{theorem}

From the above bound we notice that a  weight function $\weight$ with small $\|\omega - \omega^\star \|_{1, P}$  is crucial to have a classifier on target population with a small generalization bound. In the next subsection we study the property of the weight function $\hat \omega$ with $\hat \omega(x, k) = \exp\{ \hat \alpha_k + {\hat \theta_k}^\top T(x) \}$ where $\{(\hat \alpha_k, \hat \theta_k)\}_{k = 1}^K$ are obtained from Algorithm \ref{alg:DAET} and establish a rate of convergence for $\|\hat \omega - \omega^\star \|_{1, P}$. 

% We let $\ell$ to be the loss function under consideration and  denote the hypothesis class of classifiers as $\cF$. 
% For a weight function $w(x) = (w(x, 1), \dots , w(x, K))^\top$ and a classifier $f \in \cF$ let us define the weighted loss function and it's empirical version as the followings, 
% \begin{equation}
% \label{eq:weighted-loss}
% \begin{aligned}
% \cL(f, w, P) = \Ex_{(X, Y) \sim P} \big[w(X, Y)\ell(f(X), Y)\big]\,,\\
% \hat \cL(f, w) \equiv \cL(f, w, \hat P)  = \frac 1{n_P} \sum_{i = 1}^{n_P} w(X_i^{(P)}, Y_i^{(P)})\ell(f(X_i^{(P)}), Y_i^{(P)})\,.
% \end{aligned}
%     \end{equation} We also define the target loss function as
%     \begin{equation}
%     \label{eq:true-loss}
%     \cL_\star(f) =    \Ex_{(X, Y) \sim Q} \big[\ell(f(X), Y)\big] \,.
%     \end{equation}
%     Let $\{(\alpha_k^\star, \theta_k^\star)\}_{k= 1}^K$ be the true values of the tilt parameters, \ie, the followings hold:
%     \begin{equation}
%         q\{x, Y = k\} = p\{x, Y = k\} \exp\big(\alpha_k^\star + (\theta_k^\star)^\top T(x)  \big); \ k \in [K]\,.
%     \end{equation} We define the true weight function $w^\star$ as 
%     \begin{equation}
% \begin{aligned}
% w^\star(x) = (w^\star(x, 1), \dots, w^\star(x, K))^\top\,, \\
% w_k^\star(x) = \exp\big(\alpha_k^\star + (\theta_k^\star)^\top T(x)  \big); \ k \in [K]\,.
% \end{aligned}
%          \end{equation} One may notice that weighted loss function \eqref{eq:weighted-loss} at the true weight function $w^\star$ is the target loss function, as suggested by the following calculations:
% \[\textstyle
% \begin{aligned}
% \cL(f, w^\star, P) &= \Ex_{(X, Y) \in P} \big[ w^\star (X, Y) \ell(f(X), Y) \big] \\
% & = \int \sum_{k= 1}^K w^\star (x, k) \ell(f(x), k) p\{x, Y = k\} dx\\
% & = \int \sum_{k= 1}^K  \ell(f(x), k) q\{x, Y = k\} dx=\cL_\star(f)\,.
% \end{aligned}
% \] We define the set $\cG(\ell, \cF) = \{g_f(x, y) = w^\star(x, y) \ell(f(x), y): \ f \in \cF\}$ and it's Rademacher complexity measure
% \begin{equation}
%     \label{eq:rademacher}
%     \cR_n(\cG) \triangleq \Ex_{(X_i, Y_i)\sim P: i\in [n]} \Big[\Ex_{\xi_i:i\in [n]}\Big[\sup_{f \in \cF} \frac1{n} \sum_{i = 1}^n \xi_i w^\star(X_i, Y_i) \ell (f(X_i), Y_i)\Big]\Big]
% \end{equation}
%  with $\xi_i: i\in [n]$ are \IID\ Rademacher random variables. 





\subsection{Estimation of the tilt parameters and the weight function}
Here, for notational simplicity, we define $\coef_k = (\alpha_k, \theta_k^\top )^\top$'s
as the tilt parameters, $\coef_k^\star = (\alpha_k^\star, {\theta_k^\star}^\top )^\top$'s as their true values, $S(x) = (1, T(x)^\top )^\top $ as the sufficient statistics for exponential tilt and $\coef = (\coef_1^\top, \dots, \coef_K^\top)^\top\in \reals^{K(d+1)}$ as the long vector containing  all the tilt parameters. 
We recall from Algorithm \ref{alg:DAET} that estimation of the tilt parameters $\coef$ requires a classifier $\hat \eta_P$ on the source data. So, we define our objective for estimating $\coef$ through a generic  classifier $\eta : \cX \rightarrow \Delta^{K}$. Denoting $\eta_k(x)$ as the $k$-th co-ordinate of $\eta(x)$ we define the expected log-likelihood objective as:
\[
\textstyle
\klloss(\eta, \coef) = \Ex_{Q_X}[\log \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}] - \log [\Ex_{P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}]\,,
\] and its empirical version as 
\[
\textstyle
\hat \klloss(\eta, \coef) = \Ex_{\hat Q_X}[\log \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}] - \log [\Ex_{\hat P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}]\,.
\] The term   $\log [\Ex_{P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}]$ in the log-likelihood objective works as a normalizer: for any $\eta : \cX \to \Delta^K$ the function $[ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) ]/[\Ex_{P_X} \{ \sum_{k = 1}^K \eta_k(x) \exp(\coef_k^\top S(x)) \}] $ is a density over the support $\cX$ with respect to the base measure $P_X$. Furthermore, plugging in the Bayes classifier $\eta^\star_P$ (defined as $\eta^\star_{P, k}(x) = p\{x, Y = k\}/p_X(x)$) and  $\scoef$ we realize that the quantity $\sum_{k = 1}^K \eta_{P, k}^\star(x) \exp(\coef_k^\top S(x))$ is a density with respect to the base measure $P_X$, as we explain in the following display: 
\[\textstyle
\sum_{k = 1}^K \eta_{P, k}^\star(x) \exp\{{\coef_k^\star}^\top S(x)\} = \sum_{k = 1}^K \frac{p\{x, Y = k\}}{p_X(x)} \exp\{{\coef_k^\star}^\top S(x)\} =  \frac{\sum_{k = 1}^K q\{x, Y = k\}}{p_X(x)} = \frac{q_X(x)}{p_X(x)}
\]
and hence it holds $\Ex_{P_X} \{ \sum_{k = 1}^K \eta_{P, k}^\star(x) \exp\{{\coef_k^\star}^\top S(x)\} = 1$. In the next lemma we establish that $\scoef$ is the unique maximizer of $\klloss(\eta_P^\star, \coef)$, which is crucial for establishing that $\hcoef$ converges to $\scoef$. 

\begin{lemma}\label{lemma:uniqueness}
$\coef \mapsto \klloss(\eta_P^\star, \coef)$ is uniquely maximized at $\scoef$. 
\end{lemma}



We next make the assumption that is standard in establishing consistency of MLE. 

\begin{assumption}
\label{assmp:strong-convexity}
The loss $\coef \mapsto -\klloss(\eta^\star_P, \coef)$ is  strongly convex at $\scoef$, \ie, there exists a constant $\strongconvexity>0$ such that for any $\coef$ it holds:
\[
-\klloss(\eta^\star_P, \coef) \ge -\klloss(\eta^\star_P, \scoef) - \partial_\coef\klloss(\eta^\star_P, \scoef)  ^\top (\coef - \scoef) +\frac{\mu}{2}\|\coef - \scoef\|_2^2\,. 
\]
\end{assumption}
We note that the assumption is a restriction on the distribution $Q_X$ rather than the objective itself. For technical convenience we next assume that the feature space is bounded. 


\begin{assumption} \label{assump:bounded-covariate}
$\cX$ is bounded, \ie, there exists  an $M>0$ such that $\cX \subset B(0, M)$.
\end{assumption}

Recall, from Algorithm \ref{alg:DAET}, that we need a fitted source classifier $\hat \eta_P$  to estimate the tilt parameter: $\scoef$ is estimated by maximizing $\klloss(\hat \eta_P, \coef)$ rather than the unknown $\klloss(\eta_P^\star, \coef)$. While analyzing the convergence $\hcoef$ we need to control the difference  $\klloss(\hat \eta_P, \coef) - \klloss(\eta_P^\star, \coef)$, which requires the pre-activated logit functions for $\hat \eta_P$ to be close to $\eta_P^\star$. Though the pre-activation logit functions are not unique for a classifier as \[
\textstyle
\frac{\exp(f_k(x))}{\sum_{j = 1}^K \exp(f_j(x))} = \frac{\exp(f_k(x)+a(x))}{\sum_{j = 1}^K \exp(f_j(x) +a(x))}
\] holds  for any $f: \cX \to \reals^K$ and $a:\cX\to \reals$, we notice that the centered logit function of the classifier is unique, \ie, 
\[ \textstyle
\frac{\exp(f_k(x))}{\sum_{j = 1}^K \exp(f_j(x))} =  \eta(x), ~ \sum_{j = 1}^K{f_j(x)} = 0  \Longleftrightarrow f_k(x) = \log\{\eta_k(x)\} - \frac1K \sum_{j = 1}^K \log\{\eta_j(x)\}\,.\]
We next assume that the centered logit for $\hat \eta_P$ convegres to the one for $\eta_P^\star $. 

\begin{assumption}
\label{assmp:source-classifier}
Let $f_{k}^\star(x) = \log\{\eta_{P, k}^\star(x)\} - \frac 1K \sum_{j = 1}^K \log\{\eta_{P, j}^\star(x)\}$. We assume that there exist an estimator $\{\hat f _k(x)\}_{k =1 }^K$ for $\{f^\star_k(x)\}_{k = 1}^K$ such that the following holds: there exists a constant $c>0$ such that  for almost surely $[\bbP_X]$  it holds
\[
\Pr(\|\hat f(x) - f^\star(x)\|_{2} > t) \le \exp(-c t^2 /r_m^2), ~ t > 0\,.
\]
\end{assumption}



Having such an estimator we construct $\hat \eta_P$ as $\hat \eta_{P, k}(x) = \exp(\hat f_k(x))/\{\sum_{j = 1}^K \exp(\hat f_j(x))\}$, which we shall use in Algorithm \ref{alg:DAET} to estimate $\hcoef$and set the weights $\hat \weight$ as $\hat \weight(x, k) = \exp\{\hcoef_k^\top S(x)\}$.  With the above assumptions we're ready to establish the concentration for $\hcoef - \scoef$ and  $\hat \weight - \weight^\star$.
\begin{lemma} \label{lemma:tilt-concentration}
Let the assumptions \ref{assmp:strong-convexity}, \ref{assump:bounded-covariate} and \ref{assmp:source-classifier} hold. For the sample sizes $m, n$ define $\alpha_{m, n} = r_m \sqrt{\log(m+n)}+ m ^{-1/2} + n^{-1/2}$. There exists constants $k_1, k_2>0$ such that with probability at least the following hold:
\[
\|\htheta - \stheta \|_2 \le k_1 \alpha_{m, n}\sqrt{\log(1/\delta)}, \text{ and } \|\hat \weight - \weight^\star\|_{1, P} \le k_2 \alpha_{m, n}\sqrt{\log(1/\delta)}. 
\]
\end{lemma}

\begin{corollary}
Combining the results in Theorem \ref{th:generalization-bound} and Lemma \ref{lemma:tilt-concentration} we conclude that there exists a $k_3>0$ such that  with probability at least $1 - (2K + 2)\delta$ the following holds:
\[
\cL_Q(\hat f_{\hat w}) - \min_{f}\cL_Q (f) \le  2 \cR_m(\cG) + k_3 \alpha_{m,n}\sqrt{\log(1/\delta)}\,.
\]
\end{corollary}

\my{summarize the implications of theoretical results}


